Massive Stars in the Range $\rm 13-25 M_\odot$: Evolution and Nucleosynthesis. II. the Solar Metallicity Models

We present the evolutionary properties of a set of massive stellar models (namely 13, 15, 20 and 25 $\rm M_\odot$) from the main sequence phase up to the onset of the iron core collapse. All these models have initial solar chemical composition, i.e. Y=0.285 and Z=0.02. A 179 isotope network, extending from neutron up to $\rm ^{68}Zn$ and fully coupled to the evolutionary code has been adopted from the Carbon burning onward. Our results are compared, whenever possible, to similar computations available in literature.

==> tablsc1.tex <==
\begin{deluxetable}{lcclcc}
\tablenum{1}
\tablewidth{0pt}
\tablecaption{Nuclear network adopted in the calculations \label{network}}
\tablehead{
\colhead{Element} &
\colhead{$\rm A_{min}$}  &
\colhead{$\rm A_{max}$}    &
\colhead{Element} &
\colhead{${\rm A_{min}}$}  &
\colhead{${\rm A_{max}}$}  
}
\startdata
n     & 1  & 1  & S   & 31 & 37   \nl
H     & 1  & 3  & Cl  & 33 & 37   \nl
He    & 3  & 4  & Ar  & 36 & 41   \nl
Li    & 6  & 7  & K   & 37 & 42   \nl
Be    & 7  & 10 & Ca  & 40 & 49   \nl
B     & 10 & 11 & Sc  & 41 & 49   \nl
C     & 12 & 14 & Ti  & 44 & 51   \nl 
N     & 13 & 16 & V   & 45 & 52   \nl
O     & 15 & 19 & Cr  & 48 & 55   \nl
F     & 17 & 20 & Mn  & 51 & 57   \nl
Ne    & 20 & 23 & Fe  & 52 & 61   \nl
Na    & 21 & 24 & Co  & 55 & 61   \nl
Mg    & 23 & 27 & Ni  & 56 & 65   \nl
Al    & 25 & 28 & Cu  & 57 & 66   \nl
Si    & 27 & 32 & Zn  & 64 & 68   \nl
P     & 29 & 34 &     &    &      \nl
\enddata
\end{deluxetable}                                                                               


==> tablsc10.tex <==
\begin{deluxetable}{lrrrrrrrrr}
%\small
\tablenum{10}
\tablewidth{16cm}
\tablecaption{Presupernova nucleosynthesis of the $\rm 13~M_\odot$ model} 
\tablehead{
\colhead{Isotope}     &
\colhead{Si}    &
\colhead{O}    &
\colhead{Ne}    &
\colhead{C}    &
\colhead{$\rm He_{\rm c}$}    &
\colhead{$\rm He_{\rm sh}$}    &
\colhead{$\rm H_{\rm sh}$}    &
\colhead{$\rm H_{\rm c}$}    &
\colhead{Yield ($\rm M_\odot$)}  
}
\startdata  
$\rm ^{1 }H $   &    0   &      0   &      0    &     0    &     0   &      0    &     0   &     99 & 6.11(+00) \nl
$\rm ^{2 }H $   &    0   &      0   &      0    &     0    &     0   &      0    &     0   &     99 & 1.74(-16) \nl
$\rm ^{3 }H $   &    0   &      0   &      0    &     0    &     0   &      0    &    99   &      0 & 2.60(-40) \nl
$\rm ^{3 }He$   &    0   &      0   &      0    &     0    &     0   &      0    &     0   &     99 & 2.07(-04) \nl
$\rm ^{4 }He$   &    0   &      0   &      0    &     0    &     0   &     23    &     8   &     68 & 4.56(+00) \nl
$\rm ^{6 }Li$   &    0   &      0   &      0    &     0    &     0   &      0    &     0   &     99 & 1.11(-09) \nl
$\rm ^{7 }Li$   &    0   &      0   &      0    &     0    &     0   &      0    &     0   &     99 & 1.62(-10) \nl
$\rm ^{7 }Be$   &    0   &      0   &      0    &     0    &     0   &      0    &    99   &      0 & 3.68(-26) \nl
$\rm ^{9 }Be$   &    0   &      0   &      0    &     0    &     0   &      0    &     0   &     99 & 2.85(-10) \nl
$\rm ^{10}Be$   &    0   &      0   &      0    &     0    &     0   &      0    &     0   &     99 & 1.21(-39) \nl
$\rm ^{10}B $   &    0   &      0   &      0    &     0    &     0   &      0    &     0   &     99 & 1.84(-09) \nl
$\rm ^{11}B $   &    0   &      0   &      0    &     0    &     0   &      0    &     0   &     99 & 1.35(-08) \nl
$\rm ^{12}C $   &    0   &      0   &      0    &     1    &     0   &     82    &     0   &     14 & 1.38(-01) \nl
$\rm ^{13}C $   &    0   &      0   &      0    &     0    &     0   &      0    &     2   &     97 & 1.21(-03) \nl
$\rm ^{14}C $   &    0   &      0   &      0    &     0    &     0   &     99    &     0   &      0 & 8.22(-07) \nl
$\rm ^{13}N $   &    4   &      0   &      0    &    95    &     0   &      0    &     0   &      0 & 2.81(-16) \nl
$\rm ^{14}N $   &    0   &      0   &      0    &     0    &     0   &      2    &    13   &     83 & 3.96(-02) \nl
$\rm ^{15}N $   &    0   &      0   &      0    &     0    &     0   &      2    &     1   &     96 & 1.77(-05) \nl
$\rm ^{16}N $   &   63   &      0   &      0    &    36    &     0   &      0    &     0   &      0 & 2.74(-22) \nl
$\rm ^{15}O $   &    1   &     12   &      2    &    83    &     0   &      0    &     0   &      0 & 1.87(-14) \nl
$\rm ^{16}O $   &    0   &      1   &     20    &    35    &     0   &     22    &     0   &     19 & 4.20(-01) \nl
$\rm ^{17}O $   &    0   &      0   &      0    &     0    &     0   &      0    &     0   &     99 & 1.11(-04) \nl
$\rm ^{18}O $   &    0   &      0   &      0    &     0    &     0   &     82    &     0   &     17 & 8.19(-04) \nl
$\rm ^{19}O $   &    0   &      0   &      0    &    99    &     0   &      0    &     0   &      0 & 6.74(-18) \nl
$\rm ^{17}F $   &   49   &     46   &      3    &     1    &     0   &      0    &     0   &      0 & 4.03(-17) \nl
$\rm ^{18}F $   &    0   &      0   &      0    &    99    &     0   &      0    &     0   &      0 & 9.23(-12) \nl
$\rm ^{19}F $   &    0   &      0   &      0    &     0    &     0   &     52    &     0   &     47 & 6.77(-06) \nl
$\rm ^{20}F $   &    0   &      0   &      0    &    99    &     0   &      0    &     0   &      0 & 6.09(-15) \nl
$\rm ^{20}Ne$   &    0   &      0   &      0    &    76    &     0   &      3    &     0   &     18 & 8.51(-02) \nl
$\rm ^{21}Ne$   &    0   &      0   &      0    &    50    &     0   &     43    &     0   &      6 & 5.67(-04) \nl
$\rm ^{22}Ne$   &    0   &      0   &      0    &     0    &     0   &     94    &     0   &      4 & 2.45(-02) \nl
$\rm ^{23}Ne$   &    0   &      0   &      0    &    99    &     0   &      0    &     0   &      0 & 8.99(-11) \nl
$\rm ^{21}Na$   &    0   &      0   &      0    &    99    &     0   &      0    &     0   &      0 & 5.33(-13) \nl
$\rm ^{22}Na$   &    0   &      0   &      0    &    99    &     0   &      0    &     0   &      0 & 6.60(-07) \nl
$\rm ^{23}Na$   &    0   &      0   &      0    &    73    &     0   &      8    &     2   &     16 & 3.30(-03) \nl
$\rm ^{24}Na$   &    0   &      0   &      0    &    99    &     0   &      0    &     0   &      0 & 2.44(-07) \nl
$\rm ^{23}Mg$   &    2   &      0   &      0    &    97    &     0   &      0    &     0   &      0 & 2.23(-10) \nl
$\rm ^{24}Mg$   &    0   &      0   &     33    &    45    &     0   &      2    &     0   &     17 & 2.87(-02) \nl
$\rm ^{25}Mg$   &    0   &      0   &      4    &    66    &     0   &     18    &     0   &      9 & 6.03(-03) \nl
$\rm ^{26}Mg$   &    0   &      0   &      6    &    50    &     0   &     21    &     1   &     19 & 4.21(-03) \nl
$\rm ^{27}Mg$   &    0   &      0   &      8    &    91    &     0   &      0    &     0   &      0 & 1.87(-08) \nl
$\rm ^{25}Al$   &    3   &      2   &      4    &    90    &     0   &      0    &     0   &      0 & 5.83(-14) \nl
$\rm ^{26}Al$   &    0   &      0   &     17    &    82    &     0   &      0    &     0   &      0 & 5.41(-07) \nl
$\rm ^{27}Al$   &    0   &      0   &     18    &    57    &     0   &      2    &     0   &     20 & 2.79(-03) \nl
$\rm ^{28}Al$   &    0   &      0   &     33    &    66    &     0   &      0    &     0   &      0 & 7.67(-07) \nl
$\rm ^{27}Si$   &    0   &      1   &     31    &    66    &     0   &      0    &     0   &      0 & 1.50(-09) \nl
$\rm ^{28}Si$   &    6   &     64   &     14    &     2    &     0   &      1    &     0   &      9 & 6.53(-02) \nl
$\rm ^{29}Si$   &    0   &      3   &     72    &     9    &     0   &      3    &     0   &     10 & 3.08(-03) \nl
$\rm ^{30}Si$   &    7   &      4   &     66    &     5    &     0   &      4    &     0   &     11 & 2.05(-03) \nl
$\rm ^{31}Si$   &    3   &      0   &     29    &    67    &     0   &      0    &     0   &      0 & 5.70(-07) \nl
$\rm ^{32}Si$   &    3   &      0   &     74    &    22    &     0   &      0    &     0   &      0 & 1.66(-07) \nl
$\rm ^{29}P $   &   89   &     10   &      0    &     0    &     0   &      0    &     0   &      0 & 2.49(-11) \nl
$\rm ^{30}P $   &    6   &      8   &     61    &    23    &     0   &      0    &     0   &      0 & 8.41(-08) \nl
$\rm ^{31}P $   &    3   &      7   &     68    &     4    &     0   &      4    &     0   &     10 & 7.49(-04) \nl
$\rm ^{32}P $   &    2   &      0   &     87    &     9    &     0   &      0    &     0   &      0 & 2.56(-06) \nl
$\rm ^{33}P $   &    3   &     11   &     83    &     2    &     0   &      0    &     0   &      0 & 3.78(-06) \nl
$\rm ^{34}P $   &   55   &      0   &     35    &     9    &     0   &      0    &     0   &      0 & 4.75(-11) \nl
$\rm ^{31}S $   &    0   &      6   &     93    &     0    &     0   &      0    &     0   &      0 & 4.32(-08) \nl
$\rm ^{32}S $   &    2   &     79   &      4    &     0    &     0   &      1    &     0   &     11 & 3.41(-02) \nl
$\rm ^{33}S $   &    4   &     61   &     15    &     0    &     0   &      4    &     0   &     11 & 2.72(-04) \nl
$\rm ^{34}S $   &   12   &     82   &      1    &     0    &     0   &      0    &     0   &      2 & 7.91(-03) \nl
$\rm ^{35}S $   &    9   &      0   &     50    &    26    &     0   &     12    &     0   &      0 & 1.92(-06) \nl
$\rm ^{36}S $   &    6   &      0   &     31    &    17    &     0   &     26    &     0   &     16 & 5.51(-06) \nl
$\rm ^{37}S $   &   92   &      0   &      0    &     7    &     0   &      0    &     0   &      0 & 5.90(-13) \nl
$\rm ^{33}Cl$   &   80   &     19   &      0    &     0    &     0   &      0    &     0   &      0 & 1.59(-12) \nl
$\rm ^{34}Cl$   &   38   &     58   &      3    &     0    &     0   &      0    &     0   &      0 & 1.45(-09) \nl
$\rm ^{35}Cl$   &    8   &     60   &      2    &     1    &     0   &      4    &     0   &     21 & 1.13(-04) \nl
$\rm ^{36}Cl$   &    9   &     30   &     26    &     8    &     0   &     24    &     0   &      0 & 9.16(-07) \nl
$\rm ^{37}Cl$   &    1   &      5   &     11    &    21    &     0   &     35    &     0   &     22 & 3.70(-05) \nl
$\rm ^{38}Cl$   &    3   &      0   &      1    &    95    &     0   &      0    &     0   &      0 & 1.41(-09) \nl
$\rm ^{36}Ar$   &    0   &     78   &      0    &     0    &     0   &      1    &     0   &     17 & 4.40(-03) \nl
$\rm ^{37}Ar$   &    7   &     83   &      1    &     0    &     0   &      7    &     0   &      0 & 1.41(-05) \nl
$\rm ^{38}Ar$   &    4   &     93   &      0    &     0    &     0   &      0    &     0   &      1 & 1.02(-02) \nl
$\rm ^{39}Ar$   &    1   &      0   &      0    &    35    &     0   &     62    &     0   &      0 & 2.26(-06) \nl
$\rm ^{40}Ar$   &    1   &      0   &     19    &    21    &     0   &     41    &     0   &     15 & 1.56(-06) \nl
$\rm ^{41}Ar$   &   11   &      0   &      3    &    84    &     0   &      0    &     0   &      0 & 1.65(-10) \nl
$\rm ^{37}K $   &   74   &     25   &      0    &     0    &     0   &      0    &     0   &      0 & 2.04(-14) \nl
$\rm ^{38}K $   &   31   &     68   &      0    &     0    &     0   &      0    &     0   &      0 & 2.13(-10) \nl
$\rm ^{39}K $   &    2   &     70   &      0    &     0    &     0   &      2    &     0   &     22 & 1.52(-04) \nl
$\rm ^{40}K $   &    1   &      1   &      5    &    23    &     0   &     58    &     0   &      9 & 6.00(-07) \nl
$\rm ^{41}K $   &    0   &      0   &      4    &     7    &     0   &     16    &     2   &     67 & 3.79(-06) \nl
$\rm ^{42}K $   &    2   &      0   &     27    &    69    &     0   &      0    &     0   &      0 & 5.65(-09) \nl
$\rm ^{40}Ca$   &    0   &     75   &      0    &     0    &     0   &      2    &     0   &     20 & 2.88(-03) \nl
$\rm ^{41}Ca$   &    0   &     80   &      0    &     2    &     0   &     15    &     0   &      0 & 1.07(-05) \nl
$\rm ^{42}Ca$   &    2   &     93   &      0    &     0    &     0   &      1    &     0   &      2 & 1.95(-04) \nl
$\rm ^{43}Ca$   &    3   &      7   &      4    &    13    &     0   &     23    &     1   &     46 & 1.90(-06) \nl
$\rm ^{44}Ca$   &    5   &      0   &      2    &     4    &     0   &     12    &     3   &     71 & 1.95(-05) \nl
$\rm ^{45}Ca$   &   18   &      0   &     16    &    30    &     0   &     35    &     0   &      0 & 2.50(-07) \nl
$\rm ^{46}Ca$   &   36   &      0   &     18    &     9    &     0   &     31    &     0   &      4 & 5.77(-07) \nl
$\rm ^{47}Ca$   &   81   &      0   &     13    &     4    &     0   &      0    &     0   &      0 & 5.89(-09) \nl
$\rm ^{48}Ca$   &    0   &      0   &      0    &     1    &     0   &     11    &     3   &     81 & 1.65(-06) \nl
$\rm ^{49}Ca$   &   60   &      0   &      0    &    39    &     0   &      0    &     0   &      0 & 2.48(-13) \nl
$\rm ^{41}Sc$   &   76   &     23   &      0    &     0    &     0   &      0    &     0   &      0 & 6.46(-16) \nl
$\rm ^{42}Sc$   &   44   &     54   &      0    &     1    &     0   &      0    &     0   &      0 & 1.68(-13) \nl
$\rm ^{43}Sc$   &   16   &     83   &      0    &     0    &     0   &      0    &     0   &      0 & 4.13(-09) \nl
$\rm ^{44}Sc$   &   25   &     69   &      4    &     0    &     0   &      0    &     0   &      0 & 2.45(-09) \nl
$\rm ^{45}Sc$   &   13   &      1   &      7    &    10    &     0   &     22    &     1   &     42 & 9.02(-07) \nl
$\rm ^{46}Sc$   &   81   &      0   &     12    &     5    &     0   &      0    &     0   &      0 & 5.43(-08) \nl
$\rm ^{47}Sc$   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 6.47(-07) \nl
$\rm ^{48}Sc$   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 1.03(-07) \nl
$\rm ^{49}Sc$   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 7.07(-07) \nl
$\rm ^{44}Ti$   &    0   &     99   &      0    &     0    &     0   &      0    &     0   &      0 & 1.16(-07) \nl
$\rm ^{45}Ti$   &   32   &     67   &      0    &     0    &     0   &      0    &     0   &      0 & 6.62(-09) \nl
$\rm ^{46}Ti$   &   51   &     37   &      0    &     0    &     0   &      1    &     0   &      7 & 2.73(-05) \nl
$\rm ^{47}Ti$   &   66   &      4   &      0    &     0    &     0   &      2    &     1   &     24 & 8.25(-06) \nl
$\rm ^{48}Ti$   &   94   &      0   &      0    &     0    &     0   &      0    &     0   &      4 & 4.62(-04) \nl
$\rm ^{49}Ti$   &   96   &      0   &      0    &     0    &     0   &      1    &     0   &      1 & 9.00(-05) \nl
$\rm ^{50}Ti$   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 3.03(-03) \nl
$\rm ^{51}Ti$   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 2.13(-06) \nl
$\rm ^{45}V $   &   91   &      8   &      0    &     0    &     0   &      0    &     0   &      0 & 3.61(-18) \nl
$\rm ^{46}V $   &   81   &     18   &      0    &     0    &     0   &      0    &     0   &      0 & 5.04(-14) \nl
$\rm ^{47}V $   &   91   &      8   &      0    &     0    &     0   &      0    &     0   &      0 & 9.13(-09) \nl
$\rm ^{48}V $   &   92   &      7   &      0    &     0    &     0   &      0    &     0   &      0 & 1.47(-07) \nl
$\rm ^{49}V $   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 3.96(-05) \nl
$\rm ^{50}V $   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 3.81(-05) \nl
$\rm ^{51}V $   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 2.86(-03) \nl
$\rm ^{52}V $   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 2.76(-05) \nl
$\rm ^{48}Cr$   &   62   &     37   &      0    &     0    &     0   &      0    &     0   &      0 & 1.56(-09) \nl
$\rm ^{49}Cr$   &   94   &      5   &      0    &     0    &     0   &      0    &     0   &      0 & 7.69(-08) \nl
$\rm ^{50}Cr$   &   98   &      0   &      0    &     0    &     0   &      0    &     0   &      1 & 6.74(-04) \nl
$\rm ^{51}Cr$   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 5.22(-04) \nl
$\rm ^{52}Cr$   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 1.47(-01) \nl
$\rm ^{53}Cr$   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 6.36(-03) \nl
$\rm ^{54}Cr$   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 9.59(-03) \nl
$\rm ^{55}Cr$   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 7.18(-06) \nl
$\rm ^{51}Mn$   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 3.22(-07) \nl
$\rm ^{52}Mn$   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 5.82(-06) \nl
$\rm ^{53}Mn$   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 6.41(-03) \nl
$\rm ^{54}Mn$   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 1.71(-03) \nl
$\rm ^{55}Mn$   &   98   &      0   &      0    &     0    &     0   &      0    &     0   &      1 & 1.11(-02) \nl
$\rm ^{56}Mn$   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 7.21(-05) \nl
$\rm ^{57}Mn$   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 5.12(-06) \nl
$\rm ^{52}Fe$   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 4.34(-09) \nl
$\rm ^{53}Fe$   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 4.77(-07) \nl
$\rm ^{54}Fe$   &   95   &      0   &      0    &     0    &     0   &      0    &     0   &      3 & 1.90(-02) \nl
$\rm ^{55}Fe$   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 8.48(-03) \nl
$\rm ^{56}Fe$   &   95   &      0   &      0    &     0    &     0   &      0    &     0   &      3 & 3.02(-01) \nl
$\rm ^{57}Fe$   &   94   &      0   &      0    &     0    &     0   &      1    &     0   &      2 & 1.01(-02) \nl
$\rm ^{58}Fe$   &   97   &      0   &      0    &     0    &     0   &      1    &     0   &      0 & 1.23(-02) \nl
$\rm ^{59}Fe$   &   98   &      0   &      0    &     1    &     0   &      0    &     0   &      0 & 2.98(-05) \nl
$\rm ^{60}Fe$   &   52   &      0   &      5    &    42    &     0   &      0    &     0   &      0 & 3.35(-06) \nl
$\rm ^{61}Fe$   &   89   &      0   &      0    &    10    &     0   &      0    &     0   &      0 & 3.81(-10) \nl
$\rm ^{55}Co$   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 3.19(-06) \nl
$\rm ^{56}Co$   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 1.52(-05) \nl
$\rm ^{57}Co$   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 1.62(-03) \nl
$\rm ^{58}Co$   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 3.64(-04) \nl
$\rm ^{59}Co$   &   94   &      0   &      0    &     1    &     0   &      2    &     0   &      1 & 1.92(-03) \nl
$\rm ^{60}Co$   &   98   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 4.26(-05) \nl
$\rm ^{61}Co$   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 1.37(-05) \nl
$\rm ^{56}Ni$   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 2.27(-08) \nl
$\rm ^{57}Ni$   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 3.64(-07) \nl
$\rm ^{58}Ni$   &   37   &      0   &      0    &     0    &     0   &      4    &     2   &     55 & 8.73(-04) \nl
$\rm ^{59}Ni$   &   95   &      0   &      0    &     0    &     0   &      4    &     0   &      0 & 1.69(-04) \nl
$\rm ^{60}Ni$   &   94   &      1   &      0    &     0    &     0   &      0    &     0   &      2 & 6.51(-03) \nl
$\rm ^{61}Ni$   &   94   &      0   &      0    &     1    &     0   &      2    &     0   &      1 & 6.60(-04) \nl
$\rm ^{62}Ni$   &   95   &      0   &      1    &     0    &     0   &      1    &     0   &      1 & 2.50(-03) \nl
$\rm ^{63}Ni$   &   50   &      0   &      0    &    25    &     0   &     23    &     0   &      0 & 4.98(-05) \nl
$\rm ^{64}Ni$   &   12   &      0   &     25    &    19    &     0   &     31    &     0   &     10 & 6.71(-05) \nl
$\rm ^{65}Ni$   &   40   &      0   &      0    &    58    &     0   &      0    &     0   &      0 & 3.52(-08) \nl
$\rm ^{57}Cu$   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 4.06(-18) \nl
$\rm ^{58}Cu$   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 2.34(-14) \nl
$\rm ^{59}Cu$   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 2.96(-10) \nl
$\rm ^{60}Cu$   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 3.99(-09) \nl
$\rm ^{61}Cu$   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 8.88(-07) \nl
$\rm ^{62}Cu$   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 9.79(-07) \nl
$\rm ^{63}Cu$   &   64   &      0   &      0    &     0    &     0   &      6    &     1   &     27 & 2.06(-05) \nl
$\rm ^{64}Cu$   &   99   &      0   &      0    &     0    &     0   &      0    &     0   &      0 & 1.19(-06) \nl
$\rm ^{65}Cu$   &   15   &      0   &      3    &    20    &     0   &     34    &     1   &     25 & 1.02(-05) \nl
$\rm ^{66}Cu$   &   74   &      0   &      0    &    24    &     0   &      0    &     0   &      0 & 2.39(-08) \nl
$\rm ^{64}Zn$   &    3   &      0   &      0    &     3    &     0   &     14    &     3   &     75 & 1.29(-05) \nl
$\rm ^{65}Zn$   &   23   &      0   &      1    &    22    &     0   &     53    &     0   &      0 & 6.02(-07) \nl
$\rm ^{66}Zn$   &    7   &      0   &      7    &    17    &     0   &     30    &     1   &     34 & 1.64(-05) \nl
$\rm ^{67}Zn$   &    1   &      0   &      0    &    23    &     0   &     40    &     1   &     32 & 2.60(-06) \nl
$\rm ^{68}Zn$   &    0   &      0   &     17    &    18    &     0   &     27    &     1   &     34 & 3.41(-05) \nl
\enddata        
\end{deluxetable}

==> tablsc11.tex <==
\begin{deluxetable}{lrrrrrrrrr}
%\small
\tablenum{11}
\tablewidth{16cm}
\tablecaption{Presupernova nucleosynthesis of the $\rm 15~M_\odot$ model} 
\tablehead{
\colhead{Isotope}     &
\colhead{Si}    &
\colhead{O}    &
\colhead{Ne}    &
\colhead{C}    &
\colhead{$\rm He_{\rm c}$}    &
\colhead{$\rm He_{\rm sh}$}    &
\colhead{$\rm H_{\rm sh}$}    &
\colhead{$\rm H_{\rm c}$}    &
\colhead{Yield ($\rm M_\odot$)}  
}
\startdata  
$\rm ^{1 }H $   &   0  &   0 &   0 &   0 &   0 &   0 &    0 &   99 & 6.77(+00) \nl
$\rm ^{2 }H $   &   0  &   0 &   0 &   0 &   0 &   0 &    0 &   99 & 1.84(-16) \nl
$\rm ^{3 }H $   &   0  &   0 &   0 &   0 &   0 &   0 &   99 &    0 & 3.17(-33) \nl
$\rm ^{3 }He$   &   0  &   0 &   0 &   0 &   0 &   0 &    0 &   99 & 2.18(-04) \nl
$\rm ^{4 }He$   &   0  &   0 &   0 &   0 &   0 &  18 &   13 &   68 & 5.26(+00) \nl
$\rm ^{6 }Li$   &   0  &   0 &   0 &   0 &   0 &   0 &    0 &   99 & 1.26(-17) \nl
$\rm ^{7 }Li$   &   0  &   0 &   0 &   0 &   0 &   0 &    0 &   99 & 1.53(-10) \nl
$\rm ^{7 }Be$   &   0  &   0 &   0 &   0 &   0 &   0 &  100 &    0 & 1.10(-19) \nl
$\rm ^{9 }Be$   &   0  &   0 &   0 &   0 &   0 &   0 &    0 &  100 & 5.03(-11) \nl
$\rm ^{10}Be$   &   0  &   0 &   0 &   0 &   0 &   0 &    0 &   99 & 6.53(-37) \nl
$\rm ^{10}B $   &   0  &   0 &   0 &   0 &   0 &   0 &    0 &  100 & 1.27(-09) \nl
$\rm ^{11}B $   &   0  &   0 &   0 &   0 &   0 &   0 &    0 &  100 & 1.51(-08) \nl
$\rm ^{12}C $   &   0  &   0 &   0 &   1 &  17 &  67 &    0 &   13 & 1.77(-01) \nl
$\rm ^{13}C $   &   0  &   0 &   0 &   0 &   0 &   0 &    0 &   99 & 2.49(-04) \nl
$\rm ^{14}C $   &   0  &   0 &   0 &   4 &   0 &  95 &    0 &    0 & 3.34(-07) \nl
$\rm ^{13}N $   &  81  &   2 &   0 &   0 &  15 &   0 &    0 &    0 & 7.59(-14) \nl
$\rm ^{14}N $   &   0  &   0 &   0 &   0 &   0 &   0 &   19 &   80 & 5.08(-02) \nl
$\rm ^{15}N $   &   0  &   0 &   0 &   0 &   0 &   1 &    1 &   97 & 1.98(-05) \nl
$\rm ^{16}N $   &  98  &   0 &   1 &   0 &   0 &   0 &    0 &    0 & 1.23(-20) \nl
$\rm ^{15}O $   &  35  &  62 &   0 &   1 &   0 &   0 &    0 &    0 & 1.06(-12) \nl
$\rm ^{16}O $   &   0  &   3 &  11 &  41 &  17 &  13 &    0 &   12 & 7.07(-01) \nl
$\rm ^{17}O $   &   0  &   0 &   0 &   0 &   0 &   0 &    1 &   98 & 1.03(-04) \nl
$\rm ^{18}O $   &   0  &   0 &   0 &   0 &   0 &  92 &    0 &    7 & 2.26(-03) \nl
$\rm ^{19}O $   &   0  &   0 &  78 &  21 &   0 &   0 &    0 &    0 & 1.33(-17) \nl
$\rm ^{17}F $   &  54  &  45 &   0 &   0 &   0 &   0 &    0 &    0 & 6.31(-14) \nl
$\rm ^{18}F $   &   0  &   0 &  29 &  70 &   0 &   0 &    0 &    0 & 3.64(-11) \nl
$\rm ^{19}F $   &   0  &   0 &   0 &   0 &   0 &  27 &    0 &   71 & 4.87(-06) \nl
$\rm ^{20}F $   &   0  &   0 &  77 &  22 &   0 &   0 &    0 &    0 & 4.49(-15) \nl
$\rm ^{20}Ne$   &   0  &   0 &   9 &  73 &   0 &   2 &    0 &   14 & 1.25(-01) \nl
$\rm ^{21}Ne$   &   0  &   0 &   4 &  76 &   3 &  10 &    0 &    4 & 8.67(-04) \nl
$\rm ^{22}Ne$   &   0  &   0 &   0 &   2 &   9 &  82 &    0 &    4 & 2.62(-02) \nl
$\rm ^{23}Ne$   &   0  &   0 &  67 &  32 &   0 &   0 &    0 &    0 & 1.28(-10) \nl
$\rm ^{21}Na$   &   2  &   0 &   7 &  89 &   0 &   0 &    0 &    0 & 5.29(-13) \nl
$\rm ^{22}Na$   &   0  &   0 &   4 &  95 &   0 &   0 &    0 &    0 & 6.04(-07) \nl
$\rm ^{23}Na$   &   0  &   0 &   6 &  75 &   0 &   4 &    2 &   11 & 5.60(-03) \nl
$\rm ^{24}Na$   &   0  &   0 &  80 &  19 &   0 &   0 &    0 &    0 & 3.70(-07) \nl
$\rm ^{23}Mg$   &   4  &  37 &  20 &  38 &   0 &   0 &    0 &    0 & 3.85(-10) \nl
$\rm ^{24}Mg$   &   0  &   2 &  26 &  46 &   0 &   2 &    1 &   20 & 2.72(-02) \nl
$\rm ^{25}Mg$   &   0  &   0 &  14 &  67 &   4 &   6 &    0 &    7 & 8.60(-03) \nl
$\rm ^{26}Mg$   &   0  &   0 &  14 &  48 &   7 &  11 &    1 &   16 & 6.01(-03) \nl
$\rm ^{27}Mg$   &   0  &   0 &  97 &   2 &   0 &   0 &    0 &    0 & 1.84(-08) \nl
$\rm ^{25}Al$   &  81  &  17 &   0 &   0 &   0 &   0 &    0 &    0 & 4.32(-12) \nl
$\rm ^{26}Al$   &   0  &   0 &   8 &   0 &   0 &   6 &   77 &    5 & 4.34(-06) \nl
$\rm ^{27}Al$   &   0  &   1 &  16 &  62 &   0 &   1 &    1 &   16 & 3.82(-03) \nl
$\rm ^{28}Al$   &   0  &   0 &  97 &   1 &   0 &   0 &    0 &    0 & 4.70(-07) \nl
$\rm ^{27}Si$   &   4  &  72 &  22 &   1 &   0 &   0 &    0 &    0 & 3.42(-09) \nl
$\rm ^{28}Si$   &   5  &  83 &   2 &   1 &   0 &   0 &    0 &    6 & 1.17(-01) \nl
$\rm ^{29}Si$   &   0  &  12 &  46 &  13 &   1 &   3 &    1 &   21 & 1.74(-03) \nl
$\rm ^{30}Si$   &   0  &  11 &  34 &  14 &   2 &   5 &    1 &   27 & 9.29(-04) \nl
$\rm ^{31}Si$   &   0  &   0 &  99 &   0 &   0 &   0 &    0 &    0 & 1.41(-06) \nl
$\rm ^{32}Si$   &   0  &   9 &  64 &  25 &   0 &   0 &    0 &    0 & 1.81(-07) \nl
$\rm ^{29}P $   &  39  &  60 &   0 &   0 &   0 &   0 &    0 &    0 & 4.60(-08) \nl
$\rm ^{30}P $   &  42  &  46 &  11 &   0 &   0 &   0 &    0 &    0 & 3.85(-07) \nl
$\rm ^{31}P $   &   2  &  28 &  18 &  17 &   2 &   6 &    1 &   22 & 3.90(-04) \nl
$\rm ^{32}P $   &   1  &   7 &  65 &  25 &   0 &   0 &    0 &    0 & 1.26(-06) \nl
$\rm ^{33}P $   &   0  &  18 &  70 &  10 &   0 &   0 &    0 &    0 & 9.34(-07) \nl
$\rm ^{34}P $   &   2  &   0 &  96 &   0 &   0 &   0 &    0 &    0 & 1.81(-11) \nl
$\rm ^{31}S $   &  42  &  56 &   0 &   0 &   0 &   0 &    0 &    0 & 2.21(-08) \nl
$\rm ^{32}S $   &   5  &  87 &   0 &   0 &   0 &   0 &    0 &    5 & 7.51(-02) \nl
$\rm ^{33}S $   &   5  &  69 &   2 &   1 &   0 &   3 &    1 &   15 & 2.26(-04) \nl
$\rm ^{34}S $   &   0  &  89 &   0 &   0 &   0 &   0 &    0 &    7 & 2.77(-03) \nl
$\rm ^{35}S $   &   0  &   2 &  43 &  49 &   0 &   3 &    0 &    0 & 1.67(-06) \nl
$\rm ^{36}S $   &   0  &   1 &  16 &  39 &   8 &  14 &    1 &   18 & 5.59(-06) \nl
$\rm ^{37}S $   &   3  &   0 &  22 &  73 &   0 &   0 &    0 &    0 & 1.25(-13) \nl
$\rm ^{33}Cl$   &  55  &  44 &   0 &   0 &   0 &   0 &    0 &    0 & 1.17(-08) \nl
$\rm ^{34}Cl$   &  63  &  36 &   0 &   0 &   0 &   0 &    0 &    0 & 1.51(-07) \nl
$\rm ^{35}Cl$   &   7  &  74 &   0 &   1 &   0 &   1 &    0 &   13 & 2.08(-04) \nl
$\rm ^{36}Cl$   &  11  &  24 &   8 &  24 &  10 &  20 &    0 &    0 & 6.10(-07) \nl
$\rm ^{37}Cl$   &   0  &   1 &   9 &  36 &  14 &  16 &    1 &   20 & 4.57(-05) \nl
$\rm ^{38}Cl$   &   0  &   0 &  92 &   7 &   0 &   0 &    0 &    0 & 2.62(-09) \nl
$\rm ^{36}Ar$   &   6  &  86 &   0 &   0 &   0 &   0 &    0 &    6 & 1.33(-02) \nl
$\rm ^{37}Ar$   &   9  &  88 &   0 &   0 &   0 &   1 &    0 &    0 & 5.21(-05) \nl
$\rm ^{38}Ar$   &   0  &  95 &   0 &   0 &   0 &   0 &    0 &    3 & 5.43(-03) \nl
$\rm ^{39}Ar$   &   0  &   0 &  14 &  60 &   1 &  22 &    0 &    0 & 2.64(-06) \nl
$\rm ^{40}Ar$   &   0  &   2 &  18 &  42 &   4 &  15 &    1 &   15 & 1.77(-06) \nl
$\rm ^{41}Ar$   &   0  &   0 &  96 &   3 &   0 &   0 &    0 &    0 & 4.84(-10) \nl
$\rm ^{37}K $   &  77  &  22 &   0 &   0 &   0 &   0 &    0 &    0 & 8.32(-10) \nl
$\rm ^{38}K $   &  71  &  28 &   0 &   0 &   0 &   0 &    0 &    0 & 7.91(-08) \nl
$\rm ^{39}K $   &   6  &  81 &   0 &   0 &   0 &   1 &    0 &    9 & 3.92(-04) \nl
$\rm ^{40}K $   &   6  &   4 &   7 &  36 &  13 &  23 &    0 &    7 & 7.96(-07) \nl
$\rm ^{41}K $   &   0  &   0 &   3 &  11 &   4 &  10 &    4 &   65 & 4.38(-06) \nl
$\rm ^{42}K $   &   0  &   0 &  94 &   3 &   0 &   0 &    0 &    0 & 6.21(-09) \nl
$\rm ^{40}Ca$   &   6  &  87 &   0 &   0 &   0 &   0 &    0 &    5 & 1.19(-02) \nl
$\rm ^{41}Ca$   &  14  &  77 &   0 &   1 &   0 &   5 &    0 &    0 & 1.91(-05) \nl
$\rm ^{42}Ca$   &   2  &  92 &   0 &   0 &   0 &   0 &    0 &    2 & 1.74(-04) \nl
$\rm ^{43}Ca$   &   2  &   2 &   5 &  22 &   7 &  11 &    3 &   44 & 2.22(-06) \nl
$\rm ^{44}Ca$   &   0  &   0 &   2 &   8 &   2 &   9 &    5 &   71 & 2.17(-05) \nl
$\rm ^{45}Ca$   &   0  &   3 &  40 &  42 &   0 &  12 &    0 &    0 & 2.17(-07) \nl
$\rm ^{46}Ca$   &   0  &   4 &  30 &  50 &   0 &   3 &    0 &   10 & 2.97(-07) \nl
$\rm ^{47}Ca$   &   0  &   8 &  88 &   3 &   0 &   0 &    0 &    0 & 4.22(-09) \nl
$\rm ^{48}Ca$   &   0  &   0 &   0 &   2 &   1 &   9 &    5 &   80 & 1.88(-06) \nl
$\rm ^{49}Ca$   &   0  &   0 &  62 &  37 &   0 &   0 &    0 &    0 & 1.82(-13) \nl
$\rm ^{41}Sc$   &  91  &   8 &   0 &   0 &   0 &   0 &    0 &    0 & 1.93(-10) \nl
$\rm ^{42}Sc$   &  96  &   3 &   0 &   0 &   0 &   0 &    0 &    0 & 1.47(-09) \nl
$\rm ^{43}Sc$   &  74  &  25 &   0 &   0 &   0 &   0 &    0 &    0 & 2.45(-07) \nl
$\rm ^{44}Sc$   &  89  &  10 &   0 &   0 &   0 &   0 &    0 &    0 & 3.77(-08) \nl
$\rm ^{45}Sc$   &  21  &   2 &   4 &  19 &   3 &   8 &    2 &   36 & 1.17(-06) \nl
$\rm ^{46}Sc$   &  66  &   0 &  30 &   1 &   0 &   0 &    0 &    0 & 2.26(-08) \nl
$\rm ^{47}Sc$   &  56  &   5 &  36 &   2 &   0 &   0 &    0 &    0 & 1.13(-08) \nl
$\rm ^{48}Sc$   &  74  &   6 &  19 &   0 &   0 &   0 &    0 &    0 & 1.93(-10) \nl
$\rm ^{49}Sc$   &  89  &   2 &   6 &   0 &   0 &   0 &    0 &    0 & 2.65(-11) \nl
$\rm ^{44}Ti$   &  36  &  63 &   0 &   0 &   0 &   0 &    0 &    0 & 4.32(-06) \nl
$\rm ^{45}Ti$   &  78  &  21 &   0 &   0 &   0 &   0 &    0 &    0 & 1.33(-06) \nl
$\rm ^{46}Ti$   &  47  &  50 &   0 &   0 &   0 &   0 &    0 &    1 & 1.34(-04) \nl
$\rm ^{47}Ti$   &  69  &   4 &   0 &   1 &   0 &   2 &    1 &   20 & 1.10(-05) \nl
$\rm ^{48}Ti$   &  35  &   0 &   0 &   0 &   0 &   5 &    3 &   53 & 4.37(-05) \nl
$\rm ^{49}Ti$   &  12  &   0 &   2 &  10 &   4 &  14 &    3 &   50 & 3.54(-06) \nl
$\rm ^{50}Ti$   &   5  &   0 &   7 &  24 &   6 &  11 &    2 &   41 & 4.31(-06) \nl
$\rm ^{51}Ti$   &  33  &   0 &  64 &   1 &   0 &   0 &    0 &    0 & 3.28(-10) \nl
$\rm ^{45}V $   &  98  &   1 &   0 &   0 &   0 &   0 &    0 &    0 & 1.62(-11) \nl
$\rm ^{46}V $   &  98  &   1 &   0 &   0 &   0 &   0 &    0 &    0 & 4.01(-09) \nl
$\rm ^{47}V $   &  98  &   1 &   0 &   0 &   0 &   0 &    0 &    0 & 5.94(-06) \nl
$\rm ^{48}V $   &  98  &   1 &   0 &   0 &   0 &   0 &    0 &    0 & 8.18(-06) \nl
$\rm ^{49}V $   &  99  &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 7.20(-05) \nl
$\rm ^{50}V $   &  99  &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 8.98(-06) \nl
$\rm ^{51}V $   &  74  &   0 &   0 &   0 &   0 &   2 &    1 &   20 & 1.97(-05) \nl
$\rm ^{52}V $   &  99  &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 3.95(-08) \nl
$\rm ^{48}Cr$   &  95  &   4 &   0 &   0 &   0 &   0 &    0 &    0 & 1.21(-05) \nl
$\rm ^{49}Cr$   &  98  &   1 &   0 &   0 &   0 &   0 &    0 &    0 & 5.22(-05) \nl
$\rm ^{50}Cr$   &  97  &   2 &   0 &   0 &   0 &   0 &    0 &    0 & 4.76(-03) \nl
$\rm ^{51}Cr$   &  99  &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 8.34(-04) \nl
$\rm ^{52}Cr$   &  95  &   0 &   0 &   0 &   0 &   0 &    0 &    3 & 4.71(-03) \nl
$\rm ^{53}Cr$   &  68  &   0 &   0 &   0 &   0 &   2 &    1 &   25 & 7.47(-05) \nl
$\rm ^{54}Cr$   &  21  &   0 &   5 &  21 &   7 &  11 &    2 &   29 & 1.60(-05) \nl
$\rm ^{55}Cr$   &  73  &   0 &  25 &   0 &   0 &   0 &    0 &    0 & 2.34(-09) \nl
$\rm ^{51}Mn$   &  99  &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 3.29(-04) \nl
$\rm ^{52}Mn$   &  99  &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 4.40(-04) \nl
$\rm ^{53}Mn$   &  99  &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 1.03(-02) \nl
$\rm ^{54}Mn$   &  99  &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 5.84(-04) \nl
$\rm ^{55}Mn$   &  52  &   0 &   0 &   0 &   0 &   4 &    2 &   39 & 3.64(-04) \nl
$\rm ^{56}Mn$   &  99  &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 3.41(-07) \nl
$\rm ^{57}Mn$   &  99  &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 2.49(-09) \nl
$\rm ^{52}Fe$   &  97  &   2 &   0 &   0 &   0 &   0 &    0 &    0 & 1.31(-04) \nl
$\rm ^{53}Fe$   &  99  &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 7.49(-04) \nl
$\rm ^{54}Fe$   &  98  &   1 &   0 &   0 &   0 &   0 &    0 &    0 & 1.87(-01) \nl
$\rm ^{55}Fe$   &  99  &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 2.17(-02) \nl
$\rm ^{56}Fe$   &  68  &   0 &   0 &   0 &   0 &   2 &    1 &   26 & 4.89(-02) \nl
$\rm ^{57}Fe$   &  38  &   0 &   1 &   6 &   3 &  11 &    2 &   36 & 8.67(-04) \nl
$\rm ^{58}Fe$   &   4  &   0 &   9 &  41 &  16 &  15 &    0 &    9 & 4.07(-04) \nl
$\rm ^{59}Fe$   &   3  &   0 &  84 &  12 &   0 &   0 &    0 &    0 & 5.98(-07) \nl
$\rm ^{60}Fe$   &   0  &   0 &   8 &  91 &   0 &   0 &    0 &    0 & 1.86(-06) \nl
$\rm ^{61}Fe$   &   0  &   0 &  76 &  23 &   0 &   0 &    0 &    0 & 4.16(-11) \nl
$\rm ^{55}Co$   &  99  &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 5.73(-03) \nl
$\rm ^{56}Co$   &  99  &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 3.09(-03) \nl
$\rm ^{57}Co$   &  99  &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 1.19(-02) \nl
$\rm ^{58}Co$   &  99  &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 5.54(-04) \nl
$\rm ^{59}Co$   &  48  &   0 &   4 &  20 &   6 &   6 &    0 &   12 & 2.93(-04) \nl
$\rm ^{60}Co$   &  49  &   0 &  46 &   3 &   0 &   0 &    0 &    0 & 1.46(-06) \nl
$\rm ^{61}Co$   &  35  &   0 &  64 &   0 &   0 &   0 &    0 &    0 & 4.70(-08) \nl
$\rm ^{56}Ni$   &  97  &   2 &   0 &   0 &   0 &   0 &    0 &    0 & 1.48(-03) \nl
$\rm ^{57}Ni$   &  99  &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 1.92(-03) \nl
$\rm ^{58}Ni$   &  97  &   0 &   0 &   0 &   0 &   0 &    0 &    1 & 3.14(-02) \nl
$\rm ^{59}Ni$   &  99  &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 3.85(-03) \nl
$\rm ^{60}Ni$   &  91  &   1 &   0 &   1 &   0 &   0 &    0 &    3 & 5.56(-03) \nl
$\rm ^{61}Ni$   &  67  &   0 &   3 &  13 &   3 &   5 &    0 &    5 & 1.67(-04) \nl
$\rm ^{62}Ni$   &  12  &   2 &  15 &  30 &   5 &  10 &    1 &   20 & 1.46(-04) \nl
$\rm ^{63}Ni$   &   0  &   0 &  15 &  69 &   0 &  13 &    0 &    0 & 4.98(-05) \nl
$\rm ^{64}Ni$   &   0  &   2 &  22 &  47 &   3 &  14 &    0 &    9 & 8.54(-05) \nl
$\rm ^{65}Ni$   &   0  &   0 &  92 &   7 &   0 &   0 &    0 &    0 & 7.79(-08) \nl
$\rm ^{57}Cu$   &  99  &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 5.15(-10) \nl
$\rm ^{58}Cu$   &  99  &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 6.80(-08) \nl
$\rm ^{59}Cu$   &  99  &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 1.36(-05) \nl
$\rm ^{60}Cu$   &  99  &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 1.40(-05) \nl
$\rm ^{61}Cu$   &  99  &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 8.90(-05) \nl
$\rm ^{62}Cu$   &  99  &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 1.07(-05) \nl
$\rm ^{63}Cu$   &  37  &   0 &   0 &   4 &  14 &   4 &    2 &   36 & 1.72(-05) \nl
$\rm ^{64}Cu$   &  92  &   0 &   5 &   1 &   0 &   1 &    0 &    0 & 1.04(-07) \nl
$\rm ^{65}Cu$   &   0  &   0 &   9 &  49 &   3 &  14 &    1 &   21 & 1.38(-05) \nl
$\rm ^{66}Cu$   &   0  &   0 &  95 &   4 &   0 &   0 &    0 &    0 & 1.32(-08) \nl
$\rm ^{64}Zn$   &  24  &   0 &   0 &   8 &   8 &   6 &    3 &   47 & 2.28(-05) \nl
$\rm ^{65}Zn$   &  18  &   0 &   3 &  37 &  25 &  15 &    0 &    0 & 1.39(-06) \nl
$\rm ^{66}Zn$   &   0  &   0 &  10 &  39 &   7 &  13 &    1 &   25 & 2.48(-05) \nl
$\rm ^{67}Zn$   &   0  &   0 &  10 &  45 &   7 &  14 &    1 &   20 & 4.73(-06) \nl
$\rm ^{68}Zn$   &   0  &   1 &  16 &  39 &   3 &  12 &    1 &   23 & 5.59(-05) \nl
\enddata           
\end{deluxetable}

==> tablsc12.tex <==
\begin{deluxetable}{lrrrrrrrrr}
%\small
\tablenum{12}
\tablewidth{16cm}
\tablecaption{Presupernova nucleosynthesis of the $\rm 20~M_\odot$ model} 
\tablehead{
\colhead{Isotope}     &
\colhead{Si}    &
\colhead{O}    &
\colhead{Ne}    &
\colhead{C}    &
\colhead{$\rm He_{\rm c}$}    &
\colhead{$\rm He_{\rm sh}$}    &
\colhead{$\rm H_{\rm sh}$}    &
\colhead{$\rm H_{\rm c}$}    &
\colhead{Yield ($\rm M_\odot$)}  
}
\startdata  
$\rm ^{1 }H $   &   0 &   0 &   0 &   0 &   0 &   0 &    0 &   99 & 8.34(+00) \nl
$\rm ^{2 }H $   &   0 &   0 &   0 &   0 &   0 &   0 &    0 &   99 & 2.02(-16) \nl
$\rm ^{3 }H $   &   0 &   0 &   0 &   0 &   0 &   0 &   98 &    1 & 3.61(-33) \nl
$\rm ^{3 }He$   &   0 &   0 &   0 &   0 &   0 &   0 &    0 &   99 & 2.32(-04) \nl
$\rm ^{4 }He$   &   0 &   0 &   0 &   0 &   0 &  23 &    6 &   70 & 7.18(+00) \nl
$\rm ^{6 }Li$   &   0 &   0 &   0 &   0 &   0 &   0 &    0 &   99 & 2.33(-17) \nl
$\rm ^{7 }Li$   &   0 &   0 &   0 &   0 &   0 &   0 &    0 &   99 & 1.31(-10) \nl
$\rm ^{7 }Be$   &   0 &   0 &   0 &   0 &   0 &   0 &  100 &    0 & 5.09(-17) \nl
$\rm ^{9 }Be$   &   0 &   0 &   0 &   0 &   0 &   0 &    0 &  100 & 5.75(-11) \nl
$\rm ^{10}Be$   &   0 &   0 &   0 &   0 &   0 &   0 &    0 &   99 & 1.19(-36) \nl
$\rm ^{10}B $   &   0 &   0 &   0 &   0 &   0 &   0 &    0 &  100 & 1.54(-09) \nl
$\rm ^{11}B $   &   0 &   0 &   0 &   0 &   0 &   0 &    0 &  100 & 1.87(-08) \nl
$\rm ^{12}C $   &   0 &   0 &   0 &  10 &  36 &  45 &    0 &    7 & 3.78(-01) \nl
$\rm ^{13}C $   &   0 &   0 &   0 &   0 &   0 &   0 &    0 &   99 & 3.05(-04) \nl
$\rm ^{14}C $   &   0 &   0 &   0 &  33 &   0 &  65 &    0 &    0 & 2.47(-07) \nl
$\rm ^{13}N $   &   1 &   0 &   0 &  21 &  77 &   0 &    0 &    0 & 9.47(-12) \nl
$\rm ^{14}N $   &   0 &   0 &   0 &   0 &   0 &   0 &    9 &   89 & 7.30(-02) \nl
$\rm ^{15}N $   &   0 &   0 &   0 &   0 &   0 &   1 &    0 &   97 & 2.49(-05) \nl
$\rm ^{16}N $   &  99 &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 1.24(-17) \nl
$\rm ^{15}O $   &   0 &  25 &   0 &  73 &   0 &   0 &    0 &    0 & 2.17(-11) \nl
$\rm ^{16}O $   &   0 &  10 &  11 &  24 &  42 &   5 &    0 &    6 & 1.52(+00) \nl
$\rm ^{17}O $   &   0 &   0 &   0 &   0 &   0 &   0 &    0 &   99 & 1.14(-04) \nl
$\rm ^{18}O $   &   0 &   0 &   0 &   0 &   0 &  82 &    0 &   17 & 1.02(-03) \nl
$\rm ^{19}O $   &   0 &   0 &  16 &  83 &   0 &   0 &    0 &    0 & 4.14(-16) \nl
$\rm ^{17}F $   &  11 &  88 &   0 &   0 &   0 &   0 &    0 &    0 & 2.18(-13) \nl
$\rm ^{18}F $   &   0 &   0 &   1 &  98 &   0 &   0 &    0 &    0 & 2.04(-09) \nl
$\rm ^{19}F $   &   0 &   0 &   0 &   0 &   0 &  46 &    0 &   52 & 6.84(-06) \nl
$\rm ^{20}F $   &   0 &   0 &   1 &  98 &   0 &   0 &    0 &    0 & 4.02(-12) \nl
$\rm ^{20}Ne$   &   0 &   0 &  24 &  48 &   2 &   2 &    0 &   20 & 1.11(-01) \nl
$\rm ^{21}Ne$   &   0 &   0 &  12 &  54 &  19 &  10 &    0 &    3 & 1.05(-03) \nl
$\rm ^{22}Ne$   &   0 &   0 &   0 &   5 &  19 &  71 &    0 &    2 & 5.37(-02) \nl
$\rm ^{23}Ne$   &   0 &   0 &   5 &  94 &   0 &   0 &    0 &    0 & 1.81(-08) \nl
$\rm ^{21}Na$   &   0 &   0 &   0 &  96 &   3 &   0 &    0 &    0 & 5.97(-11) \nl
$\rm ^{22}Na$   &   0 &   0 &   3 &  93 &   2 &   0 &    0 &    0 & 2.30(-06) \nl
$\rm ^{23}Na$   &   0 &   0 &  15 &  57 &   3 &   6 &    1 &   16 & 5.74(-03) \nl
$\rm ^{24}Na$   &   0 &   0 &  16 &  83 &   0 &   0 &    0 &    0 & 1.47(-05) \nl
$\rm ^{23}Mg$   &   0 &   0 &   4 &  94 &   0 &   0 &    0 &    0 & 5.28(-08) \nl
$\rm ^{24}Mg$   &   0 &  10 &  40 &  18 &   1 &   3 &    0 &   24 & 2.99(-02) \nl
$\rm ^{25}Mg$   &   0 &   0 &  21 &  37 &  31 &   3 &    0 &    6 & 1.12(-02) \nl
$\rm ^{26}Mg$   &   0 &   0 &  17 &  25 &  36 &   5 &    0 &   13 & 1.03(-02) \nl
$\rm ^{27}Mg$   &   0 &   0 &  64 &  35 &   0 &   0 &    0 &    0 & 1.43(-07) \nl
$\rm ^{25}Al$   &  31 &  18 &   0 &  30 &  18 &   0 &    0 &    0 & 5.79(-12) \nl
$\rm ^{26}Al$   &   0 &   0 &   8 &  16 &   0 &   3 &   21 &   48 & 2.28(-05) \nl
$\rm ^{27}Al$   &   0 &   2 &  32 &  40 &   1 &   2 &    0 &   20 & 4.00(-03) \nl
$\rm ^{28}Al$   &   0 &   0 &  77 &  22 &   0 &   0 &    0 &    0 & 4.42(-06) \nl
$\rm ^{27}Si$   &   0 &  40 &  42 &  17 &   0 &   0 &    0 &    0 & 3.13(-08) \nl
$\rm ^{28}Si$   &   1 &  91 &   1 &   0 &   0 &   0 &    0 &    3 & 2.42(-01) \nl
$\rm ^{29}Si$   &   0 &  25 &  44 &   4 &   4 &   3 &    0 &   17 & 2.85(-03) \nl
$\rm ^{30}Si$   &   0 &  19 &  34 &   8 &  11 &   4 &    0 &   21 & 1.57(-03) \nl
$\rm ^{31}Si$   &   0 &   0 &  80 &  18 &   0 &   0 &    0 &    0 & 1.08(-05) \nl
$\rm ^{32}Si$   &   0 &   3 &  83 &  11 &   0 &   0 &    0 &    0 & 4.34(-07) \nl
$\rm ^{29}P $   &  28 &  71 &   0 &   0 &   0 &   0 &    0 &    0 & 3.00(-08) \nl
$\rm ^{30}P $   &  15 &  56 &  26 &   1 &   0 &   0 &    0 &    0 & 9.16(-07) \nl
$\rm ^{31}P $   &   1 &  46 &  13 &   9 &  12 &   2 &    0 &   13 & 8.31(-04) \nl
$\rm ^{32}P $   &   4 &   8 &  64 &  22 &   0 &   0 &    0 &    0 & 4.76(-06) \nl
$\rm ^{33}P $   &   7 &  15 &  66 &  10 &   0 &   0 &    0 &    0 & 1.44(-06) \nl
$\rm ^{34}P $   &  76 &   0 &  23 &   0 &   0 &   0 &    0 &    0 & 7.07(-10) \nl
$\rm ^{31}S $   &   8 &  90 &   0 &   0 &   0 &   0 &    0 &    0 & 4.60(-08) \nl
$\rm ^{32}S $   &   1 &  94 &   0 &   0 &   0 &   0 &    0 &    3 & 1.52(-01) \nl
$\rm ^{33}S $   &   1 &  88 &   1 &   0 &   0 &   1 &    0 &    5 & 8.63(-04) \nl
$\rm ^{34}S $   &   0 &  95 &   0 &   0 &   0 &   0 &    0 &    3 & 8.75(-03) \nl
$\rm ^{35}S $   &   9 &   6 &  50 &  19 &   1 &  11 &    0 &    0 & 2.68(-06) \nl
$\rm ^{36}S $   &   0 &   1 &  18 &  27 &  36 &   4 &    0 &   10 & 1.23(-05) \nl
$\rm ^{37}S $   &  41 &   0 &   0 &  58 &   0 &   0 &    0 &    0 & 7.65(-11) \nl
$\rm ^{33}Cl$   &  38 &  61 &   0 &   0 &   0 &   0 &    0 &    0 & 6.25(-09) \nl
$\rm ^{34}Cl$   &  31 &  68 &   0 &   0 &   0 &   0 &    0 &    0 & 2.10(-07) \nl
$\rm ^{35}Cl$   &   3 &  88 &   0 &   0 &   0 &   0 &    0 &    6 & 5.91(-04) \nl
$\rm ^{36}Cl$   &  17 &  45 &   4 &   8 &  15 &   8 &    0 &    0 & 2.23(-06) \nl
$\rm ^{37}Cl$   &   0 &   1 &  10 &  24 &  41 &   8 &    0 &   12 & 1.00(-04) \nl
$\rm ^{38}Cl$   &   2 &   0 &  23 &  73 &   0 &   0 &    0 &    0 & 6.35(-08) \nl
$\rm ^{36}Ar$   &   1 &  93 &   0 &   0 &   0 &   0 &    0 &    4 & 2.57(-02) \nl
$\rm ^{37}Ar$   &   3 &  95 &   0 &   0 &   0 &   0 &    0 &    0 & 1.69(-04) \nl
$\rm ^{38}Ar$   &   0 &  96 &   0 &   0 &   0 &   0 &    0 &    1 & 1.15(-02) \nl
$\rm ^{39}Ar$   &   7 &   1 &  31 &  38 &   5 &  15 &    0 &    0 & 3.26(-06) \nl
$\rm ^{40}Ar$   &   2 &   2 &  26 &  26 &  25 &   4 &    0 &   12 & 2.96(-06) \nl
$\rm ^{41}Ar$   &   7 &   0 &  47 &  44 &   0 &   0 &    0 &    0 & 8.38(-09) \nl
$\rm ^{37}K $   &  58 &  41 &   0 &   0 &   0 &   0 &    0 &    0 & 3.16(-10) \nl
$\rm ^{38}K $   &  34 &  65 &   0 &   0 &   0 &   0 &    0 &    0 & 8.97(-08) \nl
$\rm ^{39}K $   &   2 &  90 &   0 &   0 &   0 &   0 &    0 &    5 & 9.33(-04) \nl
$\rm ^{40}K $   &  11 &   6 &   7 &  20 &  34 &  15 &    0 &    3 & 2.13(-06) \nl
$\rm ^{41}K $   &   2 &   0 &   4 &   9 &  16 &   9 &    2 &   54 & 6.78(-06) \nl
$\rm ^{42}K $   &   3 &   2 &  62 &  30 &   0 &   0 &    0 &    0 & 2.61(-07) \nl
$\rm ^{40}Ca$   &   1 &  93 &   0 &   0 &   0 &   0 &    0 &    4 & 1.85(-02) \nl
$\rm ^{41}Ca$   &   4 &  90 &   0 &   0 &   1 &   3 &    0 &    0 & 5.56(-05) \nl
$\rm ^{42}Ca$   &   1 &  94 &   0 &   0 &   0 &   0 &    0 &    1 & 3.87(-04) \nl
$\rm ^{43}Ca$   &  18 &   6 &   4 &  12 &  22 &   6 &    1 &   27 & 4.62(-06) \nl
$\rm ^{44}Ca$   &   6 &   0 &   3 &   7 &  10 &   8 &    2 &   59 & 3.37(-05) \nl
$\rm ^{45}Ca$   &  26 &   2 &  38 &  21 &   2 &   8 &    0 &    0 & 8.17(-07) \nl
$\rm ^{46}Ca$   &  27 &   5 &  39 &  13 &   0 &   2 &    0 &    9 & 4.24(-07) \nl
$\rm ^{47}Ca$   &  19 &   7 &  65 &   7 &   0 &   0 &    0 &    0 & 3.51(-08) \nl
$\rm ^{48}Ca$   &   0 &   0 &   1 &   2 &   4 &  11 &    2 &   78 & 2.51(-06) \nl
$\rm ^{49}Ca$   &  15 &   0 &   3 &  80 &   0 &   0 &    0 &    0 & 1.18(-11) \nl
$\rm ^{41}Sc$   &  82 &  17 &   0 &   0 &   0 &   0 &    0 &    0 & 5.93(-11) \nl
$\rm ^{42}Sc$   &  81 &  18 &   0 &   0 &   0 &   0 &    0 &    0 & 6.54(-10) \nl
$\rm ^{43}Sc$   &  35 &  64 &   0 &   0 &   0 &   0 &    0 &    0 & 4.16(-07) \nl
$\rm ^{44}Sc$   &  86 &  13 &   0 &   0 &   0 &   0 &    0 &    0 & 1.53(-07) \nl
$\rm ^{45}Sc$   &  63 &   2 &   0 &   4 &   9 &   2 &    0 &   15 & 3.53(-06) \nl
$\rm ^{46}Sc$   &  92 &   0 &   2 &   4 &   0 &   0 &    0 &    0 & 1.06(-06) \nl
$\rm ^{47}Sc$   &  97 &   0 &   1 &   0 &   0 &   0 &    0 &    0 & 1.75(-06) \nl
$\rm ^{48}Sc$   &  99 &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 3.88(-07) \nl
$\rm ^{49}Sc$   &  99 &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 2.48(-07) \nl
$\rm ^{44}Ti$   &   8 &  91 &   0 &   0 &   0 &   0 &    0 &    0 & 7.52(-06) \nl
$\rm ^{45}Ti$   &  49 &  50 &   0 &   0 &   0 &   0 &    0 &    0 & 1.68(-06) \nl
$\rm ^{46}Ti$   &  45 &  51 &   0 &   0 &   0 &   0 &    0 &    1 & 2.07(-04) \nl
$\rm ^{47}Ti$   &  88 &   2 &   0 &   0 &   0 &   0 &    0 &    6 & 4.52(-05) \nl
$\rm ^{48}Ti$   &  87 &   0 &   0 &   0 &   0 &   1 &    0 &   10 & 2.96(-04) \nl
$\rm ^{49}Ti$   &  92 &   0 &   0 &   0 &   1 &   1 &    0 &    3 & 6.12(-05) \nl
$\rm ^{50}Ti$   &  94 &   0 &   0 &   1 &   1 &   0 &    0 &    1 & 1.24(-04) \nl
$\rm ^{51}Ti$   &  99 &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 7.10(-07) \nl
$\rm ^{45}V $   &  94 &   5 &   0 &   0 &   0 &   0 &    0 &    0 & 1.91(-12) \nl
$\rm ^{46}V $   &  94 &   5 &   0 &   0 &   0 &   0 &    0 &    0 & 1.23(-09) \nl
$\rm ^{47}V $   &  91 &   8 &   0 &   0 &   0 &   0 &    0 &    0 & 4.16(-06) \nl
$\rm ^{48}V $   &  97 &   2 &   0 &   0 &   0 &   0 &    0 &    0 & 8.62(-06) \nl
$\rm ^{49}V $   &  99 &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 2.29(-04) \nl
$\rm ^{50}V $   &  99 &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 1.71(-04) \nl
$\rm ^{51}V $   &  99 &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 9.98(-04) \nl
$\rm ^{52}V $   &  99 &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 3.27(-05) \nl
$\rm ^{48}Cr$   &  84 &  15 &   0 &   0 &   0 &   0 &    0 &    0 & 5.31(-06) \nl
$\rm ^{49}Cr$   &  96 &   3 &   0 &   0 &   0 &   0 &    0 &    0 & 3.45(-05) \nl
$\rm ^{50}Cr$   &  96 &   3 &   0 &   0 &   0 &   0 &    0 &    0 & 5.77(-03) \nl
$\rm ^{51}Cr$   &  99 &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 1.91(-03) \nl
$\rm ^{52}Cr$   &  98 &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 2.47(-02) \nl
$\rm ^{53}Cr$   &  98 &   0 &   0 &   0 &   0 &   0 &    0 &    1 & 2.19(-03) \nl
$\rm ^{54}Cr$   &  97 &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 8.51(-04) \nl
$\rm ^{55}Cr$   &  99 &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 4.89(-06) \nl
$\rm ^{51}Mn$   &  99 &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 1.92(-04) \nl
$\rm ^{52}Mn$   &  99 &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 4.29(-04) \nl
$\rm ^{53}Mn$   &  99 &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 1.94(-02) \nl
$\rm ^{54}Mn$   &  99 &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 3.02(-03) \nl
$\rm ^{55}Mn$   &  96 &   0 &   0 &   0 &   0 &   0 &    0 &    3 & 5.67(-03) \nl
$\rm ^{56}Mn$   &  99 &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 9.87(-05) \nl
$\rm ^{57}Mn$   &  99 &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 3.71(-06) \nl
$\rm ^{52}Fe$   &  97 &   2 &   0 &   0 &   0 &   0 &    0 &    0 & 4.57(-05) \nl
$\rm ^{53}Fe$   &  99 &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 4.25(-04) \nl
$\rm ^{54}Fe$   &  96 &   3 &   0 &   0 &   0 &   0 &    0 &    0 & 1.72(-01) \nl
$\rm ^{55}Fe$   &  99 &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 3.39(-02) \nl
$\rm ^{56}Fe$   &  84 &   0 &   0 &   0 &   0 &   1 &    0 &   12 & 1.30(-01) \nl
$\rm ^{57}Fe$   &  88 &   0 &   0 &   0 &   1 &   2 &    0 &    5 & 6.82(-03) \nl
$\rm ^{58}Fe$   &  73 &   0 &   2 &   6 &  12 &   2 &    0 &    1 & 2.67(-03) \nl
$\rm ^{59}Fe$   &  64 &   0 &  10 &  24 &   0 &   0 &    0 &    0 & 3.52(-05) \nl
$\rm ^{60}Fe$   &  18 &   2 &  48 &  30 &   0 &   0 &    0 &    0 & 5.31(-06) \nl
$\rm ^{61}Fe$   &  32 &   0 &  14 &  53 &   0 &   0 &    0 &    0 & 3.08(-09) \nl
$\rm ^{55}Co$   &  98 &   1 &   0 &   0 &   0 &   0 &    0 &    0 & 3.06(-03) \nl
$\rm ^{56}Co$   &  99 &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 2.40(-03) \nl
$\rm ^{57}Co$   &  99 &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 1.63(-02) \nl
$\rm ^{58}Co$   &  99 &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 2.21(-03) \nl
$\rm ^{59}Co$   &  88 &   0 &   0 &   2 &   5 &   0 &    0 &    2 & 2.33(-03) \nl
$\rm ^{60}Co$   &  89 &   0 &   4 &   6 &   0 &   0 &    0 &    0 & 1.26(-04) \nl
$\rm ^{61}Co$   &  74 &   0 &  19 &   5 &   0 &   0 &    0 &    0 & 1.58(-05) \nl
$\rm ^{56}Ni$   &  97 &   2 &   0 &   0 &   0 &   0 &    0 &    0 & 4.16(-04) \nl
$\rm ^{57}Ni$   &  99 &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 9.02(-04) \nl
$\rm ^{58}Ni$   &  95 &   1 &   0 &   0 &   0 &   0 &    0 &    2 & 2.42(-02) \nl
$\rm ^{59}Ni$   &  99 &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 4.57(-03) \nl
$\rm ^{60}Ni$   &  92 &   3 &   0 &   0 &   0 &   0 &    0 &    2 & 1.33(-02) \nl
$\rm ^{61}Ni$   &  93 &   0 &   0 &   1 &   2 &   0 &    0 &    0 & 1.68(-03) \nl
$\rm ^{62}Ni$   &  75 &   3 &   3 &   5 &   7 &   0 &    0 &    3 & 1.19(-03) \nl
$\rm ^{63}Ni$   &  32 &   0 &  23 &  36 &   4 &   2 &    0 &    0 & 9.94(-05) \nl
$\rm ^{64}Ni$   &   1 &   3 &  32 &  29 &  25 &   1 &    0 &    5 & 1.78(-04) \nl
$\rm ^{65}Ni$   &   1 &   0 &  27 &  70 &   0 &   0 &    0 &    0 & 2.19(-06) \nl
$\rm ^{57}Cu$   &  99 &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 5.14(-11) \nl
$\rm ^{58}Cu$   &  99 &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 1.36(-08) \nl
$\rm ^{59}Cu$   &  99 &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 4.61(-06) \nl
$\rm ^{60}Cu$   &  99 &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 9.23(-06) \nl
$\rm ^{61}Cu$   &  99 &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 8.93(-05) \nl
$\rm ^{62}Cu$   &  99 &   0 &   0 &   0 &   0 &   0 &    0 &    0 & 2.75(-05) \nl
$\rm ^{63}Cu$   &  58 &   0 &   0 &   5 &  26 &   0 &    0 &    7 & 1.13(-04) \nl
$\rm ^{64}Cu$   &  83 &   0 &   1 &  13 &   1 &   0 &    0 &    0 & 9.91(-06) \nl
$\rm ^{65}Cu$   &   9 &   1 &   9 &  31 &  32 &   2 &    0 &   12 & 3.02(-05) \nl
$\rm ^{66}Cu$   &  37 &   0 &  24 &  38 &   0 &   0 &    0 &    0 & 2.42(-07) \nl
$\rm ^{64}Zn$   &  18 &   0 &   1 &  13 &  40 &   3 &    0 &   21 & 6.52(-05) \nl
$\rm ^{65}Zn$   &  26 &   0 &   2 &  21 &  46 &   2 &    0 &    0 & 1.07(-05) \nl
$\rm ^{66}Zn$   &   5 &   4 &  10 &  28 &  38 &   2 &    0 &   10 & 8.20(-05) \nl
$\rm ^{67}Zn$   &   1 &   0 &  12 &  33 &  42 &   2 &    0 &    7 & 1.57(-05) \nl
$\rm ^{68}Zn$   &   0 &   3 &  26 &  31 &  27 &   1 &    0 &    9 & 1.73(-04) \nl
\enddata           
\end{deluxetable}

==> tablsc13.tex <==
\begin{deluxetable}{lrrrrrrrrr}
%\small
\tablenum{13}
\tablewidth{16cm}
\tablecaption{Presupernova nucleosynthesis of the $\rm 25~M_\odot$ model} 
\tablehead{
\colhead{Isotope}     &
\colhead{Si}    &
\colhead{O}    &
\colhead{Ne}    &
\colhead{C}    &
\colhead{$\rm He_{\rm c}$}    &
\colhead{$\rm He_{\rm sh}$}    &
\colhead{$\rm H_{\rm sh}$}    &
\colhead{$\rm H_{\rm c}$}    &
\colhead{Yield ($\rm M_\odot$)}  
}
\startdata  
$\rm ^{1 }H $   &   0 &   0 &   0 &   0 &   0 &   0 &   0 &  99 & 9.82(+00)   \nl
$\rm ^{2 }H $   &   0 &   0 &   0 &   0 &   0 &   0 &   0 &  99 & 2.29(-16)   \nl
$\rm ^{3 }H $   &   0 &   0 &   0 &   0 &   0 &   0 &  93 &   6 & 3.98(-33)   \nl
$\rm ^{3 }He$   &   0 &   0 &   0 &   0 &   0 &   0 &   0 &  99 & 2.65(-04)   \nl
$\rm ^{4 }He$   &   0 &   0 &   0 &   0 &   0 &  23 &   5 &  70 & 8.99(+00)   \nl
$\rm ^{6 }Li$   &   0 &   0 &   0 &   0 &   0 &   0 &   0 &  99 & 3.67(-17)   \nl
$\rm ^{7 }Li$   &   0 &   0 &   0 &   0 &   0 &   0 &   0 &  99 & 9.27(-11)   \nl
$\rm ^{7 }Be$   &   0 &   0 &   0 &   0 &   0 &   0 & 100 &   0 & 2.08(-15)   \nl
$\rm ^{9 }Be$   &   0 &   0 &   0 &   0 &   0 &   0 &   0 &  99 & 6.36(-11)   \nl
$\rm ^{10}Be$   &   0 &   0 &   0 &   0 &   0 &   0 &   0 &  99 & 1.58(-36)   \nl
$\rm ^{10}B $   &   0 &   0 &   0 &   0 &   0 &   0 &   0 &  99 & 1.78(-09)   \nl
$\rm ^{11}B $   &   0 &   0 &   0 &   0 &   0 &   0 &   0 &  99 & 2.19(-08)   \nl
$\rm ^{12}C $   &   0 &   0 &   0 &   4 &  31 &  54 &   0 &   8 & 3.89(-01)   \nl
$\rm ^{13}C $   &   0 &   0 &   0 &   0 &   0 &   0 &   0 &  99 & 3.61(-04)   \nl
$\rm ^{14}C $   &   0 &   0 &   3 &  15 &   0 &  81 &   0 &   0 & 1.73(-07)   \nl
$\rm ^{13}N $   &  80 &  19 &   0 &   0 &   0 &   0 &   0 &   0 & 1.17(-13)   \nl
$\rm ^{14}N $   &   0 &   0 &   0 &   0 &   0 &   0 &   8 &  91 & 9.37(-02)   \nl
$\rm ^{15}N $   &   0 &   0 &   0 &   0 &   0 &   1 &   0 &  97 & 2.94(-05)   \nl
$\rm ^{16}N $   &   2 &   0 &  92 &   4 &   0 &   0 &   0 &   0 & 4.02(-22)   \nl
$\rm ^{15}O $   &   6 &  89 &   4 &   0 &   0 &   0 &   0 &   0 & 5.53(-12)   \nl
$\rm ^{16}O $   &   0 &   6 &  23 &  43 &  19 &   2 &   0 &   4 & 2.68(+00)   \nl
$\rm ^{17}O $   &   0 &   0 &   0 &   0 &   0 &   0 &   0 &  99 & 1.15(-04)   \nl
$\rm ^{18}O $   &   0 &   0 &   0 &   0 &   0 &  83 &   0 &  16 & 1.31(-03)   \nl
$\rm ^{19}O $   &   0 &   0 &  99 &   0 &   0 &   0 &   0 &   0 & 8.98(-18)   \nl
$\rm ^{17}F $   &  23 &  76 &   0 &   0 &   0 &   0 &   0 &   0 & 2.27(-13)   \nl
$\rm ^{18}F $   &   0 &   0 &  88 &  11 &   0 &   0 &   0 &   0 & 1.43(-10)   \nl
$\rm ^{19}F $   &   0 &   0 &   0 &   0 &   0 &  44 &   0 &  55 & 7.44(-06)   \nl
$\rm ^{20}F $   &   0 &   0 &  99 &   0 &   0 &   0 &   0 &   0 & 1.13(-13)   \nl
$\rm ^{20}Ne$   &   0 &   0 &  26 &  66 &   0 &   0 &   0 &   5 & 4.87(-01)   \nl
$\rm ^{21}Ne$   &   0 &   0 &  19 &  67 &   7 &   3 &   0 &   1 & 2.38(-03)   \nl
$\rm ^{22}Ne$   &   0 &   0 &   0 &   2 &  13 &  80 &   0 &   2 & 6.04(-02)   \nl
$\rm ^{23}Ne$   &   0 &   0 &  99 &   0 &   0 &   0 &   0 &   0 & 2.01(-10)   \nl
$\rm ^{21}Na$   &   0 &   1 &  63 &  34 &   0 &   0 &   0 &   0 & 1.75(-12)   \nl
$\rm ^{22}Na$   &   0 &   0 &  18 &  81 &   0 &   0 &   0 &   0 & 7.15(-06)   \nl
$\rm ^{23}Na$   &   0 &   0 &  21 &  69 &   0 &   2 &   0 &   5 & 1.97(-02)   \nl
$\rm ^{24}Na$   &   0 &   0 &  78 &  21 &   0 &   0 &   0 &   0 & 5.61(-06)   \nl
$\rm ^{23}Mg$   &   0 &   1 &  98 &   0 &   0 &   0 &   0 &   0 & 2.97(-08)   \nl
$\rm ^{24}Mg$   &   0 &  11 &  36 &  41 &   0 &   1 &   0 &   8 & 1.05(-01)   \nl
$\rm ^{25}Mg$   &   0 &   0 &  27 &  58 &  10 &   1 &   0 &   2 & 3.21(-02)   \nl
$\rm ^{26}Mg$   &   0 &   1 &  26 &  49 &  13 &   2 &   0 &   6 & 2.60(-02)   \nl
$\rm ^{27}Mg$   &   0 &   1 &  98 &   0 &   0 &   0 &   0 &   0 & 4.81(-07)   \nl
$\rm ^{25}Al$   &  69 &  29 &   0 &   0 &   0 &   0 &   0 &   0 & 4.40(-11)   \nl
$\rm ^{26}Al$   &   0 &   0 &  25 &   0 &   0 &   1 &  14 &  58 & 3.98(-05)   \nl
$\rm ^{27}Al$   &   0 &   3 &  31 &  58 &   0 &   0 &   0 &   5 & 1.80(-02)   \nl
$\rm ^{28}Al$   &   0 &   7 &  92 &   0 &   0 &   0 &   0 &   0 & 2.69(-05)   \nl
$\rm ^{27}Si$   &   0 &   3 &  96 &   0 &   0 &   0 &   0 &   0 & 1.89(-07)   \nl
$\rm ^{28}Si$   &  12 &  75 &   4 &   2 &   0 &   0 &   0 &   4 & 2.50(-01)   \nl
$\rm ^{29}Si$   &   0 &  30 &  42 &  15 &   1 &   1 &   0 &   7 & 7.46(-03)   \nl
$\rm ^{30}Si$   &   0 &  35 &  34 &  15 &   3 &   1 &   0 &   9 & 4.34(-03)   \nl
$\rm ^{31}Si$   &   0 &   0 &  98 &   0 &   0 &   0 &   0 &   0 & 2.48(-05)   \nl
$\rm ^{32}Si$   &   0 &  12 &  60 &  27 &   0 &   0 &   0 &   0 & 1.33(-06)   \nl
$\rm ^{29}P $   &  57 &  42 &   0 &   0 &   0 &   0 &   0 &   0 & 4.69(-07)   \nl
$\rm ^{30}P $   &  32 &  40 &  26 &   0 &   0 &   0 &   0 &   0 & 2.54(-06)   \nl
$\rm ^{31}P $   &   1 &  36 &  22 &  23 &   5 &   1 &   0 &   8 & 1.65(-03)   \nl
$\rm ^{32}P $   &   0 &  19 &  45 &  35 &   0 &   0 &   0 &   0 & 1.95(-05)   \nl
$\rm ^{33}P $   &   0 &  36 &  43 &  20 &   0 &   0 &   0 &   0 & 5.39(-06)   \nl
$\rm ^{34}P $   &   0 &   2 &  97 &   0 &   0 &   0 &   0 &   0 & 7.24(-10)   \nl
$\rm ^{31}S $   &  36 &  62 &   1 &   0 &   0 &   0 &   0 &   0 & 2.74(-07)   \nl
$\rm ^{32}S $   &   9 &  82 &   0 &   0 &   0 &   0 &   0 &   5 & 1.22(-01)   \nl
$\rm ^{33}S $   &   3 &  78 &   3 &   1 &   0 &   2 &   0 &   8 & 6.33(-04)   \nl
$\rm ^{34}S $   &   0 &  91 &   1 &   0 &   0 &   0 &   0 &   5 & 6.38(-03)   \nl
$\rm ^{35}S $   &   0 &   1 &  46 &  49 &   0 &   1 &   0 &   0 & 8.58(-06)   \nl
$\rm ^{36}S $   &   0 &   5 &  27 &  45 &  14 &   1 &   0 &   5 & 2.98(-05)   \nl
$\rm ^{37}S $   &   0 &   0 &  98 &   0 &   0 &   0 &   0 &   0 & 4.03(-13)   \nl
$\rm ^{33}Cl$   &  59 &  40 &   0 &   0 &   0 &   0 &   0 &   0 & 7.85(-08)   \nl
$\rm ^{34}Cl$   &  48 &  51 &   0 &   0 &   0 &   0 &   0 &   0 & 5.19(-07)   \nl
$\rm ^{35}Cl$   &   5 &  80 &   1 &   1 &   0 &   1 &   0 &   8 & 5.17(-04)   \nl
$\rm ^{36}Cl$   &   1 &  42 &  15 &  21 &  11 &   7 &   0 &   0 & 2.69(-06)   \nl
$\rm ^{37}Cl$   &   0 &   3 &  21 &  42 &  20 &   4 &   0 &   8 & 1.77(-04)   \nl
$\rm ^{38}Cl$   &   0 &   0 &  99 &   0 &   0 &   0 &   0 &   0 & 2.74(-08)   \nl
$\rm ^{36}Ar$   &   8 &  83 &   0 &   0 &   0 &   0 &   0 &   6 & 1.96(-02)   \nl
$\rm ^{37}Ar$   &   6 &  91 &   0 &   0 &   0 &   1 &   0 &   0 & 1.06(-04)   \nl
$\rm ^{38}Ar$   &   0 &  92 &   0 &   1 &   0 &   0 &   0 &   3 & 7.01(-03)   \nl
$\rm ^{39}Ar$   &   0 &   0 &  32 &  62 &   1 &   3 &   0 &   0 & 1.17(-05)   \nl
$\rm ^{40}Ar$   &   0 &   5 &  31 &  47 &   8 &   1 &   0 &   4 & 8.75(-06)   \nl
$\rm ^{41}Ar$   &   0 &   0 &  98 &   1 &   0 &   0 &   0 &   0 & 1.14(-08)   \nl
$\rm ^{37}K $   &  63 &  36 &   0 &   0 &   0 &   0 &   0 &   0 & 2.77(-09)   \nl
$\rm ^{38}K $   &  47 &  52 &   0 &   0 &   0 &   0 &   0 &   0 & 1.70(-07)   \nl
$\rm ^{39}K $   &   3 &  84 &   0 &   1 &   0 &   1 &   0 &   7 & 7.65(-04)   \nl
$\rm ^{40}K $   &   0 &   3 &  20 &  43 &  19 &  10 &   0 &   2 & 3.42(-06)   \nl
$\rm ^{41}K $   &   0 &   2 &  11 &  22 &   9 &   7 &   1 &  44 & 1.01(-05)   \nl
$\rm ^{42}K $   &   0 &   1 &  86 &  12 &   0 &   0 &   0 &   0 & 4.52(-07)   \nl
$\rm ^{40}Ca$   &   6 &  84 &   0 &   0 &   0 &   1 &   0 &   7 & 1.40(-02)   \nl
$\rm ^{41}Ca$   &   6 &  82 &   1 &   2 &   1 &   6 &   0 &   0 & 3.46(-05)   \nl
$\rm ^{42}Ca$   &   1 &  91 &   1 &   2 &   1 &   0 &   0 &   2 & 2.59(-04)   \nl
$\rm ^{43}Ca$   &   0 &   4 &  15 &  32 &  14 &   5 &   0 &  26 & 5.83(-06)   \nl
$\rm ^{44}Ca$   &   0 &   1 &  10 &  19 &   6 &   7 &   1 &  51 & 4.72(-05)   \nl
$\rm ^{45}Ca$   &   0 &   2 &  42 &  52 &   0 &   1 &   0 &   0 & 2.56(-06)   \nl
$\rm ^{46}Ca$   &   0 &  12 &  38 &  45 &   0 &   0 &   0 &   2 & 1.70(-06)   \nl
$\rm ^{47}Ca$   &   0 &   5 &  69 &  24 &   0 &   0 &   0 &   0 & 9.95(-08)   \nl
$\rm ^{48}Ca$   &   0 &   0 &   2 &   5 &   2 &  10 &   2 &  74 & 3.18(-06)   \nl
$\rm ^{49}Ca$   &   0 &   0 &  99 &   0 &   0 &   0 &   0 &   0 & 5.89(-13)   \nl
$\rm ^{41}Sc$   &  68 &  31 &   0 &   0 &   0 &   0 &   0 &   0 & 2.36(-10)   \nl
$\rm ^{42}Sc$   &  70 &  29 &   0 &   0 &   0 &   0 &   0 &   0 & 6.95(-10)   \nl
$\rm ^{43}Sc$   &  25 &  74 &   0 &   0 &   0 &   0 &   0 &   0 & 3.13(-07)   \nl
$\rm ^{44}Sc$   &  27 &  70 &   1 &   0 &   0 &   0 &   0 &   0 & 2.09(-08)   \nl
$\rm ^{45}Sc$   &   2 &   5 &   9 &  26 &  14 &   7 &   1 &  33 & 2.01(-06)   \nl
$\rm ^{46}Sc$   &   0 &  14 &  50 &  34 &   0 &   0 &   0 &   0 & 1.64(-07)   \nl
$\rm ^{47}Sc$   &   0 &  24 &  52 &  22 &   0 &   0 &   0 &   0 & 1.59(-07)   \nl
$\rm ^{48}Sc$   &   0 &  18 &  81 &   0 &   0 &   0 &   0 &   0 & 1.29(-08)   \nl
$\rm ^{49}Sc$   &   0 &  14 &  85 &   0 &   0 &   0 &   0 &   0 & 9.71(-10)   \nl
$\rm ^{44}Ti$   &  18 &  81 &   0 &   0 &   0 &   0 &   0 &   0 & 7.57(-06)   \nl
$\rm ^{45}Ti$   &  38 &  61 &   0 &   0 &   0 &   0 &   0 &   0 & 1.16(-06)   \nl
$\rm ^{46}Ti$   &  33 &  60 &   0 &   1 &   0 &   0 &   0 &   2 & 1.36(-04)   \nl
$\rm ^{47}Ti$   &  24 &  10 &   4 &  10 &   3 &   5 &   1 &  40 & 8.84(-06)   \nl
$\rm ^{48}Ti$   &   8 &   1 &   1 &   3 &   1 &   9 &   2 &  72 & 5.08(-05)   \nl
$\rm ^{49}Ti$   &   0 &   1 &  14 &  26 &   8 &  12 &   1 &  35 & 7.96(-06)   \nl
$\rm ^{50}Ti$   &   0 &   4 &  21 &  38 &  11 &   4 &   0 &  18 & 1.49(-05)   \nl
$\rm ^{51}Ti$   &   0 &   0 &  99 &   0 &   0 &   0 &   0 &   0 & 8.31(-09)   \nl
$\rm ^{45}V $   &  79 &  20 &   0 &   0 &   0 &   0 &   0 &   0 & 3.90(-12)   \nl
$\rm ^{46}V $   &  82 &  17 &   0 &   0 &   0 &   0 &   0 &   0 & 9.38(-10)   \nl
$\rm ^{47}V $   &  84 &  15 &   0 &   0 &   0 &   0 &   0 &   0 & 3.01(-06)   \nl
$\rm ^{48}V $   &  91 &   8 &   0 &   0 &   0 &   0 &   0 &   0 & 2.56(-06)   \nl
$\rm ^{49}V $   &  97 &   1 &   0 &   0 &   0 &   0 &   0 &   0 & 2.36(-05)   \nl
$\rm ^{50}V $   &  95 &   1 &   0 &   0 &   0 &   0 &   0 &   1 & 1.05(-06)   \nl
$\rm ^{51}V $   &  12 &   0 &   2 &   5 &   1 &   9 &   2 &  65 & 9.93(-06)   \nl
$\rm ^{52}V $   &   4 &   1 &  94 &   0 &   0 &   0 &   0 &   0 & 1.07(-08)   \nl
$\rm ^{48}Cr$   &  71 &  28 &   0 &   0 &   0 &   0 &   0 &   0 & 1.13(-05)   \nl
$\rm ^{49}Cr$   &  89 &  10 &   0 &   0 &   0 &   0 &   0 &   0 & 2.81(-05)   \nl
$\rm ^{50}Cr$   &  90 &   8 &   0 &   0 &   0 &   0 &   0 &   0 & 3.43(-03)   \nl
$\rm ^{51}Cr$   &  97 &   2 &   0 &   0 &   0 &   0 &   0 &   0 & 3.51(-04)   \nl
$\rm ^{52}Cr$   &  85 &   2 &   0 &   0 &   0 &   1 &   0 &   9 & 2.57(-03)   \nl
$\rm ^{53}Cr$   &  12 &   0 &   0 &   2 &   1 &  11 &   2 &  69 & 4.23(-05)   \nl
$\rm ^{54}Cr$   &   0 &   2 &  17 &  34 &  15 &   7 &   0 &  21 & 3.49(-05)   \nl
$\rm ^{55}Cr$   &   0 &   0 &  99 &   0 &   0 &   0 &   0 &   0 & 1.12(-08)   \nl
$\rm ^{51}Mn$   &  90 &   9 &   0 &   0 &   0 &   0 &   0 &   0 & 1.65(-04)   \nl
$\rm ^{52}Mn$   &  97 &   2 &   0 &   0 &   0 &   0 &   0 &   0 & 1.66(-04)   \nl
$\rm ^{53}Mn$   &  97 &   2 &   0 &   0 &   0 &   0 &   0 &   0 & 5.00(-03)   \nl
$\rm ^{54}Mn$   &  99 &   0 &   0 &   0 &   0 &   0 &   0 &   0 & 1.02(-04)   \nl
$\rm ^{55}Mn$   &   5 &   0 &   0 &   0 &   0 &  10 &   2 &  78 & 2.91(-04)   \nl
$\rm ^{56}Mn$   &  15 &   0 &  83 &   0 &   0 &   0 &   0 &   0 & 2.72(-08)   \nl
$\rm ^{57}Mn$   &   1 &   0 &  97 &   0 &   0 &   0 &   0 &   0 & 5.40(-10)   \nl
$\rm ^{52}Fe$   &  74 &  25 &   0 &   0 &   0 &   0 &   0 &   0 & 9.07(-05)   \nl
$\rm ^{53}Fe$   &  90 &   9 &   0 &   0 &   0 &   0 &   0 &   0 & 3.45(-04)   \nl
$\rm ^{54}Fe$   &  88 &  10 &   0 &   0 &   0 &   0 &   0 &   1 & 1.05(-01)   \nl
$\rm ^{55}Fe$   &  97 &   2 &   0 &   0 &   0 &   0 &   0 &   0 & 9.64(-03)   \nl
$\rm ^{56}Fe$   &  34 &   1 &   0 &   0 &   0 &   7 &   1 &  54 & 3.71(-02)   \nl
$\rm ^{57}Fe$   &   3 &   0 &   3 &   9 &   7 &  22 &   1 &  52 & 9.37(-04)   \nl
$\rm ^{58}Fe$   &   0 &   3 &  20 &  40 &  23 &   6 &   0 &   5 & 1.13(-03)   \nl
$\rm ^{59}Fe$   &   0 &   0 &  58 &  41 &   0 &   0 &   0 &   0 & 1.55(-05)   \nl
$\rm ^{60}Fe$   &   0 &   2 &  53 &  43 &   0 &   0 &   0 &   0 & 1.55(-05)   \nl
$\rm ^{61}Fe$   &   0 &   0 &  99 &   0 &   0 &   0 &   0 &   0 & 1.06(-09)   \nl
$\rm ^{55}Co$   &  89 &  10 &   0 &   0 &   0 &   0 &   0 &   0 & 2.60(-03)   \nl
$\rm ^{56}Co$   &  98 &   1 &   0 &   0 &   0 &   0 &   0 &   0 & 1.01(-03)   \nl
$\rm ^{57}Co$   &  98 &   1 &   0 &   0 &   0 &   0 &   0 &   0 & 4.01(-03)   \nl
$\rm ^{58}Co$   &  99 &   0 &   0 &   0 &   0 &   0 &   0 &   0 & 6.08(-05)   \nl
$\rm ^{59}Co$   &   2 &   1 &  15 &  41 &  21 &   3 &   0 &  13 & 4.39(-04)   \nl
$\rm ^{60}Co$   &   0 &   0 &  67 &  32 &   0 &   0 &   0 &   0 & 1.90(-05)   \nl
$\rm ^{61}Co$   &   0 &   2 &  97 &   0 &   0 &   0 &   0 &   0 & 1.02(-05)   \nl
$\rm ^{56}Ni$   &  72 &  27 &   0 &   0 &   0 &   0 &   0 &   0 & 7.85(-04)   \nl
$\rm ^{57}Ni$   &  92 &   7 &   0 &   0 &   0 &   0 &   0 &   0 & 6.63(-04)   \nl
$\rm ^{58}Ni$   &  87 &   4 &   0 &   0 &   0 &   0 &   0 &   6 & 1.34(-02)   \nl
$\rm ^{59}Ni$   &  97 &   0 &   0 &   0 &   0 &   1 &   0 &   0 & 8.80(-04)   \nl
$\rm ^{60}Ni$   &  50 &   9 &   4 &  11 &   5 &   2 &   0 &  15 & 2.15(-03)   \nl
$\rm ^{61}Ni$   &   2 &   0 &  20 &  46 &  19 &   3 &   0 &   6 & 2.13(-04)   \nl
$\rm ^{62}Ni$   &   0 &  17 &  22 &  36 &  13 &   1 &   0 &   7 & 6.45(-04)   \nl
$\rm ^{63}Ni$   &   0 &   0 &  31 &  66 &   1 &   0 &   0 &   0 & 3.00(-04)   \nl
$\rm ^{64}Ni$   &   0 &   7 &  33 &  48 &   8 &   0 &   0 &   2 & 6.00(-04)   \nl
$\rm ^{65}Ni$   &   0 &   0 &  94 &   5 &   0 &   0 &   0 &   0 & 1.44(-06)   \nl
$\rm ^{57}Cu$   &  93 &   6 &   0 &   0 &   0 &   0 &   0 &   0 & 4.11(-11)   \nl
$\rm ^{58}Cu$   &  97 &   2 &   0 &   0 &   0 &   0 &   0 &   0 & 6.39(-09)   \nl
$\rm ^{59}Cu$   &  98 &   1 &   0 &   0 &   0 &   0 &   0 &   0 & 2.12(-06)   \nl
$\rm ^{60}Cu$   &  99 &   0 &   0 &   0 &   0 &   0 &   0 &   0 & 1.33(-06)   \nl
$\rm ^{61}Cu$   &  99 &   0 &   0 &   0 &   0 &   0 &   0 &   0 & 1.00(-05)   \nl
$\rm ^{62}Cu$   &  99 &   0 &   0 &   0 &   0 &   0 &   0 &   0 & 4.26(-07)   \nl
$\rm ^{63}Cu$   &   0 &   0 &   4 &  16 &  56 &   2 &   0 &  19 & 5.10(-05)   \nl
$\rm ^{64}Cu$   &   0 &   0 &  42 &  55 &   1 &   0 &   0 &   0 & 1.09(-06)   \nl
$\rm ^{65}Cu$   &   0 &   1 &  21 &  59 &  11 &   0 &   0 &   4 & 9.35(-05)   \nl
$\rm ^{66}Cu$   &   0 &   0 &  99 &   0 &   0 &   0 &   0 &   0 & 3.61(-07)   \nl
$\rm ^{64}Zn$   &   0 &   0 &   7 &  26 &  37 &   3 &   0 &  23 & 7.12(-05)   \nl
$\rm ^{65}Zn$   &   0 &   0 &  13 &  43 &  40 &   2 &   0 &   0 & 1.24(-05)   \nl
$\rm ^{66}Zn$   &   0 &   7 &  21 &  49 &  16 &   0 &   0 &   4 & 2.07(-04)   \nl
$\rm ^{67}Zn$   &   0 &   0 &  23 &  55 &  17 &   0 &   0 &   3 & 4.24(-05)   \nl
$\rm ^{68}Zn$   &   0 &   6 &  30 &  51 &   8 &   0 &   0 &   2 & 6.91(-04)   \nl
\enddata           
\end{deluxetable}

==> tablsc14.tex <==
\begin{deluxetable}{lrrrrr}
%\small
\tablenum{14}
\tablewidth{10cm}
\tablecaption{Comparison of the last C convective shell extension among NH88, WW95, APB96 and the present computations.}
\tablehead{
\colhead{Initial Mass}     &
\colhead{NH88}    &
\colhead{WW95}    &
\colhead{APB96}   &
\colhead{LCS}       
}
\startdata  
13   &  1.44-1.70       &  \nodata         &  \nodata           & 1.52-1.75    \nl
15   &  1.50-2.00       &  2.00-2.30       &  \nodata           & 1.64-2.18    \nl
20   &  1.67-3.70       &  \nodata         &  1.40-3.80         & 2.39-2.77    \nl
25   &  1.79-5.40       &  3.70-5.60       &  \nodata           & 2.28-4.61    \nl
\enddata        
\end{deluxetable}


==> tablsc15.tex <==
\begin{deluxetable}{lrrrl}
%\small
\tablenum{15}
\tablewidth{12cm}
\tablecaption{Nucleosynthesis after central Ne exhaustion for isotopes lighter than A=27 in the
$\rm 20~M_\odot$ model} 
\tablehead{
\colhead{Isotope}     &
\colhead{Ne exh. (A)}    &
\colhead{Last Model (B)}    &
\colhead{(A-B)/A}    &
\colhead{Burning Site}   
}
\startdata  
$\rm ^{1 }H $   & 8.34E+00 & 8.34E+00 &   0.0000 &    \nl
$\rm ^{2 }H $   & 2.02E-16 & 2.02E-16 &   0.0000 &    \nl
$\rm ^{3 }He$   & 2.32E-04 & 2.32E-04 &   0.0000 &    \nl
$\rm ^{4 }He$   & 7.19E+00 & 7.18E+00 &   0.0014 &    \nl
$\rm ^{6 }Li$   & 2.33E-17 & 2.33E-17 &   0.0000 &    \nl
$\rm ^{7 }Li$   & 1.31E-10 & 1.31E-10 &   0.0000 &    \nl
$\rm ^{9 }Be$   & 5.75E-11 & 5.75E-11 &   0.0000 &    \nl
$\rm ^{10}B $   & 1.54E-09 & 1.54E-09 &   0.0000 &    \nl
$\rm ^{11}B $   & 1.87E-08 & 1.87E-08 &   0.0000 &    \nl
$\rm ^{12}C $   & 3.91E-01 & 3.78E-01 &   0.0332 &    \nl
$\rm ^{13}C $   & 3.04E-04 & 3.05E-04 &  -0.0033 &    \nl
$\rm ^{14}N $   & 7.41E-02 & 7.30E-02 &   0.0148 &    \nl
$\rm ^{15}N $   & 2.47E-05 & 2.49E-05 &  -0.0081 &    \nl
$\rm ^{16}O $   & 1.57E+00 & 1.48E+00 &   0.0573 &    \nl
$\rm ^{17}O $   & 1.14E-04 & 1.14E-04 &   0.0000 &    \nl
$\rm ^{18}O $   & 4.61E-03 & 1.02E-03 &   0.7787 & d(He shell)   \nl
$\rm ^{19}F $   & 5.35E-06 & 6.84E-06 &  -0.2785 & p(He shell)   \nl
$\rm ^{20}Ne$   & 1.74E-01 & 1.11E-01 &   0.3621 & d(Ne shell)   \nl
$\rm ^{21}Ne$   & 1.71E-03 & 1.05E-03 &   0.3860 & d(Ne shell)  \nl
$\rm ^{22}Ne$   & 5.03E-02 & 5.37E-02 &  -0.0676 & p(He shell)   \nl
$\rm ^{23}Na$   & 9.66E-03 & 5.74E-03 &   0.4058 & d(Ne shell)   \nl
$\rm ^{24}Mg$   & 2.32E-02 & 2.96E-02 &  -0.2759 & p(Ne shell)   \nl
$\rm ^{25}Mg$   & 1.36E-02 & 1.12E-02 &   0.1765 & d(Ne shell)   \nl
$\rm ^{26}Mg$   & 1.13E-02 & 1.03E-02 &   0.0885 & d(O shell)   \nl
$\rm ^{27}Al$   & 4.99E-03 & 4.00E-03 &   0.1984 & d(Ne shell)   \nl
\enddata           
\end{deluxetable}

==> tablsc16.tex <==
\begin{deluxetable}{lrrrrr}
%\small
\tablenum{A1}
%\tablewidth{16cm}
\tablecaption{Explosive nucleosynthesis of the $\rm 13~M_\odot~~Z=2\cdot10^{-2}$ model}
\tablehead{
\colhead{}        & \colhead{(1)} & \colhead{(2)} & \colhead{(3)} & \colhead{(4)} & \colhead{(5)}
}
\startdata  
$\rm M(^{56}Ni)$  &    0.001  &      0.005  &      0.010  &      0.050  &      0.060  \nl
$\rm M_{ejected}$ &     11.41 &       11.42 &       11.43 &       11.50 &       11.51 \nl
$\rm M_{cut}$     &      1.59 &        1.58 &        1.57 &        1.50 &        1.49 \nl
C                 &  1.37(-01)&   1.37(-01) &   1.37(-01) &   1.37(-01) &   1.37(-01) \nl
N                 &  3.97(-02)&   3.97(-02) &   3.97(-02) &   3.97(-02) &   3.97(-02) \nl
O                 &  2.66(-01)&   2.66(-01) &   2.66(-01) &   2.66(-01) &   2.66(-01) \nl
F                 &  6.75(-06)&   6.75(-06) &   6.75(-06) &   6.75(-06) &   6.75(-06) \nl
Ne                &  5.15(-02)&   5.15(-02) &   5.15(-02) &   5.15(-02) &   5.15(-02) \nl
Na                &  1.05(-03)&   1.05(-03) &   1.05(-03) &   1.05(-03) &   1.05(-03) \nl
Mg                &  1.84(-02)&   1.84(-02) &   1.84(-02) &   1.84(-02) &   1.84(-02) \nl
Al                &  9.80(-04)&   9.80(-04) &   9.80(-04) &   9.80(-04) &   9.80(-04) \nl
Si                &  3.97(-02)&   4.50(-02) &   4.52(-02) &   4.52(-02) &   4.52(-02) \nl
P                 &  3.21(-04)&   3.21(-04) &   3.21(-04) &   3.21(-04) &   3.21(-04) \nl
S                 &  2.01(-02)&   2.40(-02) &   2.42(-02) &   2.42(-02) &   2.42(-02) \nl
Cl                &  8.56(-05)&   8.57(-05) &   8.57(-05) &   8.58(-05) &   8.58(-05) \nl
Ar                &  3.54(-03)&   4.37(-03) &   4.48(-03) &   4.49(-03) &   4.50(-03) \nl
K                 &  6.49(-05)&   6.50(-05) &   6.50(-05) &   6.52(-05) &   6.53(-05) \nl
Ca                &  2.19(-03)&   3.04(-03) &   3.24(-03) &   3.33(-03) &   3.34(-03) \nl
Sc                &  7.96(-07)&   7.99(-07) &   8.00(-07) &   8.27(-07) &   8.28(-07) \nl
Ti                &  4.48(-05)&   5.97(-05) &   6.62(-05) &   1.48(-04) &   1.65(-04) \nl
V                 &  6.74(-06)&   8.61(-06) &   9.21(-06) &   9.24(-06) &   9.24(-06) \nl
Cr                &  3.30(-04)&   5.79(-04) &   7.45(-04) &   8.70(-04) &   8.93(-04) \nl
Mn                &  2.34(-04)&   3.25(-04) &   3.83(-04) &   3.93(-04) &   3.93(-04) \nl
Fe                &  1.76(-02)&   2.25(-02) &   2.78(-02) &   6.99(-02) &   8.04(-02) \nl
Co                &  9.24(-05)&   9.24(-05) &   9.24(-05) &   1.06(-03) &   1.32(-03) \nl
Ni                &  1.08(-03)&   1.15(-03) &   1.21(-03) &   3.65(-03) &   4.15(-03) \nl
Cu                &  2.93(-05)&   2.93(-05) &   2.93(-05) &   2.93(-05) &   2.93(-05) \nl
Zn                &  5.06(-05)&   5.06(-05) &   5.06(-05) &   5.07(-05) &   5.08(-05) \nl
\enddata           
\end{deluxetable} 


==> tablsc17.tex <==
\begin{deluxetable}{lrrrrr}
%\small
\tablenum{A2}
%\tablewidth{16cm}
\tablecaption{Explosive nucleosynthesis of the $\rm 13~M_\odot~~Z=10^{-3}$ model} 
\tablehead{
\colhead{}        & \colhead{(1)} & \colhead{(2)} & \colhead{(3)} & \colhead{(4)} & \colhead{(5)}
}
\startdata  
$\rm M(^{56}Ni)$  &    0.001  &      0.005  &      0.010  &      0.050  &      0.063  \nl  
$\rm M_{ejected}$ &      1.65 &        1.63 &        1.62 &        1.56 &        1.53 \nl  
$\rm M_{cut}$     &     11.35 &       11.37 &       11.38 &       11.44 &       11.47 \nl
C                 &  1.24(-01)&   1.24(-01) &   1.24(-01) &   1.24(-01) &   1.24(-01) \nl
N                 &  2.61(-03)&   2.61(-03) &   2.61(-03) &   2.61(-03) &   2.61(-03) \nl
O                 &  1.89(-01)&   1.89(-01) &   1.89(-01) &   1.89(-01) &   1.89(-01) \nl
F                 &  2.70(-07)&   2.70(-07) &   2.70(-07) &   2.70(-07) &   2.70(-07) \nl
Ne                &  1.05(-02)&   1.05(-02) &   1.05(-02) &   1.05(-02) &   1.05(-02) \nl
Na                &  1.37(-04)&   1.37(-04) &   1.37(-04) &   1.37(-04) &   1.37(-04) \nl
Mg                &  1.57(-02)&   1.57(-02) &   1.57(-02) &   1.57(-02) &   1.57(-02) \nl
Al                &  1.56(-04)&   1.56(-04) &   1.56(-04) &   1.56(-04) &   1.56(-04) \nl
Si                &  3.03(-02)&   3.87(-02) &   3.98(-02) &   3.99(-02) &   3.99(-02) \nl
P                 &  6.69(-05)&   6.70(-05) &   6.71(-05) &   6.71(-05) &   6.71(-05) \nl
S                 &  1.43(-02)&   2.00(-02) &   2.11(-02) &   2.12(-02) &   2.12(-02) \nl
Cl                &  1.71(-05)&   1.71(-05) &   1.71(-05) &   1.83(-05) &   2.39(-05) \nl
Ar                &  2.39(-03)&   3.55(-03) &   3.86(-03) &   3.92(-03) &   3.92(-03) \nl
K                 &  9.31(-06)&   9.33(-06) &   9.34(-06) &   9.34(-06) &   9.40(-06) \nl
Ca                &  1.94(-03)&   3.04(-03) &   3.47(-03) &   3.64(-03) &   3.68(-03) \nl
Sc                &  5.31(-08)&   5.49(-08) &   5.58(-08) &   6.37(-07) &   4.79(-06) \nl
Ti                &  7.76(-06)&   2.52(-05) &   3.64(-05) &   9.34(-05) &   1.37(-04) \nl
V                 &  7.42(-07)&   1.57(-06) &   1.90(-06) &   2.02(-06) &   2.02(-06) \nl
Cr                &  8.11(-05)&   3.37(-04) &   5.60(-04) &   7.59(-04) &   8.19(-04) \nl
Mn                &  3.20(-05)&   7.31(-05) &   9.72(-05) &   1.12(-04) &   1.12(-04) \nl
Fe                &  2.08(-03)&   6.32(-03) &   1.14(-02) &   5.25(-02) &   6.56(-02) \nl
Co                &  4.18(-06)&   4.18(-06) &   4.18(-06) &   4.47(-04) &   6.81(-04) \nl
Ni                &  7.66(-05)&   1.02(-04) &   1.18(-04) &   5.52(-04) &   1.07(-03) \nl
Cu                &  8.82(-07)&   8.82(-07) &   8.82(-07) &   8.82(-07) &   8.82(-07) \nl
Zn                &  2.09(-06)&   2.09(-06) &   2.09(-06) &   2.10(-06) &   2.14(-06) \nl
\enddata           
\end{deluxetable} 


==> tablsc18.tex <==
\begin{deluxetable}{lrrrrrr}
%\small
\tablenum{A3}
%\tablewidth{16cm}
\tablecaption{Explosive nucleosynthesis of the $\rm 15~M_\odot~~Z=2\cdot10^{-2}$ model} 
\tablehead{
\colhead{}        & \colhead{(1)} & \colhead{(2)} & \colhead{(3)} & \colhead{(4)} & \colhead{(5)} & \colhead{(6)}
}
\startdata  
$\rm M(^{56}Ni)$  &     0.001  &      0.005  &      0.010  &      0.050  &      0.100  &      0.129  \nl
$\rm M_{ejected}$ &      13.21 &       13.24 &       13.26 &       13.31 &       13.38 &       13.43 \nl
$\rm M_{cut}$     &       1.79 &        1.76 &        1.74 &        1.69 &        1.62 &        1.57 \nl
C                 &   1.72(-01)&   1.72(-01) &   1.72(-01) &   1.72(-01) &   1.72(-01) &   1.72(-01) \nl
N                 &   5.08(-02)&   5.08(-02) &   5.08(-02) &   5.08(-02) &   5.08(-02) &   5.08(-02) \nl
O                 &   5.51(-01)&   5.51(-01) &   5.51(-01) &   5.51(-01) &   5.51(-01) &   5.51(-01) \nl
F                 &   4.86(-06)&   4.86(-06) &   4.86(-06) &   4.86(-06) &   4.86(-06) &   4.86(-06) \nl
Ne                &   5.97(-02)&   5.97(-02) &   5.97(-02) &   5.97(-02) &   5.97(-02) &   5.97(-02) \nl
Na                &   1.59(-03)&   1.59(-03) &   1.59(-03) &   1.59(-03) &   1.59(-03) &   1.59(-03) \nl
Mg                &   2.91(-02)&   2.91(-02) &   2.91(-02) &   2.91(-02) &   2.91(-02) &   2.91(-02) \nl
Al                &   1.55(-03)&   1.55(-03) &   1.55(-03) &   1.55(-03) &   1.55(-03) &   1.55(-03) \nl
Si                &   8.20(-02)&   9.49(-02) &   9.82(-02) &   9.94(-02) &   9.94(-02) &   9.94(-02) \nl
P                 &   6.66(-04)&   6.66(-04) &   6.66(-04) &   6.66(-04) &   6.66(-04) &   6.66(-04) \nl
S                 &   4.04(-02)&   4.90(-02) &   5.18(-02) &   5.31(-02) &   5.31(-02) &   5.31(-02) \nl
Cl                &   1.42(-04)&   1.42(-04) &   1.42(-04) &   1.43(-04) &   1.43(-04) &   1.43(-04) \nl
Ar                &   6.85(-03)&   8.51(-03) &   9.19(-03) &   9.66(-03) &   9.67(-03) &   9.68(-03) \nl
K                 &   1.07(-04)&   1.07(-04) &   1.07(-04) &   1.07(-04) &   1.07(-04) &   1.07(-04) \nl
Ca                &   3.83(-03)&   5.32(-03) &   6.09(-03) &   6.87(-03) &   6.93(-03) &   6.99(-03) \nl
Sc                &   1.08(-06)&   1.09(-06) &   1.09(-06) &   1.09(-06) &   1.10(-06) &   1.10(-06) \nl
Ti                &   6.00(-05)&   8.00(-05) &   9.59(-05) &   1.36(-04) &   2.03(-04) &   2.57(-04) \nl
V                 &   9.44(-06)&   1.26(-05) &   1.43(-05) &   1.68(-05) &   1.68(-05) &   1.68(-05) \nl
Cr                &   4.17(-04)&   7.25(-04) &   1.01(-03) &   1.71(-03) &   1.81(-03) &   1.88(-03) \nl
Mn                &   2.97(-04)&   4.27(-04) &   5.16(-04) &   7.32(-04) &   7.32(-04) &   7.32(-04) \nl
Fe                &   2.14(-02)&   2.70(-02) &   3.27(-02) &   7.48(-02) &   1.27(-01) &   1.58(-01) \nl
Co                &   1.16(-04)&   1.16(-04) &   1.16(-04) &   2.52(-04) &   8.55(-04) &   1.57(-03) \nl
Ni                &   1.46(-03)&   1.57(-03) &   1.63(-03) &   2.93(-03) &   5.99(-03) &   7.64(-03) \nl
Cu                &   4.58(-05)&   4.58(-05) &   4.58(-05) &   4.58(-05) &   4.58(-05) &   4.58(-05) \nl
Zn                &   7.50(-05)&   7.50(-05) &   7.50(-05) &   7.50(-05) &   7.51(-05) &   7.52(-05) \nl
\enddata           
\end{deluxetable} 


==> tablsc19.tex <==
\begin{deluxetable}{lrrrrrr}
%\small
\tablenum{A4}
%\tablewidth{16cm}
\tablecaption{Explosive nucleosynthesis of the $\rm 15~M_\odot~~Z=10^{-3}$ model} 
\tablehead{
\colhead{}        & \colhead{(1)} & \colhead{(2)} & \colhead{(3)} & \colhead{(4)} & \colhead{(5)} & \colhead{(6)}
}
\startdata  
$\rm M(^{56}Ni)$  &     0.001   &     0.005   &     0.010   &     0.050   &     0.100   &     0.127  \nl
$\rm M_{ejected}$ &      13.18  &      13.21  &      13.23  &      13.28  &      13.35  &      13.39 \nl
$\rm M_{cut}$     &       1.82  &       1.79  &       1.77  &       1.72  &       1.65  &       1.61 \nl
C                 &   1.58(-01) &  1.58(-01)  &  1.58(-01)  &  1.58(-01)  &  1.58(-01)  &  1.58(-01) \nl
N                 &   3.16(-03) &  3.16(-03)  &  3.16(-03)  &  3.16(-03)  &  3.16(-03)  &  3.16(-03) \nl
O                 &   3.58(-01) &  3.58(-01)  &  3.58(-01)  &  3.58(-01)  &  3.58(-01)  &  3.58(-01) \nl
F                 &   3.42(-07) &  3.42(-07)  &  3.42(-07)  &  3.42(-07)  &  3.42(-07)  &  3.42(-07) \nl
Ne                &   1.56(-02) &  1.56(-02)  &  1.56(-02)  &  1.56(-02)  &  1.56(-02)  &  1.56(-02) \nl
Na                &   2.38(-04) &  2.38(-04)  &  2.38(-04)  &  2.38(-04)  &  2.38(-04)  &  2.38(-04) \nl
Mg                &   3.23(-02) &  3.23(-02)  &  3.23(-02)  &  3.23(-02)  &  3.23(-02)  &  3.23(-02) \nl
Al                &   3.46(-04) &  3.46(-04)  &  3.46(-04)  &  3.46(-04)  &  3.46(-04)  &  3.46(-04) \nl
Si                &   5.69(-02) &  7.12(-02)  &  7.65(-02)  &  7.80(-02)  &  7.80(-02)  &  7.80(-02) \nl
P                 &   1.33(-04) &  1.33(-04)  &  1.33(-04)  &  1.33(-04)  &  1.33(-04)  &  1.33(-04) \nl
S                 &   2.58(-02) &  3.51(-02)  &  3.94(-02)  &  4.10(-02)  &  4.10(-02)  &  4.10(-02) \nl
Cl                &   3.74(-05) &  3.74(-05)  &  3.75(-05)  &  3.75(-05)  &  4.04(-05)  &  4.35(-05) \nl
Ar                &   4.11(-03) &  5.86(-03)  &  6.86(-03)  &  7.38(-03)  &  7.39(-03)  &  7.40(-03) \nl
K                 &   1.73(-05) &  1.73(-05)  &  1.73(-05)  &  1.74(-05)  &  1.74(-05)  &  1.74(-05) \nl
Ca                &   3.15(-03) &  4.69(-03)  &  5.74(-03)  &  6.54(-03)  &  6.61(-03)  &  6.66(-03) \nl
Sc                &   8.22(-08) &  8.46(-08)  &  8.62(-08)  &  1.09(-07)  &  2.07(-06)  &  4.83(-06) \nl
Ti                &   9.15(-06) &  2.96(-05)  &  4.89(-05)  &  8.97(-05)  &  1.63(-04)  &  2.09(-04) \nl
V                 &   9.36(-07) &  2.04(-06)  &  2.75(-06)  &  3.50(-06)  &  3.50(-06)  &  3.50(-06) \nl
Cr                &   8.74(-05) &  3.68(-04)  &  6.70(-04)  &  1.30(-03)  &  1.41(-03)  &  1.47(-03) \nl
Mn                &   3.80(-05) &  8.82(-05)  &  1.26(-04)  &  1.90(-04)  &  1.90(-04)  &  1.90(-04) \nl
Fe                &   2.34(-03) &  6.67(-03)  &  1.18(-02)  &  5.27(-02)  &  1.04(-01)  &  1.32(-01) \nl
Co                &   6.19(-06) &  6.19(-06)  &  6.19(-06)  &  1.45(-04)  &  5.64(-04)  &  9.66(-04) \nl
Ni                &   9.66(-05) &  1.25(-04)  &  1.44(-04)  &  3.22(-04)  &  1.08(-03)  &  1.70(-03) \nl
Cu                &   1.10(-06) &  1.10(-06)  &  1.10(-06)  &  1.10(-06)  &  1.10(-06)  &  1.10(-06) \nl
Zn                &   2.51(-06) &  2.51(-06)  &  2.51(-06)  &  2.51(-06)  &  2.53(-06)  &  2.57(-06) \nl
\enddata           
\end{deluxetable} 































==> tablsc2.tex <==
\begin{deluxetable}{lcccc}
%\small
\tablenum{2}
\tablewidth{14cm}
\tablecaption{Selected quantities for $\rm 13~M_\odot$, $\rm 15~M_\odot$, $\rm 20~M_\odot$ and $\rm 25~M_\odot$ models.}
\tablehead{
\colhead{}   &
\colhead{$\rm 13~M_\odot$}    &
\colhead{$\rm 15~M_\odot$}    &
\colhead{$\rm 20~M_\odot$}    &
\colhead{$\rm 25~M_\odot$}    
}
\startdata  
\cutinhead{H Burning}
% HYDROGEN
 $\tau_{\rm H}$ (yr)                                                  &   1.25(7)     &   1.07(7)    &   7.48(6)    &    5.93(6)  \nl   
\tablevspace{0.1cm}                                                                   
 $\rm M_{\rm cc}$ ($\rm M_\odot$)                                     &    4.92       &    6.11      &   9.30       &   13.77     \nl   
\tablevspace{0.1cm}                                                                   
 $\Delta t_{\rm ~H~conv~shell}$           (yr)                        &   6.4(4)      &   4.8(4)     &   8.9(5)     &   8.2(5)    \nl   
\tablevspace{0.1cm}                                                                   
 $\Delta M_{\rm ~H~conv~shell}$           ($\rm M_\odot$)             & 2.50-5.60     & 3.32-6.33    & 4.71-10.69   & 6.74-15.95  \nl  
\tablevspace{0.1cm}                                                                   
 $\rm M_{\rm H~shell}^{\rm final}$ ($\rm M_\odot$)                    &    3.42       &    4.20      &   6.00       &    8.10     \nl   
\tablevspace{0.1cm}                                                                   
 $\rm M_{\rm He~core}^{\rm final}$ ($\rm M_\odot$)                    &    3.33       &    4.10      &   5.94       &    8.01     \nl  
\tablevspace{0.1cm}                                                                   
 $\rm R_{\rm H~shell}^{\rm final}$ ($\rm R_\odot$)                    &    2.00       &    1.00      &   6.80(-1)   &    6.70(-1) \nl   
\tablevspace{0.1cm}                                                                   
 $\rm R_{\rm He~core}^{\rm final}$ ($\rm R_\odot$)                    &    1.42       &    6.70(-1)  &   6.00(-1)   &    5.66(-1) \nl  
\cutinhead{Convective Envelope}                                                       
% CONVECTIVE ENVELOPE                                                                 
 $\rm M_{\rm  conv.~env.}^{\rm final}$ ($\rm M_\odot$)                &    3.48       &    4.28      &   6.15       &    8.27     \nl  
\tablevspace{0.1cm}                                                                   
 $\rm        ^{12}C/^{13}C $                                          &     18        &     93       &    91        &      90     \nl   
\tablevspace{0.1cm}                                                                   
 $\rm        ^{14}N/^{15}N $                                          &     1948      &     2132     &    2702      &     2977    \nl  
\tablevspace{0.1cm}                                                                   
 $\rm        ^{16}O/^{17}O $                                          &      745      &       881    &     919      &      1052   \nl   
\tablevspace{0.1cm}                                                                   
 $\rm        ^{16}O/^{18}O $                                          &      568      &       565    &     574      &      572    \nl   
\cutinhead{He Burning}                                                                
% HELIUM                                                                              
$\Delta t$(H exh.-He ign.)                                            &    5.47(4)    &   3.70(4)    &   1.89(4)    &   1.16(4)   \nl
\tablevspace{0.1cm}                                                                   
 $\tau_{\rm He}$ (yr)                                                 &    1.9(6)     &    1.4(6)    &   9.3(5)     &    6.8(5)   \nl  
\tablevspace{0.1cm}                                                                   
 $\rm M_{\rm cc}$ ($\rm M_\odot$)                                     &    1.73       &    2.33      &   3.63       &    5.23     \nl   
\tablevspace{0.1cm}                                                                   
$\rm ^{12}C/^{16}O$                                                   & 0.257/0.717   & 0.195/0.777  & 0.171/0.800  & 0.179/0.790 \nl  
\tablevspace{0.1cm}                                                                   
 $\Delta t_{\rm ~1~He~conv~shell}$ (yr)                               &    3.0(2)     &    3.8(4)    &   2.2(3)     &    6.2(3)   \nl   
\tablevspace{0.1cm}                                                                   
 $\Delta M_{\rm ~1~He~conv~shell}$       ($\rm M_\odot$)              & 1.94-2.03     & 2.50-2.88    & 3.86-4.54    & 5.46-6.45   \nl  
\tablevspace{0.1cm}                                                                   
 $\Delta t_{\rm ~2~He~conv~shell}$ (yr)                               &    1.7(2)     &    1.9(3)    &  1.18(3)     &    2.37(3)  \nl   
\tablevspace{0.1cm}                                                                   
 $\Delta M_{\rm ~2~He~conv~shell}$       ($\rm M_\odot$)              & 1.75-3.08     & 2.43-3.54    & 3.73-5.64    & 5.30-7.68   \nl  
\tablevspace{0.1cm}                                                                   
$\rm ^{4}He_{\rm shell}$                                              &  0.809        &    0.858     &   0.863      &   0.877     \nl
\tablevspace{0.1cm}                                                                   
$\rm ^{12}C_{\rm shell}$                                              &  8.95(-2)     &    8.36(-2)  &  8.49(-2)    &   8.04(-2)  \nl
\tablevspace{0.1cm}                                                                   
$\rm ^{16}O_{\rm shell}$                                              &  7.47(-2)     &    3.23(-2)  &  2.59(-2)    &   1.67(-2)  \nl
\tablevspace{0.1cm}                                                                   
$\rm ^{18}O_{\rm shell}$                                              &  5.23(-4)     &    1.92(-3)  &  4.86(-4)    &   4.81(-4)  \nl
\tablevspace{0.1cm}                                                                   
$\rm ^{22}Ne_{\rm shell}$                                             &  1.82(-2)     &    1.82(-2)  &  2.01(-2)    &   2.01(-2)  \nl
\tablevspace{0.1cm}                                                                   
$\rm ^{25}Mg_{\rm shell}$                                             &  9.07(-4)     &    9.55(-5)  &  1.23(-4)    &   9.49(-5)  \nl
\tablevspace{0.1cm}                                                                   
$\rm ^{56}Fe_{\rm shell}$                                             &  9.17(-4)     &    1.15(-3)  &  1.13(-3)    &   1.13(-3)  \nl
\tablevspace{0.1cm}                                                                   
 $\rm M_{\rm He~shell}^{\rm final}$ ($\rm M_\odot$)                   &    1.75       &    2.43      &   3.73       &    5.31     \nl   
\tablevspace{0.1cm}                                                                   
 $\rm M_{\rm CO~core}^{\rm final}$ ($\rm M_\odot$)                    &    1.75       &    2.39      &   3.44       &    4.90     \nl   
\tablevspace{0.1cm}                                                                   
 $\rm R_{\rm He~shell}^{\rm final}$ ($\rm R_\odot$)                   &    2.18(-2)   &    4.00(-2)  &   4.63(-2)   &    7.12(-2) \nl   
\tablevspace{0.1cm}                                                                   
 $\rm R_{\rm CO~core}^{\rm final}$ ($\rm R_\odot$)                    &    2.18(-2)   &    3.41(-2)  &   2.92(-2)   &    5.22(-2) \nl  
\tablebreak                                                                           
\cutinhead{C Burning}                                                                 
% CARBON                                                                              
$\Delta t$(He exh.-C ign.)                                            &    5.94(4)    &   3.67(4)    &  2.16(4)     &   1.59(4)   \nl
\tablevspace{0.1cm}                                                                   
 $\tau_{\rm C }$ (yr)                                             &    4.8(3)     &    2.6(3)    &   1.45(3)    &    9.7(2)   \nl  
\tablevspace{0.1cm}                                                                   
 $\rm M_{\rm cc}$ ($\rm M_\odot$)                                     &    0.56       &    0.41      &              &             \nl   
\tablevspace{0.1cm}                                                                   
 $\Delta t_{\rm ~1~C~conv~shell}$ (yr)                                &    6.30(2)    &    2.40(2)   &   2.80       &    5.64     \nl   
\tablevspace{0.1cm}                                                                   
 $\Delta M_{\rm ~1~C~conv~shell}$ ($\rm M_\odot$)                     & 0.55-1.10     & 0.39-0.80    & 1.07-1.50    & 1.48-2.43   \nl  
\tablevspace{0.1cm}                                                                   
 $\Delta t_{\rm ~2~C~conv~shell}$ (yr)                                &    60         &    56        &   2.16       &    0.34     \nl   
\tablevspace{0.1cm}                                                                   
 $\Delta M_{\rm ~2~C~conv~shell}$ ($\rm M_\odot$)                     & 0.92-1.42     & 0.80-1.20    & 1.46-2.64    & 2.28-4.61   \nl  
\tablevspace{0.1cm}                                                                   
 $\Delta t_{\rm ~3~C~conv~shell}$ (yr)                                &   8.7         &   13         &   3.8(-4)    &             \nl   
\tablevspace{0.1cm}                                                                   
 $\Delta M_{\rm ~3~C~conv~shell}$ ($\rm M_\odot$)                     & 1.25-1.64     & 1.18-1.77    & 2.39-2.77    &             \nl  
\tablevspace{0.1cm}                                                                   
 $\Delta t_{\rm ~4~C~conv~shell}$ (yr)                                &   1.32(-2)    &   0.7        &              &             \nl   
\tablevspace{0.1cm}                                                                   
 $\Delta M_{\rm ~4~C~conv~shell}$ ($\rm M_\odot$)                     & 1.52-1.75     & 1.56-1.67    &              &             \nl  
\tablevspace{0.1cm}                                                                   
 $\Delta t_{\rm ~5~C~conv~shell}$ (yr)                                &               &   0.32       &              &             \nl   
\tablevspace{0.1cm}                                                                   
 $\Delta M_{\rm ~5~C~conv~shell}$ ($\rm M_\odot$)                     &               & 1.64-2.18    &              &             \nl  
\tablevspace{0.1cm}                                                                   
 $\rm M_{\rm  C~shell}^{\rm final}$ ($\rm M_\odot$)                   &    1.56       &    1.80      &   2.41       &    2.39     \nl   
\tablevspace{0.1cm}                                                                   
 $\rm R_{\rm  C~shell}^{\rm final}$ ($\rm R_\odot$)                   &    7.03(-3)   &    9.29(-3)  &   1.14(-2)   &    1.09(-2) \nl   
\cutinhead{Ne Burning}                                                                
% NEON   
$\Delta t$(C exh.-Ne ign.)                                            &    1.52(3)    &   5.50(2)    &   3.02(2)    &    9.20(1)  \nl
\tablevspace{0.1cm}                                                                   
 $\tau_{\rm Ne}$ (yr)                                                 &    3.00       &    2.00      &   1.46       &    0.77     \nl  
\tablevspace{0.1cm}                                                                   
 $\rm M_{\rm cc}$ ($\rm M_\odot$)                                     &    0.86       &    0.66      &   0.50       &    0.50     \nl   
\tablevspace{0.1cm}                                                                   
 $\Delta t_{\rm ~1~Ne~conv~shell}$ (yr)                               &    3.40(-2)   &    0.05      &              &             \nl   
\tablevspace{0.1cm}                                                                   
 $\Delta M_{\rm ~1~Ne~conv~shell}$ ($\rm M_\odot$)                    & 0.93-1.26     & 0.93-1.24    &              &             \nl  
\tablevspace{0.1cm}                                                                   
 $\Delta t_{\rm ~2~Ne~conv~shell}$ (yr)                               &    1.39(-2)   &              &              &             \nl   
\tablevspace{0.1cm}                                                                   
 $\Delta M_{\rm ~2~Ne~conv~shell}$ ($\rm M_\odot$)                    & 1.33-1.42     &              &              &             \nl  
\tablevspace{0.1cm}                                                                   
 $\Delta t_{\rm ~3~Ne~conv~shell}$ (yr)                               &    8.40(-3)   &              &              &             \nl   
\tablevspace{0.1cm}                                                                   
 $\Delta M_{\rm ~3~Ne~conv~shell}$ ($\rm M_\odot$)                    & 1.42-1.47     &              &              &             \nl  
\tablevspace{0.1cm}                                                                   
 $\rm M_{\rm Ne~shell}^{\rm final}$ ($\rm M_\odot$)                   &    1.52       &    1.69      &   2.24       &    2.28     \nl   
\tablevspace{0.1cm}                                                                   
 $\rm R_{\rm Ne~shell}^{\rm final}$ ($\rm R_\odot$)                   &    5.70(-3)   &    7.04(-3)  &   9.66(-3)   &    9.12(-3) \nl   
\cutinhead{O Burning}                                                                 
% OSSIGENO                                                                            
$\Delta t$(Ne exh.-O ign.)                                            &    2.66       &   0.00       &   0.00       &    0.00     \nl
\tablevspace{0.1cm}                                                                   
 $\tau_{\rm O }$ (yr)                                                 &    8.07       &    2.47      &   0.72       &    0.33     \nl  
\tablevspace{0.1cm}                                                                   
 $\rm M_{\rm cc}$ ($\rm M_\odot$)                                     &    0.93       &    0.94      &   1.12       &    1.15     \nl   
\tablevspace{0.1cm}                                                                   
 $\Delta t_{\rm ~1~O~conv~shell}$ (yr)                                &    2.8(-1)    &    2.0(-1)   &   2.8(-2)    &    3.0(-2)  \nl   
\tablevspace{0.1cm}                                                                   
 $\Delta M_{\rm ~1~O~conv~shell}$ ($\rm M_\odot$)                     & 0.92-1.33     & 0.92-1.44    & 1.11-1.77    & 1.14-1.86   \nl  
\tablevspace{0.1cm}                                                                   
 $\Delta t_{\rm ~2~O~conv~shell}$ (yr)                                &  1.7(-2)      &  1.0(-2)     &   2.3(-3)    &    1.4(-3)  \nl   
\tablevspace{0.1cm}                                                                   
 $\Delta M_{\rm ~2~O~conv~shell}$ ($\rm M_\odot$)                     & 0.48-0.92     & 0.46-0.92    & 0.76-1.11    & 0.97-1.12   \nl  
\tablevspace{0.1cm}                                                                   
 $\Delta t_{\rm ~3~O~conv~shell}$ (yr)                                &  1.4(-2)      &  3.0(-4)     &   2.3(-4)    &    8.0(-5)  \nl   
\tablevspace{0.1cm}                                                                   
 $\Delta M_{\rm ~3~O~conv~shell}$ ($\rm M_\odot$)                     & 1.05-1.39     & 1.43-1.65    & 1.64-2.22    & 1.83-2.09   \nl  
\tablevspace{0.1cm}                                                                   
 $\rm M_{\rm  O~shell}^{\rm final}$ ($\rm M_\odot$)                   &    1.39       &    1.48      &   1.74       &    1.84     \nl   
\tablevspace{0.1cm}                                                                   
 $\rm R_{\rm  O~shell}^{\rm final}$ ($\rm R_\odot$)                   &    3.74(-3)   &    3.80(-3)  &   4.42(-2)   &    4.75(-3) \nl   
\tablebreak                                                                           
\cutinhead{Si Burning Radiative}                                                      
% SILICIO RADIATIVO                                                                   
$\Delta t$(O exh.-Si ign.)                                            &    4.48(-1)   &   1.50(-2)   &   3.00(-2)   &   3.00(-2)  \nl
\tablevspace{0.1cm}                                                                   
 $\tau_{\rm Si-rad}$ (yr)                                             &    0.58       &    0.29      &   2.80(-2)   &    1.94(-2) \nl  
\tablevspace{0.1cm}                                                                   
 ${\rm Log}T_{\rm c}$                                                 &  9.308-9.497  &  9.342-9.486 & 9.367-9.507  & 9.360-9.497 \nl  
\tablevspace{0.1cm}                                                                   
 ${\rm Log}\rho_{\rm c}$                                              &  7.808-8.643  &  7.362-8.351 & 7.475-8.007  & 7.480-7.980 \nl  
\cutinhead{Si Burning Convective}                                                     
% SILICIO CONVECTIVO                                                                  
 $\tau_{\rm Si-con}$ (yr)                                             &    0.07       &    0.02      &   3.50(-3)   &    3.41(-3) \nl  
\tablevspace{0.1cm}                                                                   
 $\rm M_{\rm cc}$ ($\rm M_\odot$)                                     &    1.13       &    1.14      &   1.11       &    1.12     \nl   
\tablevspace{0.1cm}                                                                   
 $\Delta t_{\rm ~1~Si~conv~shell}$ (yr)                               &    1.4(-4)    &    1.0(-5)   &   2.5(-5)    &    1.9(-5)  \nl   
\tablevspace{0.1cm}                                                                   
 $\Delta M_{\rm ~1~Si~conv~shell}$ ($\rm M_\odot$)                    & 0.47-0.83     & 0.65-0.82    & 0.88-1.11    & 0.88-1.13   \nl  
\tablevspace{0.1cm}                                                                   
 $\Delta t_{\rm ~2~Si~conv~shell}$ (yr)                               &    5.6(-4)    &    3.0(-5)   &   8.1(-5)    &    4.3(-5)  \nl   
\tablevspace{0.1cm}                                                                   
 $\Delta M_{\rm ~2~Si~conv~shell}$ ($\rm M_\odot$)                    & 0.84-1.29     & 0.81-1.02    & 1.11-1.57    & 1.09-1.54   \nl  
\tablevspace{0.1cm}                                                                   
 $\Delta t_{\rm ~3~Si~conv~shell}$ (yr)                               &    1.3(-5)    &    2.3(-6)   &   6.9(-6)    &             \nl   
\tablevspace{0.1cm}                                                                   
 $\Delta M_{\rm ~3~Si~conv~shell}$ ($\rm M_\odot$)                    & 0.84-1.05     & 1.00-1.13    & 1.11-1.28    &             \nl  
\tablevspace{0.1cm}                                                                   
 $\Delta t_{\rm ~4~Si~conv~shell}$ (yr)                               &               &    1.1(-5)   &              &             \nl   
\tablevspace{0.1cm}                                                                   
 $\Delta M_{\rm ~4~Si~conv~shell}$ ($\rm M_\odot$)                    &               & 1.02-1.43    &              &             \nl  
\tablevspace{0.1cm}                                                                   
 $\rm M_{\rm Si~shell}^{\rm final}$ ($\rm M_\odot$)                   &    1.09       &    1.29      &   1.43       &    1.54     \nl   
\tablevspace{0.1cm}                                                                   
 $\rm R_{\rm Si~shell}^{\rm final}$ ($\rm R_\odot$)                   &    2.40(-3)   &    2.24(-3)  &   2.79(-3)   &    3.11(-3) \nl   
\cutinhead{Last Model}                                                                
% LAST MODEL                                                                          
  ${\rm Log}~T_{\rm c}$                                               &     9.60      &     9.72     &    9.72      &     9.74     \nl 
\tablevspace{0.1cm}                                                                   
  ${\rm Log}~\rho_{\rm c}$                                            &     9.00      &     9.53     &    9.26      &     9.20     \nl 
\tablevspace{0.1cm}                                                                   
  $\psi_{\rm c}$\tablenotemark{a}                                     &    10.10      &    12.03     &    9.35      &     8.57     \nl 
\tablevspace{0.1cm}                                                                   
  $\eta_{\rm c}$\tablenotemark{b}                                     &     0.124     &     0.136    &    0.130     &     0.128    \nl 
\tablevspace{0.1cm}                                                                   
  $Y_{\rm e,c}$                                                       &     0.438     &     0.432    &    0.435     &     0.436    \nl 
\tablevspace{0.1cm}                                                                   
  $S_{\rm c}/(N_{\rm A}k)$                                            &     0.438     &     0.432    &    0.435     &     0.436    \nl 
\tablevspace{0.1cm}                                                                   
  $M_{\rm Fe}$ ($\rm M_\odot$)                                        &     1.292     &     1.429    &    1.552     &     1.527    \nl 
\tablevspace{0.1cm}                                                                   
  $R_{\rm Fe}$ ($\rm R_\odot$)                                        &     2.95(-3)  &     3.07(-3) &    3.30(-3)  &    3.09(-3)  \nl 
\tablenotetext{a}{Cantral value of the degeneracy parameter}
\tablenotetext{b}{Central value of the neutron excess}
\enddata        
\end{deluxetable}


==> tablsc20.tex <==
\begin{deluxetable}{lrrrrr}
%\small
\tablenum{A5}
%\tablewidth{16cm}
\tablecaption{Explosive nucleosynthesis of the $\rm 15~M_\odot~~Z=0$ model} 
\tablehead{
\colhead{}        & \colhead{(1)} & \colhead{(2)} & \colhead{(3)} & \colhead{(4)} & \colhead{(5)} 
}
\startdata  
$\rm M(^{56}Ni)$  &      0.001  &      0.005   &     0.010   &     0.050  &      0.065  \nl
$\rm M_{ejected}$ &       13.31 &       13.34  &      13.35  &      13.40 &       13.43 \nl
$\rm M_{cut}$     &        1.69 &        1.66  &       1.65  &       1.60 &        1.57 \nl
C                 &    1.05(-01)&   1.05(-01)  &  1.05(-01)  &  1.05(-01) &   1.05(-01) \nl
N                 &    1.12(-02)&   1.12(-02)  &  1.12(-02)  &  1.12(-02) &   1.12(-02) \nl
O                 &    1.63(-01)&   1.63(-01)  &  1.63(-01)  &  1.63(-01) &   1.63(-01) \nl
F                 &    3.00(-11)&   3.00(-11)  &  3.00(-11)  &  3.00(-11) &   3.00(-11) \nl
Ne                &    3.99(-03)&   3.99(-03)  &  3.99(-03)  &  3.99(-03) &   3.99(-03) \nl
Na                &    2.64(-05)&   2.64(-05)  &  2.64(-05)  &  2.64(-05) &   2.64(-05) \nl
Mg                &    1.36(-02)&   1.36(-02)  &  1.36(-02)  &  1.36(-02) &   1.36(-02) \nl
Al                &    5.23(-05)&   5.23(-05)  &  5.23(-05)  &  5.23(-05) &   5.23(-05) \nl
Si                &    2.74(-02)&   3.67(-02)  &  3.87(-02)  &  3.88(-02) &   3.88(-02) \nl
P                 &    2.42(-05)&   2.44(-05)  &  2.45(-05)  &  2.46(-05) &   2.47(-05) \nl
S                 &    1.38(-02)&   2.02(-02)  &  2.19(-02)  &  2.21(-02) &   2.21(-02) \nl
Cl                &    9.58(-06)&   9.62(-06)  &  9.63(-06)  &  1.27(-05) &   2.03(-05) \nl
Ar                &    2.48(-03)&   3.73(-03)  &  4.19(-03)  &  4.27(-03) &   4.27(-03) \nl
K                 &    4.19(-06)&   4.20(-06)  &  4.21(-06)  &  4.23(-06) &   4.31(-06) \nl
Ca                &    2.24(-03)&   3.41(-03)  &  3.99(-03)  &  4.19(-03) &   4.23(-03) \nl
Sc                &    2.14(-08)&   2.29(-08)  &  2.38(-08)  &  1.69(-06) &   7.92(-06) \nl
Ti                &    5.85(-06)&   2.37(-05)  &  3.72(-05)  &  9.09(-05) &   1.42(-04) \nl
V                 &    2.19(-07)&   6.16(-07)  &  7.72(-07)  &  7.97(-07) &   7.97(-07) \nl
Cr                &    6.06(-05)&   3.16(-04)  &  5.60(-04)  &  7.82(-04) &   8.53(-04) \nl
Mn                &    1.24(-05)&   3.34(-05)  &  4.40(-05)  &  4.68(-05) &   4.68(-05) \nl
Fe                &    1.12(-03)&   5.21(-03)  &  1.03(-02)  &  5.08(-02) &   6.64(-02) \nl
Co                &    2.13(-08)&   2.21(-08)  &  2.25(-08)  &  1.92(-04) &   3.77(-04) \nl
Ni                &    1.84(-05)&   3.53(-05)  &  4.60(-05)  &  8.44(-04) &   1.53(-03) \nl
Cu                &    1.23(-14)&   1.23(-14)  &  1.23(-14)  &  3.59(-14) &   3.22(-13) \nl
Zn                &    5.76(-14)&   5.76(-14)  &  5.76(-14)  &  1.22(-08) &   4.62(-08) \nl
\enddata           
\end{deluxetable} 

























































==> tablsc21.tex <==
\begin{deluxetable}{lrrrrrrrr}
%\small
\tablenum{A6}
%\tablewidth{16cm}
\tablecaption{Explosive nucleosynthesis of the $\rm 20~M_\odot~~Z=2\cdot10^{-2}$ model} 
\tablehead{
\colhead{}        & \colhead{(1)} & \colhead{(2)} & \colhead{(3)} & \colhead{(4)} & \colhead{(5)} & \colhead{(6)} & \colhead{(7)} & \colhead{(8)}
}
\startdata  
$\rm M(^{56}Ni)$  &     0.001   &     0.005   &     0.010   &     0.050   &     0.100   &     0.150   &     0.200   &     0.244  \nl
$\rm M_{ejected}$ &      17.76  &      17.81  &      17.84  &      17.90  &      17.96  &      18.02  &      18.09  &      18.16 \nl
$\rm M_{cut}$     &       2.24  &       2.19  &       2.16  &       2.10  &       2.04  &       1.98  &       1.91  &       1.84 \nl
C                 &   3.05(-01) &  3.05(-01)  &  3.05(-01)  &  3.05(-01)  &  3.05(-01)  &  3.05(-01)  &  3.05(-01)  &  3.05(-01) \nl
N                 &   7.31(-02) &  7.31(-02)  &  7.31(-02)  &  7.31(-02)  &  7.31(-02)  &  7.31(-02)  &  7.31(-02)  &  7.31(-02) \nl
O                 &   1.19(+00) &  1.19(+00)  &  1.19(+00)  &  1.19(+00)  &  1.19(+00)  &  1.19(+00)  &  1.19(+00)  &  1.19(+00) \nl
F                 &   6.82(-06) &  6.82(-06)  &  6.82(-06)  &  6.82(-06)  &  6.82(-06)  &  6.82(-06)  &  6.82(-06)  &  6.82(-06) \nl
Ne                &   9.42(-02) &  9.42(-02)  &  9.42(-02)  &  9.42(-02)  &  9.42(-02)  &  9.42(-02)  &  9.42(-02)  &  9.42(-02) \nl
Na                &   2.59(-03) &  2.59(-03)  &  2.59(-03)  &  2.59(-03)  &  2.59(-03)  &  2.59(-03)  &  2.59(-03)  &  2.59(-03) \nl
Mg                &   4.30(-02) &  4.30(-02)  &  4.30(-02)  &  4.30(-02)  &  4.30(-02)  &  4.30(-02)  &  4.30(-02)  &  4.30(-02) \nl
Al                &   2.95(-03) &  2.95(-03)  &  2.95(-03)  &  2.95(-03)  &  2.95(-03)  &  2.95(-03)  &  2.95(-03)  &  2.95(-03) \nl
Si                &   1.67(-01) &  1.92(-01)  &  2.03(-01)  &  2.10(-01)  &  2.10(-01)  &  2.10(-01)  &  2.10(-01)  &  2.10(-01) \nl
P                 &   1.35(-03) &  1.35(-03)  &  1.35(-03)  &  1.35(-03)  &  1.35(-03)  &  1.35(-03)  &  1.35(-03)  &  1.35(-03) \nl
S                 &   8.76(-02) &  1.02(-01)  &  1.10(-01)  &  1.17(-01)  &  1.17(-01)  &  1.17(-01)  &  1.17(-01)  &  1.17(-01) \nl
Cl                &   3.91(-04) &  3.91(-04)  &  3.91(-04)  &  3.91(-04)  &  3.91(-04)  &  3.91(-04)  &  3.92(-04)  &  3.92(-04) \nl
Ar                &   1.47(-02) &  1.72(-02)  &  1.88(-02)  &  2.07(-02)  &  2.07(-02)  &  2.07(-02)  &  2.07(-02)  &  2.07(-02) \nl
K                 &   2.32(-04) &  2.32(-04)  &  2.32(-04)  &  2.32(-04)  &  2.32(-04)  &  2.33(-04)  &  2.33(-04)  &  2.33(-04) \nl
Ca                &   7.56(-03) &  9.64(-03)  &  1.11(-02)  &  1.36(-02)  &  1.36(-02)  &  1.37(-02)  &  1.37(-02)  &  1.38(-02) \nl
Sc                &   2.10(-06) &  2.11(-06)  &  2.11(-06)  &  2.12(-06)  &  2.12(-06)  &  2.12(-06)  &  2.14(-06)  &  2.15(-06) \nl
Ti                &   1.01(-04) &  1.24(-04)  &  1.47(-04)  &  2.18(-04)  &  2.38(-04)  &  2.78(-04)  &  3.42(-04)  &  4.02(-04) \nl
V                 &   1.61(-05) &  2.06(-05)  &  2.34(-05)  &  2.98(-05)  &  2.98(-05)  &  2.98(-05)  &  2.98(-05)  &  2.98(-05) \nl
Cr                &   6.08(-04) &  9.64(-04)  &  1.32(-03)  &  2.83(-03)  &  2.86(-03)  &  2.92(-03)  &  3.00(-03)  &  3.09(-03) \nl
Mn                &   4.34(-04) &  5.98(-04)  &  7.27(-04)  &  1.15(-03)  &  1.15(-03)  &  1.15(-03)  &  1.15(-03)  &  1.15(-03) \nl
Fe                &   2.96(-02) &  3.61(-02)  &  4.24(-02)  &  8.54(-02)  &  1.37(-01)  &  1.89(-01)  &  2.41(-01)  &  2.88(-01) \nl
Co                &   2.25(-04) &  2.25(-04)  &  2.25(-04)  &  2.52(-04)  &  5.03(-04)  &  8.60(-04)  &  1.50(-03)  &  2.29(-03) \nl
Ni                &   2.47(-03) &  2.63(-03)  &  2.73(-03)  &  3.36(-03)  &  5.91(-03)  &  8.53(-03)  &  1.07(-02)  &  1.21(-02) \nl
Cu                &   1.32(-04) &  1.32(-04)  &  1.32(-04)  &  1.32(-04)  &  1.32(-04)  &  1.32(-04)  &  1.32(-04)  &  1.32(-04) \nl
Zn                &   2.34(-04) &  2.34(-04)  &  2.34(-04)  &  2.34(-04)  &  2.34(-04)  &  2.34(-04)  &  2.35(-04)  &  2.35(-04) \nl
\enddata           
\end{deluxetable}


































==> tablsc22.tex <==
\begin{deluxetable}{lrrrrrrrr}
%\small
\tablenum{A7}
%\tablewidth{16cm}
\tablecaption{Explosive nucleosynthesis of the $\rm 20~M_\odot~~Z=10^{-3}$ model} 
\tablehead{
\colhead{}        & \colhead{(1)} & \colhead{(2)} & \colhead{(3)} & \colhead{(4)} & \colhead{(5)} & \colhead{(6)} & \colhead{(7)} & \colhead{(8)}
}
\startdata  
$\rm M(^{56}Ni)$  &    0.001   &     0.005   &     0.010   &     0.050  &      0.100   &     0.150   &     0.200   &     0.225  \nl
$\rm M_{ejected}$ &     18.07  &      18.12  &      18.14  &      18.21 &       18.27  &      18.33  &      18.40  &      18.44 \nl
$\rm M_{cut}$     &      1.93  &       1.88  &       1.86  &       1.79 &        1.73  &       1.67  &       1.60  &       1.56 \nl
C                 &  2.75(-01) &  2.75(-01)  &  2.75(-01)  &  2.75(-01) &   2.75(-01)  &  2.75(-01)  &  2.75(-01)  &  2.75(-01) \nl
N                 &  4.76(-03) &  4.76(-03)  &  4.76(-03)  &  4.76(-03) &   4.76(-03)  &  4.76(-03)  &  4.76(-03)  &  4.76(-03) \nl
O                 &  1.02(+00) &  1.02(+00)  &  1.02(+00)  &  1.02(+00) &   1.02(+00)  &  1.02(+00)  &  1.02(+00)  &  1.02(+00) \nl
F                 &  4.16(-07) &  4.16(-07)  &  4.16(-07)  &  4.16(-07) &   4.16(-07)  &  4.16(-07)  &  4.16(-07)  &  4.16(-07) \nl
Ne                &  2.00(-01) &  2.00(-01)  &  2.00(-01)  &  2.00(-01) &   2.00(-01)  &  2.00(-01)  &  2.00(-01)  &  2.00(-01) \nl
Na                &  2.02(-03) &  2.02(-03)  &  2.02(-03)  &  2.02(-03) &   2.02(-03)  &  2.02(-03)  &  2.02(-03)  &  2.02(-03) \nl
Mg                &  7.42(-02) &  7.42(-02)  &  7.42(-02)  &  7.42(-02) &   7.42(-02)  &  7.42(-02)  &  7.42(-02)  &  7.42(-02) \nl
Al                &  1.28(-03) &  1.28(-03)  &  1.28(-03)  &  1.28(-03) &   1.28(-03)  &  1.28(-03)  &  1.28(-03)  &  1.28(-03) \nl
Si                &  8.00(-02) &  1.02(-01)  &  1.13(-01)  &  1.21(-01) &   1.21(-01)  &  1.21(-01)  &  1.21(-01)  &  1.21(-01) \nl
P                 &  1.64(-04) &  1.64(-04)  &  1.64(-04)  &  1.64(-04) &   1.64(-04)  &  1.64(-04)  &  1.64(-04)  &  1.64(-04) \nl
S                 &  3.69(-02) &  5.05(-02)  &  5.83(-02)  &  6.60(-02) &   6.60(-02)  &  6.60(-02)  &  6.60(-02)  &  6.60(-02) \nl
Cl                &  5.81(-05) &  5.82(-05)  &  5.82(-05)  &  5.82(-05) &   5.83(-05)  &  5.83(-05)  &  5.85(-05)  &  5.85(-05) \nl
Ar                &  5.90(-03) &  8.33(-03)  &  9.89(-03)  &  1.20(-02) &   1.20(-02)  &  1.20(-02)  &  1.20(-02)  &  1.20(-02) \nl
K                 &  2.37(-05) &  2.37(-05)  &  2.37(-05)  &  2.37(-05) &   2.38(-05)  &  2.40(-05)  &  2.42(-05)  &  2.44(-05) \nl
Ca                &  4.45(-03) &  6.47(-03)  &  7.96(-03)  &  1.06(-02) &   1.06(-02)  &  1.07(-02)  &  1.07(-02)  &  1.08(-02) \nl
Sc                &  1.27(-07) &  1.30(-07)  &  1.32(-07)  &  1.36(-07) &   1.42(-07)  &  1.42(-07)  &  1.76(-07)  &  1.84(-07) \nl
Ti                &  1.05(-05) &  3.30(-05)  &  5.58(-05)  &  1.23(-04) &   1.49(-04)  &  1.93(-04)  &  2.69(-04)  &  2.98(-04) \nl
V                 &  9.51(-07) &  2.13(-06)  &  3.02(-06)  &  4.81(-06) &   4.81(-06)  &  4.81(-06)  &  4.82(-06)  &  4.82(-06) \nl
Cr                &  8.75(-05) &  3.81(-04)  &  7.11(-04)  &  2.05(-03) &   2.09(-03)  &  2.15(-03)  &  2.25(-03)  &  2.29(-03) \nl
Mn                &  3.89(-05) &  9.04(-05)  &  1.33(-04)  &  2.63(-04) &   2.63(-04)  &  2.63(-04)  &  2.63(-04)  &  2.63(-04) \nl
Fe                &  2.59(-03) &  6.94(-03)  &  1.22(-02)  &  5.29(-02) &   1.04(-01)  &  1.56(-01)  &  2.08(-01)  &  2.36(-01) \nl
Co                &  1.44(-05) &  1.44(-05)  &  1.44(-05)  &  5.25(-05) &   2.92(-04)  &  6.81(-04)  &  1.52(-03)  &  2.06(-03) \nl
Ni                &  1.28(-04) &  1.57(-04)  &  1.77(-04)  &  2.57(-04) &   7.31(-04)  &  2.65(-03)  &  4.30(-03)  &  5.59(-03) \nl
Cu                &  3.01(-06) &  3.01(-06)  &  3.01(-06)  &  3.01(-06) &   3.01(-06)  &  3.01(-06)  &  3.01(-06)  &  3.01(-06) \nl
Zn                &  6.18(-06) &  6.18(-06)  &  6.18(-06)  &  6.18(-06) &   6.19(-06)  &  6.23(-06)  &  6.31(-06)  &  6.49(-06) \nl
\enddata           
\end{deluxetable}






























































==> tablsc23.tex <==
\begin{deluxetable}{lrrrrrrr}
%\small
\tablenum{A8}
%\tablewidth{16cm}
\tablecaption{Explosive nucleosynthesis of the $\rm 20~M_\odot~~Z=0$ model} 
\tablehead{
\colhead{}        & \colhead{(1)} & \colhead{(2)} & \colhead{(3)} & \colhead{(4)} & \colhead{(5)} & \colhead{(6)} & \colhead{(7)} 
}
\startdata  
$\rm M(^{56}Ni)$  &      0.001   &     0.005   &     0.010   &     0.050   &     0.100   &     0.150   &     0.201  \nl
$\rm M_{ejected}$ &       18.02  &      18.07  &      18.10  &      18.16  &      18.22  &      18.29  &      18.36 \nl
$\rm M_{cut}$     &        1.98  &       1.93  &       1.90  &       1.84  &       1.78  &       1.71  &       1.64 \nl
C                 &    2.48(-01) &  2.48(-01)  &  2.48(-01)  &  2.48(-01)  &  2.48(-01)  &  2.48(-01)  &  2.48(-01) \nl
N                 &    4.24(-03) &  4.24(-03)  &  4.24(-03)  &  4.24(-03)  &  4.24(-03)  &  4.24(-03)  &  4.24(-03) \nl
O                 &    9.15(-01) &  9.15(-01)  &  9.15(-01)  &  9.15(-01)  &  9.15(-01)  &  9.15(-01)  &  9.15(-01) \nl
F                 &    3.01(-10) &  3.01(-10)  &  3.01(-10)  &  3.01(-10)  &  3.01(-10)  &  3.01(-10)  &  3.01(-10) \nl
Ne                &    1.05(-01) &  1.05(-01)  &  1.05(-01)  &  1.05(-01)  &  1.05(-01)  &  1.05(-01)  &  1.05(-01) \nl
Na                &    5.37(-04) &  5.37(-04)  &  5.37(-04)  &  5.37(-04)  &  5.37(-04)  &  5.37(-04)  &  5.37(-04) \nl
Mg                &    6.05(-02) &  6.05(-02)  &  6.05(-02)  &  6.05(-02)  &  6.05(-02)  &  6.05(-02)  &  6.05(-02) \nl
Al                &    4.67(-04) &  4.67(-04)  &  4.67(-04)  &  4.67(-04)  &  4.67(-04)  &  4.67(-04)  &  4.67(-04) \nl
Si                &    8.42(-02) &  1.07(-01)  &  1.21(-01)  &  1.31(-01)  &  1.31(-01)  &  1.31(-01)  &  1.31(-01) \nl
P                 &    7.80(-05) &  7.83(-05)  &  7.86(-05)  &  7.92(-05)  &  7.93(-05)  &  7.93(-05)  &  7.94(-05) \nl
S                 &    4.16(-02) &  5.64(-02)  &  6.57(-02)  &  7.45(-02)  &  7.45(-02)  &  7.45(-02)  &  7.45(-02) \nl
Cl                &    3.46(-05) &  3.47(-05)  &  3.47(-05)  &  3.48(-05)  &  3.50(-05)  &  3.52(-05)  &  4.36(-05) \nl
Ar                &    6.93(-03) &  9.60(-03)  &  1.14(-02)  &  1.37(-02)  &  1.37(-02)  &  1.37(-02)  &  1.37(-02) \nl
K                 &    1.39(-05) &  1.40(-05)  &  1.40(-05)  &  1.40(-05)  &  1.40(-05)  &  1.40(-05)  &  1.41(-05) \nl
Ca                &    5.78(-03) &  8.06(-03)  &  9.73(-03)  &  1.25(-02)  &  1.25(-02)  &  1.26(-02)  &  1.27(-02) \nl
Sc                &    6.35(-08) &  6.61(-08)  &  6.79(-08)  &  7.21(-08)  &  1.66(-07)  &  2.77(-07)  &  7.89(-06) \nl
Ti                &    8.80(-06) &  3.14(-05)  &  5.56(-05)  &  1.24(-04)  &  1.54(-04)  &  2.08(-04)  &  2.89(-04) \nl
V                 &    3.50(-07) &  9.98(-07)  &  1.51(-06)  &  2.36(-06)  &  2.36(-06)  &  2.36(-06)  &  2.36(-06) \nl
Cr                &    6.46(-05) &  3.48(-04)  &  6.84(-04)  &  2.06(-03)  &  2.10(-03)  &  2.17(-03)  &  2.29(-03) \nl
Mn                &    1.77(-05) &  4.79(-05)  &  7.31(-05)  &  1.35(-04)  &  1.35(-04)  &  1.35(-04)  &  1.35(-04) \nl
Fe                &    1.23(-03) &  5.38(-03)  &  1.05(-02)  &  5.08(-02)  &  1.02(-01)  &  1.53(-01)  &  2.05(-01) \nl
Co                &    5.15(-08) &  5.25(-08)  &  5.31(-08)  &  7.77(-06)  &  1.75(-04)  &  6.42(-04)  &  9.46(-04) \nl
Ni                &    2.77(-05) &  4.44(-05)  &  5.72(-05)  &  1.70(-04)  &  6.72(-04)  &  9.70(-04)  &  2.39(-03) \nl
Cu                &    6.30(-14) &  6.30(-14)  &  6.30(-14)  &  6.30(-14)  &  6.77(-14)  &  9.89(-14)  &  1.73(-13) \nl
Zn                &    1.93(-13) &  1.93(-13)  &  1.93(-13)  &  3.45(-11)  &  4.95(-09)  &  2.05(-08)  &  4.84(-08) \nl
\enddata           
\end{deluxetable}

==> tablsc24.tex <==
\begin{deluxetable}{lrrrrrrrr}
%\small
\tablenum{A9}
%\tablewidth{16cm}
\tablecaption{Explosive nucleosynthesis of the $\rm 25~M_\odot~~Z=2\cdot10^{-2}$ model} 
\tablehead{
\colhead{}        & \colhead{(1)} & \colhead{(2)} & \colhead{(3)} & \colhead{(4)} & \colhead{(5)} & \colhead{(6)} & \colhead{(7)} & \colhead{(8)}
}
\startdata  
$\rm M(^{56}Ni)$  &      0.001   &     0.005   &     0.010   &     0.050   &     0.100   &     0.150   &     0.200   &     0.267   \nl
$\rm M_{ejected}$ &       22.67  &      22.71  &      22.73  &      22.80  &      22.86  &      22.92  &      22.99  &      23.07  \nl
$\rm M_{cut}$     &        2.33  &       2.29  &       2.27  &       2.20  &       2.14  &       2.08  &       2.01  &       1.93  \nl
C                 &    3.87(-01) &  3.87(-01)  &  3.87(-01)  &  3.87(-01)  &  3.87(-01)  &  3.87(-01)  &  3.87(-01)  &  3.87(-01)  \nl
N                 &    9.38(-02) &  9.38(-02)  &  9.38(-02)  &  9.38(-02)  &  9.38(-02)  &  9.38(-02)  &  9.38(-02)  &  9.38(-02)  \nl
O                 &    2.29(+00) &  2.29(+00)  &  2.29(+00)  &  2.29(+00)  &  2.29(+00)  &  2.29(+00)  &  2.29(+00)  &  2.29(+00)  \nl
F                 &    7.43(-06) &  7.43(-06)  &  7.43(-06)  &  7.43(-06)  &  7.43(-06)  &  7.43(-06)  &  7.43(-06)  &  7.43(-06)  \nl
Ne                &    4.13(-01) &  4.13(-01)  &  4.13(-01)  &  4.13(-01)  &  4.13(-01)  &  4.13(-01)  &  4.13(-01)  &  4.13(-01)  \nl
Na                &    1.43(-02) &  1.43(-02)  &  1.43(-02)  &  1.43(-02)  &  1.43(-02)  &  1.43(-02)  &  1.43(-02)  &  1.43(-02)  \nl
Mg                &    1.27(-01) &  1.27(-01)  &  1.27(-01)  &  1.27(-01)  &  1.27(-01)  &  1.27(-01)  &  1.27(-01)  &  1.27(-01)  \nl
Al                &    1.25(-02) &  1.25(-02)  &  1.25(-02)  &  1.25(-02)  &  1.25(-02)  &  1.25(-02)  &  1.25(-02)  &  1.25(-02)  \nl
Si                &    1.43(-01) &  1.62(-01)  &  1.71(-01)  &  1.77(-01)  &  1.77(-01)  &  1.77(-01)  &  1.77(-01)  &  1.77(-01)  \nl
P                 &    1.74(-03) &  1.74(-03)  &  1.74(-03)  &  1.74(-03)  &  1.74(-03)  &  1.74(-03)  &  1.74(-03)  &  1.74(-03)  \nl
S                 &    6.64(-02) &  7.84(-02)  &  8.47(-02)  &  9.05(-02)  &  9.05(-02)  &  9.05(-02)  &  9.05(-02)  &  9.05(-02)  \nl
Cl                &    3.67(-04) &  3.67(-04)  &  3.67(-04)  &  3.67(-04)  &  3.67(-04)  &  3.67(-04)  &  3.67(-04)  &  3.67(-04)  \nl
Ar                &    1.11(-02) &  1.33(-02)  &  1.46(-02)  &  1.62(-02)  &  1.63(-02)  &  1.63(-02)  &  1.63(-02)  &  1.63(-02)  \nl
K                 &    2.11(-04) &  2.11(-04)  &  2.11(-04)  &  2.11(-04)  &  2.11(-04)  &  2.12(-04)  &  2.12(-04)  &  2.12(-04)  \nl
Ca                &    5.94(-03) &  7.78(-03)  &  9.10(-03)  &  1.14(-02)  &  1.14(-02)  &  1.14(-02)  &  1.15(-02)  &  1.15(-02)  \nl
Sc                &    3.74(-06) &  3.75(-06)  &  3.75(-06)  &  3.76(-06)  &  3.76(-06)  &  3.76(-06)  &  3.76(-06)  &  3.77(-06)  \nl
Ti                &    1.09(-04) &  1.32(-04)  &  1.53(-04)  &  2.20(-04)  &  2.46(-04)  &  2.85(-04)  &  3.42(-04)  &  4.16(-04)  \nl
V                 &    1.46(-05) &  1.84(-05)  &  2.10(-05)  &  2.68(-05)  &  2.69(-05)  &  2.69(-05)  &  2.69(-05)  &  2.69(-05)  \nl
Cr                &    6.09(-04) &  9.42(-04)  &  1.28(-03)  &  2.74(-03)  &  2.78(-03)  &  2.83(-03)  &  2.91(-03)  &  3.01(-03)  \nl
Mn                &    4.30(-04) &  5.77(-04)  &  6.98(-04)  &  1.10(-03)  &  1.10(-03)  &  1.10(-03)  &  1.10(-03)  &  1.10(-03)  \nl
Fe                &    3.27(-02) &  3.87(-02)  &  4.49(-02)  &  8.77(-02)  &  1.39(-01)  &  1.91(-01)  &  2.44(-01)  &  3.13(-01)  \nl
Co                &    3.90(-04) &  3.90(-04)  &  3.91(-04)  &  4.16(-04)  &  6.86(-04)  &  1.04(-03)  &  1.60(-03)  &  2.57(-03)  \nl
Ni                &    3.33(-03) &  3.46(-03)  &  3.55(-03)  &  4.18(-03)  &  6.57(-03)  &  8.98(-03)  &  1.11(-02)  &  1.35(-02)  \nl
Cu                &    3.63(-04) &  3.63(-04)  &  3.63(-04)  &  3.63(-04)  &  3.63(-04)  &  3.63(-04)  &  3.63(-04)  &  3.63(-04)  \nl
Zn                &    8.01(-04) &  8.01(-04)  &  8.01(-04)  &  8.01(-04)  &  8.01(-04)  &  8.01(-04)  &  8.01(-04)  &  8.01(-04)  \nl
\enddata           
\end{deluxetable}



























































==> tablsc25.tex <==
\begin{deluxetable}{lrrrrrrrr}
%\small
\tablenum{A10}
%\tablewidth{16cm}
\tablecaption{Explosive nucleosynthesis of the $\rm 25~M_\odot~~Z=10^{-3}$ model} 
\tablehead{
\colhead{}        & \colhead{(1)} & \colhead{(2)} & \colhead{(3)} & \colhead{(4)} & \colhead{(5)} & \colhead{(6)} & \colhead{(7)} & \colhead{(8)}
}
\startdata  
$\rm M(^{56}Ni)$  &     0.001  &      0.005   &     0.010   &     0.050   &     0.100   &     0.150   &     0.200   &     0.287   \nl
$\rm M_{ejected}$ &      22.75 &       22.81  &      22.85  &      22.93  &      22.99  &      23.05  &      23.11  &      23.23  \nl
$\rm M_{cut}$     &       2.25 &        2.19  &       2.15  &       2.07  &       2.01  &       1.95  &       1.89  &       1.77  \nl
C                 &   4.23(-01)&   4.23(-01)  &  4.23(-01)  &  4.23(-01)  &  4.23(-01)  &  4.23(-01)  &  4.23(-01)  &  4.23(-01)  \nl
N                 &   6.45(-03)&   6.45(-03)  &  6.45(-03)  &  6.45(-03)  &  6.45(-03)  &  6.45(-03)  &  6.45(-03)  &  6.45(-03)  \nl
O                 &   1.80(+00)&   1.80(+00)  &  1.80(+00)  &  1.80(+00)  &  1.80(+00)  &  1.80(+00)  &  1.80(+00)  &  1.80(+00)  \nl
F                 &   4.99(-07)&   4.99(-07)  &  4.99(-07)  &  4.99(-07)  &  4.99(-07)  &  4.99(-07)  &  4.99(-07)  &  4.99(-07)  \nl
Ne                &   2.65(-01)&   2.65(-01)  &  2.65(-01)  &  2.65(-01)  &  2.65(-01)  &  2.65(-01)  &  2.65(-01)  &  2.65(-01)  \nl
Na                &   2.73(-03)&   2.73(-03)  &  2.73(-03)  &  2.73(-03)  &  2.73(-03)  &  2.73(-03)  &  2.73(-03)  &  2.73(-03)  \nl
Mg                &   9.41(-02)&   9.41(-02)  &  9.41(-02)  &  9.41(-02)  &  9.41(-02)  &  9.41(-02)  &  9.41(-02)  &  9.41(-02)  \nl
Al                &   1.60(-03)&   1.60(-03)  &  1.60(-03)  &  1.60(-03)  &  1.60(-03)  &  1.60(-03)  &  1.60(-03)  &  1.60(-03)  \nl
Si                &   1.19(-01)&   1.45(-01)  &  1.65(-01)  &  1.81(-01)  &  1.81(-01)  &  1.81(-01)  &  1.81(-01)  &  1.81(-01)  \nl
P                 &   1.99(-04)&   1.99(-04)  &  1.99(-04)  &  1.99(-04)  &  1.99(-04)  &  2.00(-04)  &  2.00(-04)  &  2.00(-04)  \nl
S                 &   5.68(-02)&   7.37(-02)  &  8.66(-02)  &  1.00(-01)  &  1.00(-01)  &  1.00(-01)  &  1.00(-01)  &  1.00(-01)  \nl
Cl                &   8.35(-05)&   8.36(-05)  &  8.36(-05)  &  8.37(-05)  &  8.38(-05)  &  8.41(-05)  &  8.55(-05)  &  8.89(-05)  \nl
Ar                &   8.92(-03)&   1.19(-02)  &  1.43(-02)  &  1.76(-02)  &  1.76(-02)  &  1.76(-02)  &  1.77(-02)  &  1.77(-02)  \nl
K                 &   3.62(-05)&   3.62(-05)  &  3.63(-05)  &  3.63(-05)  &  3.63(-05)  &  3.63(-05)  &  3.63(-05)  &  3.65(-05)  \nl
Ca                &   6.63(-03)&   9.15(-03)  &  1.12(-02)  &  1.52(-02)  &  1.53(-02)  &  1.53(-02)  &  1.54(-02)  &  1.55(-02)  \nl
Sc                &   2.04(-07)&   2.07(-07)  &  2.10(-07)  &  2.15(-07)  &  2.60(-07)  &  3.82(-07)  &  1.09(-06)  &  3.27(-06)  \nl
Ti                &   1.27(-05)&   3.60(-05)  &  6.27(-05)  &  1.59(-04)  &  1.80(-04)  &  2.20(-04)  &  2.73(-04)  &  3.73(-04)  \nl
V                 &   1.11(-06)&   2.18(-06)  &  3.22(-06)  &  5.39(-06)  &  5.39(-06)  &  5.39(-06)  &  5.39(-06)  &  5.39(-06)  \nl
Cr                &   9.31(-05)&   3.84(-04)  &  7.42(-04)  &  2.56(-03)  &  2.59(-03)  &  2.65(-03)  &  2.72(-03)  &  2.86(-03)  \nl
Mn                &   4.35(-05)&   9.12(-05)  &  1.38(-04)  &  2.82(-04)  &  2.82(-04)  &  2.82(-04)  &  2.82(-04)  &  2.82(-04)  \nl
Fe                &   2.92(-03)&   7.24(-03)  &  1.25(-02)  &  5.31(-02)  &  1.04(-01)  &  1.55(-01)  &  2.06(-01)  &  2.96(-01)  \nl
Co                &   2.16(-05)&   2.16(-05)  &  2.16(-05)  &  2.75(-05)  &  1.46(-04)  &  2.98(-04)  &  4.77(-04)  &  1.38(-03)  \nl
Ni                &   1.74(-04)&   2.00(-04)  &  2.23(-04)  &  3.00(-04)  &  7.20(-04)  &  1.26(-03)  &  2.10(-03)  &  4.32(-03)  \nl
Cu                &   6.69(-06)&   6.69(-06)  &  6.69(-06)  &  6.69(-06)  &  6.69(-06)  &  6.69(-06)  &  6.69(-06)  &  6.69(-06)  \nl
Zn                &   1.53(-05)&   1.53(-05)  &  1.53(-05)  &  1.53(-05)  &  1.53(-05)  &  1.53(-05)  &  1.53(-05)  &  1.54(-05)  \nl
\enddata           
\end{deluxetable}

















































==> tablsc26.tex <==
\begin{deluxetable}{lrrrrrrrr}
%\small
\tablenum{A11}
%\tablewidth{16cm}
\tablecaption{Explosive nucleosynthesis of the $\rm 25~M_\odot~~Z=0$ model} 
\tablehead{
\colhead{}        & \colhead{(1)} & \colhead{(2)} & \colhead{(3)} & \colhead{(4)} & \colhead{(5)} & \colhead{(6)} & \colhead{(7)} & \colhead{(8)}
}
\startdata  
$\rm M(^{56}Ni)$  &      0.001   &     0.005   &     0.010   &     0.050   &     0.100   &     0.150   &     0.200   &     0.413    \nl
$\rm M_{ejected}$ &       22.37  &      22.43  &      22.48  &      22.59  &      22.64  &      22.70  &      22.75  &      23.01   \nl
$\rm M_{cut}$     &        2.63  &       2.57  &       2.52  &       2.41  &       2.36  &       2.30  &       2.25  &       1.99   \nl
C                 &    4.71(-01) &  4.71(-01)  &  4.71(-01)  &  4.71(-01)  &  4.71(-01)  &  4.71(-01)  &  4.71(-01)  &  4.71(-01)   \nl
N                 &    3.03(-03) &  3.03(-03)  &  3.03(-03)  &  3.03(-03)  &  3.03(-03)  &  3.03(-03)  &  3.03(-03)  &  3.03(-03)   \nl
O                 &    2.13(+00) &  2.13(+00)  &  2.13(+00)  &  2.13(+00)  &  2.13(+00)  &  2.13(+00)  &  2.13(+00)  &  2.13(+00)   \nl
F                 &    1.88(-10) &  1.88(-10)  &  1.88(-10)  &  1.88(-10)  &  1.88(-10)  &  1.88(-10)  &  1.88(-10)  &  1.88(-10)   \nl
Ne                &    2.58(-01) &  2.58(-01)  &  2.58(-01)  &  2.58(-01)  &  2.58(-01)  &  2.58(-01)  &  2.58(-01)  &  2.58(-01)   \nl
Na                &    2.60(-04) &  2.60(-04)  &  2.60(-04)  &  2.60(-04)  &  2.60(-04)  &  2.60(-04)  &  2.60(-04)  &  2.60(-04)   \nl
Mg                &    1.09(-01) &  1.09(-01)  &  1.09(-01)  &  1.09(-01)  &  1.09(-01)  &  1.09(-01)  &  1.09(-01)  &  1.09(-01)   \nl
Al                &    4.31(-04) &  4.31(-04)  &  4.31(-04)  &  4.31(-04)  &  4.31(-04)  &  4.31(-04)  &  4.31(-04)  &  4.31(-04)   \nl
Si                &    1.39(-01) &  1.70(-01)  &  1.94(-01)  &  2.24(-01)  &  2.24(-01)  &  2.24(-01)  &  2.24(-01)  &  2.24(-01)   \nl
P                 &    7.78(-05) &  7.83(-05)  &  7.88(-05)  &  8.05(-05)  &  8.06(-05)  &  8.06(-05)  &  8.07(-05)  &  8.09(-05)   \nl
S                 &    7.34(-02) &  9.33(-02)  &  1.08(-01)  &  1.32(-01)  &  1.32(-01)  &  1.32(-01)  &  1.32(-01)  &  1.32(-01)   \nl
Cl                &    5.04(-05) &  5.05(-05)  &  5.05(-05)  &  5.06(-05)  &  5.07(-05)  &  5.11(-05)  &  5.17(-05)  &  6.63(-05)   \nl
Ar                &    1.26(-02) &  1.63(-02)  &  1.90(-02)  &  2.44(-02)  &  2.47(-02)  &  2.47(-02)  &  2.47(-02)  &  2.48(-02)   \nl
K                 &    2.18(-05) &  2.18(-05)  &  2.18(-05)  &  2.19(-05)  &  2.19(-05)  &  2.19(-05)  &  2.19(-05)  &  2.21(-05)   \nl
Ca                &    1.07(-02) &  1.41(-02)  &  1.64(-02)  &  2.24(-02)  &  2.30(-02)  &  2.30(-02)  &  2.30(-02)  &  2.32(-02)   \nl
Sc                &    1.42(-07) &  1.46(-07)  &  1.48(-07)  &  1.55(-07)  &  1.74(-07)  &  3.53(-07)  &  6.53(-07)  &  1.50(-05)   \nl
Ti                &    1.25(-05) &  3.73(-05)  &  6.52(-05)  &  1.92(-04)  &  2.22(-04)  &  2.48(-04)  &  2.78(-04)  &  4.59(-04)   \nl
V                 &    3.40(-07) &  9.05(-07)  &  1.51(-06)  &  3.00(-06)  &  3.21(-06)  &  3.21(-06)  &  3.21(-06)  &  3.21(-06)   \nl
Cr                &    6.77(-05) &  3.50(-04)  &  7.14(-04)  &  2.91(-03)  &  3.72(-03)  &  3.75(-03)  &  3.80(-03)  &  4.05(-03)   \nl
Mn                &    1.76(-05) &  4.55(-05)  &  7.46(-05)  &  1.64(-04)  &  1.87(-04)  &  1.87(-04)  &  1.87(-04)  &  1.87(-04)   \nl
Fe                &    1.24(-03) &  5.37(-03)  &  1.05(-02)  &  5.08(-02)  &  1.01(-01)  &  1.52(-01)  &  2.02(-01)  &  4.18(-01)   \nl
Co                &    1.37(-07) &  1.38(-07)  &  1.38(-07)  &  1.39(-07)  &  2.15(-05)  &  7.05(-05)  &  1.25(-04)  &  5.37(-04)   \nl
Ni                &    3.81(-05) &  5.46(-05)  &  6.89(-05)  &  1.10(-04)  &  3.64(-04)  &  1.13(-03)  &  1.93(-03)  &  6.58(-03)   \nl
Cu                &    3.27(-13) &  3.27(-13)  &  3.27(-13)  &  3.27(-13)  &  3.27(-13)  &  3.28(-13)  &  3.29(-13)  &  3.60(-13)   \nl
Zn                &    1.08(-12) &  1.08(-12)  &  1.08(-12)  &  1.08(-12)  &  2.19(-10)  &  2.19(-09)  &  5.15(-09)  &  3.71(-08)   \nl
\enddata           
\end{deluxetable}








































==> tablsc3.tex <==
\begin{deluxetable}{lcccc}
%\small
\tablenum{3}
\tablewidth{12cm}
\tablecaption{Most abundant nuclear species at the center left
by the various nuclear burnings for $\rm 13~M_\odot$, $\rm 15~M_\odot$, $\rm 20~M_\odot$ and $\rm 25~M_\odot$ models.}
\tablehead{
\colhead{Isotope}   &
\colhead{$\rm 13~M_\odot$}    &
\colhead{$\rm 15~M_\odot$}    &
\colhead{$\rm 20~M_\odot$}    &
\colhead{$\rm 25~M_\odot$}    
}
\startdata  
\cutinhead{H Burning}
% HYDROGEN
$\rm ^{4}He$               &     0.981        &     0.980        &    0.980           & 0.980     \nl
$\rm ^{14}N$               &     1.32(-2)     &     1.33(-2)     &    1.33(-2)        & 1.33(-2)  \nl
$\rm ^{20}Ne$              &     1.67(-3)     &     1.66(-3)     &    1.66(-3)        & 1.66(-3)  \nl
$\rm ^{21}Ne$              &     8.40(-8)     &     6.98(-8)     &    5.35(-8)        & 4.58(-8)  \nl
$\rm ^{22}Ne$              &     1.01(-5)     &     1.21(-5)     &    1.77(-5)        & 2.32(-5)  \nl
$\rm ^{23}Na$              &     1.90(-4)     &     1.90(-4)     &    1.88(-4)        & 1.85(-4)  \nl
$\rm ^{24}Mg$              &     5.35(-4)     &     5.35(-4)     &    5.35(-4)        & 5.35(-4)  \nl
$\rm ^{25}Mg$              &     6.35(-7)     &     7.28(-9)     &    2.21(-9)        & 1.00(-9)  \nl
$\rm ^{26}Mg$              &     1.52(-4)     &     1.53(-4)     &    1.53(-4)        & 1.53(-4)  \nl
$\rm ^{26}Al$              &     1.58(-6)     &     1.58(-7)     &    2.64(-7)        & 4.16(-7)  \nl
$\rm ^{27}Al$              &     6.03(-5)     &     6.03(-5)     &    6.04(-5)        & 6.05(-5)  \nl
\cutinhead{He Burning}                                            
$\rm ^{12}C$               &    0.257         &    0.195         &     0.171          &  0.179    \nl
$\rm ^{16}O$               &    0.717         &    0.777         &     0.800          &  0.790    \nl
$\rm ^{20}Ne$              &    1.66(-3)      &    1.90(-3)      &     2.83(-3)       &  3.71(-3) \nl
$\rm ^{22}Ne$              &    1.80(-2)      &    1.61(-2)      &     1.30(-2)       &  1.16(-2) \nl
$\rm ^{23}Na$              &    2.04(-4)      &    2.15(-4)      &     2.22(-4)       &  2.23(-4) \nl
$\rm ^{24}Mg$              &    4.57(-4)      &    4.41(-4)      &     4.63(-3)       &  4.96(-3) \nl
$\rm ^{25}Mg$              &    1.62(-3)      &    2.84(-3)      &     4.49(-3)       &  5.20(-3) \nl
$\rm ^{26}Mg$              &    1.65(-3)      &    2.29(-3)      &     4.91(-3)       &  5.80(-3) \nl
$\rm ^{56}Fe$              &    6.06(-4)      &    3.76(-4)      &     2.05(-4)       &  1.61(-4) \nl
$\rm ^{58}Fe$              &    3.34(-4)      &    4.41(-4)      &     4.15(-4)       &  3.81(-4) \nl
$\eta_{\rm c}$             &    1.987(-3)     &    1.980(-3)     &     1.936(-3)      &  1.917(-3)\nl
$Y_{\rm e}$                &    0.4990        &    0.4990        &     0.4990         &  0.4990   \nl
\cutinhead{C Burning}                                             
$\rm ^{16}O$               &    0.614         &    0.700         &     0.730          &  0.710    \nl
$\rm ^{20}Ne$              &    0.294         &    0.230         &     0.200          &  0.220    \nl
$\rm ^{23}Na$              &    2.34(-2)      &    1.82(-2)      &     1.72(-2)       &  1.72(-2) \nl
$\rm ^{24}Mg$              &    2.61(-2)      &    1.70(-2)      &     1.27(-2)       &  1.42(-2) \nl
$\eta_{\rm c}$             &    2.839(-3)     &    2.490(-3)     &     2.215(-3)      &  2.168(-3)\nl
$Y_{\rm e}$                &    0.4986        &    0.4987        &     0.4989         &  0.4989   \nl
\tablebreak                                                       
\cutinhead{Ne Burning}                                            
$\rm ^{16}O$               &    0.768         &    0.811         &     0.830          &  0.826    \nl
$\rm ^{24}Mg$              &    8.16(-2)      &    4.90(-2)      &     4.37(-2)       &  4.71(-2) \nl
$\rm ^{28}Si$              &    8.22(-2)      &    7.03(-2)      &     6.35(-2)       &  6.35(-2) \nl
$\rm ^{29}Si$              &    2.07(-2)      &    1.74(-2)      &     1.54(-2)       &  1.51(-2) \nl
$\rm ^{30}Si$              &    9.24(-3)      &    1.09(-2)      &     1.07(-2)       &  1.14(-2) \nl
$\rm ^{31}P$               &    6.17(-3)      &    1.24(-2)      &     1.02(-2)       &  7.77(-3) \nl
$\rm ^{32}S$               &    9.48(-2)      &    1.33(-2)      &     1.34(-2)       &  1.52(-2) \nl
$\eta_{\rm c}$             &    2.685(-3)     &    2.543(-3)     &     2.272(-3)      &  2.156(-3)\nl
$Y_{\rm e}$                &    0.4987        &    0.4987        &     0.4989         &  0.4989   \nl
\cutinhead{O Burning}                                             
$\rm ^{28}Si$              &    0.300         &    0.343         &     0.401          &  0.428    \nl
$\rm ^{30}Si$              &    0.268         &    5.90(-3)      &     1.30(-3)       &  8.70(-4) \nl
$\rm ^{32}S$               &    2.45(-2)      &    0.115         &     0.253          &  0.288    \nl
$\rm ^{34}S$               &    0.356         &    0.217         &     7.43(-2)       &  5.32(-2) \nl
$\rm ^{36}Ar$              &    1.48(-4)      &    6.22(-3)      &     3.76(-2)       &  4.53(-2) \nl
$\rm ^{38}Ar$              &    3.77(-2)      &    0.210         &     0.151          &  0.115    \nl
$\rm ^{40}Ca$              &    9.57(-7)      &    2.62(-3)      &     3.56(-2)       &  4.54(-2) \nl
$\eta_{\rm c}$             &    4.116(-2)     &    2.447(-2)     &     1.419(-2)      &  9.983(-3)\nl
$Y_{\rm e}$                &    0.4794        &    0.4878        &     0.4929         &  0.4950   \nl
\cutinhead{Si Burning Radiative}             
$\rm ^{28}Si$              &    4.46(-3)      &    4.73(-2)      &     0.364          &  0.430    \nl
$\rm ^{30}Si$              &    0.818         &    0.675         &     0.249          &  0.197    \nl
$\rm ^{32}S$               &    1.24(-5)      &    3.00(-4)      &     6.92(-3)       &  9.93(-3) \nl
$\rm ^{34}S$               &    7.98(-2)      &    0.166         &     0.189          &  0.165    \nl
$\rm ^{38}Ar$              &    5.98(-4)      &    2.74(-3)      &     9.60(-3)       &  9.92(-3) \nl
$\rm ^{50}Ti$              &    6.17(-2)      &    1.21(-2)      &     3.99(-4)       &  2.79(-4) \nl
$\rm ^{52}Cr$              &    8.43(-3)      &    7.01(-2)      &     0.121          &  0.120    \nl
$\eta_{\rm c}$             &    6.994(-2)     &    6.423(-2)     &     4.100(-2)      &  3.653(-2)\nl
$Y_{\rm e}$                &    0.4650        &    0.4679        &     0.4795         &  0.4817   \nl
\cutinhead{Si Burning Convective (first phase)}
$\rm ^{28}Si$              &    0.160         &    0.347         &     0.442          &  0.461    \nl
$\rm ^{30}Si$              &    0.196         &    0.146         &     4.31(-3)       &  2.25(-3) \nl
$\rm ^{32}S$               &    3.63(-3)      &    1.14(-2)      &     6.09(-2)       &  7.41(-2) \nl
$\rm ^{34}S$               &    0.145         &    0.151         &     1.42(-2)       &  8.83(-3) \nl
$\rm ^{38}Ar$              &    8.23(-3)      &    1.23(-2)      &     4.50(-3)       &  3.27(-3) \nl
$\rm ^{52}Cr$              &    0.338         &    0.206         &     9.72(-2)       &  6.02(-2) \nl
$\rm ^{54}Fe$              &    5.00(-4)      &    2.61(-3)      &     0.132          &  3.42(-2) \nl
$\rm ^{56}Fe$              &    1.09(-1)      &    9.29(-2)      &     0.154          &  0.112    \nl
\tablebreak                                                       
\cutinhead{Si Burning (final abundances)}   
$\rm ^{50}Ti$              &    4.21(-2)      &    1.03(-2)      &     1.21(-4)       &  1.10(-4) \nl
$\rm ^{51}V $              &    2.47(-2)      &    1.24(-2)      &     1.25(-3)       &  1.19(-3) \nl
$\rm ^{52}Cr$              &    0.431         &    0.437         &     0.258          &  0.246    \nl
$\rm ^{53}Cr$              &    3.87(-2)      &    2.35(-2)      &     3.51(-3)       &  3.41(-3) \nl
$\rm ^{54}Cr$              &    7.40(-2)      &    2.66(-2)      &     7.75(-4)       &  7.42(-4) \nl
$\rm ^{55}Mn$              &    3.98(-2)      &    2.93(-2)      &     7.06(-3)       &  7.06(-3) \nl
$\rm ^{54}Fe$              &    1.53(-4)      &    6.56(-4)      &     3.05(-2)       &  3.24(-2) \nl
$\rm ^{55}Fe$              &    1.24(-3)      &    3.15(-3)      &     3.04(-2)       &  3.20(-2) \nl
$\rm ^{56}Fe$              &    0.268         &    0.398         &     0.600          &  0.605    \nl
$\rm ^{57}Fe$              &    1.88(-2)      &    1.68(-2)      &     6.57(-3)       &  6.76(-3) \nl
$\rm ^{58}Fe$              &    4.16(-2)      &    2.20(-2)      &     1.59(-3)       &  1.60(-3) \nl
$\eta_{\rm c}$             &    8.283(-2)     &    7.731(-2)     &     7.100(-2)      &  7.053(-2)\nl
$Y_{\rm e}$                &    0.4586        &    0.4613        &     0.4645         &  0.4647   \nl
\enddata        
\end{deluxetable}


==> tablsc4.tex <==
\begin{deluxetable}{lccccc}
%\small
\tablenum{4}
\tablewidth{12cm}
\tablecaption{Final surface abundances 
for $\rm 13~M_\odot$, $\rm 15~M_\odot$, $\rm 20~M_\odot$ and $\rm 25~M_\odot$ models.}
\tablehead{
\colhead{Isotope}   &
\colhead{Solar}    &
\colhead{$\rm 13~M_\odot$}    &
\colhead{$\rm 15~M_\odot$}    &
\colhead{$\rm 20~M_\odot$}    &
\colhead{$\rm 25~M_\odot$}    
}
\startdata  
$\rm ^{1}H$   &   6.95(-01) & 6.49(-01)  & 6.38(-01)  & 6.09(-01)  & 5.93(-01)           \nl
$\rm ^{3}He$  &   3.04(-05) & 2.20(-05)  & 2.06(-05)  & 1.70(-05)  & 1.61(-05)           \nl
$\rm ^{4}He$  &   2.85(-01) & 3.31(-01)  & 3.42(-01)  & 3.71(-01)  & 3.87(-01)           \nl
$\rm ^{12}C$  &   3.46(-03) & 2.20(-03)  & 2.19(-03)  & 2.02(-03)  & 1.97(-03)           \nl
$\rm ^{13}C$  &   4.16(-05) & 1.25(-04)  & 2.36(-05)  & 2.23(-05)  & 2.19(-05)           \nl
$\rm ^{14}N$  &   1.02(-03) & 3.54(-03)  & 3.88(-03)  & 4.81(-03)  & 5.21(-03)           \nl
$\rm ^{15}N$  &   4.03(-06) & 1.82(-06)  & 1.82(-06)  & 1.78(-06)  & 1.75(-06)           \nl
$\rm ^{16}O$  &   1.00(-02) & 8.72(-03)  & 8.48(-03)  & 7.64(-03)  & 7.26(-03)           \nl
$\rm ^{17}O$  &   4.04(-06) & 1.17(-05)  & 9.62(-06)  & 8.31(-06)  & 6.90(-06)           \nl
$\rm ^{18}O$  &   2.25(-05) & 1.54(-05)  & 1.50(-05)  & 1.33(-05)  & 1.27(-05)           \nl
$\rm ^{19}F$  &   4.21(-07) & 3.43(-07)  & 3.31(-07)  & 2.65(-07)  & 2.49(-07)           \nl
$\rm ^{20}Ne$ &   1.68(-03) & 1.68(-03)  & 1.68(-03)  & 1.68(-03)  & 1.68(-03)           \nl
$\rm ^{21}Ne$ &   4.29(-06) & 4.00(-06)  & 3.80(-06)  & 2.97(-06)  & 2.72(-06)           \nl
$\rm ^{22}Ne$ &   1.35(-04) & 1.16(-04)  & 1.14(-04)  & 1.08(-04)  & 1.07(-04)           \nl
$\rm ^{23}Na$ &   3.47(-05) & 5.67(-05)  & 5.95(-05)  & 6.77(-05)  & 7.01(-05)           \nl
$\rm ^{24}Mg$ &   5.35(-04) & 5.35(-04)  & 5.35(-04)  & 5.35(-04)  & 5.35(-04)           \nl
$\rm ^{25}Mg$ &   7.03(-05) & 6.19(-05)  & 5.83(-05)  & 5.04(-05)  & 4.71(-05)           \nl
$\rm ^{26}Mg$ &   8.07(-05) & 8.94(-05)  & 9.33(-05)  & 1.00(-04)  & 1.02(-04)           \nl
$\rm ^{26}Al$ &   0.00(+00) & 1.20(-08)  & 2.27(-08)  & 8.19(-07)  & 1.42(-06)           \nl
$\rm ^{27}Al$ &   6.03(-05) & 6.03(-05)  & 6.03(-05)  & 6.03(-05)  & 6.03(-05)           \nl
\enddata        
\end{deluxetable}


==> tablsc5.tex <==
\begin{deluxetable}{lcccc}
\tablenum{5}
\tablecaption{Selected properties of the C convective shells 
for the $\rm 15~M_\odot$ model.}
\tablehead{
                 &
\colhead{(1)}    &
\colhead{(2)}    &
\colhead{(3)}    &
\colhead{(4)}    
}
\startdata  
$\rm ^{12}C$                      & 0.160-3.96(-2)    & 0.150-3.66(-2)    & 0.168-2.89(-2)    & 5.00(-2)-4.82(-3)    \nl
$\rm ^{20}Ne$                     & 3.61(-2)-0.197    & 4.77(-2)-0.203    & 3.39(-2)-0.212    & 0.186-0.222          \nl
$\rm ^{22}Ne$                     & 1.38(-2)-7.89(-3) & 1.29(-2)-6.86(-3) & 1.31(-2)-5.25(-3) & 6.39(-3)-1.66(-3)    \nl
$\rm ^{23}Na$                     & 7.01(-3)-1.57(-2) & 7.56(-3)-1.47(-2) & 6.04(-3)-1.34(-2) & 1.26(-2)-1.01(-2)    \nl
$\rm ^{24}Mg$                     & 1.96(-3)-1.37(-2) & 2.38(-3)-1.52(-2) & 1.53(-3)-1.83(-2) & 1.49(-2)-3.08(-2)    \nl
$\rm ^{25}Mg$                     & 2.99(-3)-7.83(-3) & 3.55(-3)-8.53(-3) & 3.51(-3)-9.93(-3) & 8.99(-3)-1.38(-2)    \nl
$\rm ^{27}Al$                     & 1.58(-3)-3.98(-3) & 1.89(-3)-4.08(-3) & 1.56(-3)-4.33(-3) & 3.90(-3)-5.76(-3)    \nl
$n_{\rm n}$                       & 2.16(8)-5.90(7)   & 7.51(8)-2.75(8)   & 9.36(9)-1.84(9)   & 2.00(12)-5.70(11)    \nl
$T$                               &  7.8(8)-8.8(8)    &   8.9(8)-9.5(8)   &  9.8(8)-1.1(9)    &  1.2(9)-1.3(9)       \nl
$\rho$                            &  3.11(5)-3.36(5)  & 2.50(5)-2.90(5)   & 2.04(5)-2.25(5)   & 2.28(5)-2.28(5)      \nl                    
$\rm ^{22}Ne(\alpha,n)^{25}Mg$    &  1.6(19)          &    1.6(20)        &    2.6(15)        &      8.2(17)         \nl
$\rm ^{20}Ne(n,\gamma)^{21}Ne$    &  8.1(18)          &    1.3(20)        &    2.4(15)        &      9.1(17)         \nl
$\rm ^{25}Mg(n,\gamma)^{26}Mg$    &  2.3(18)          &    2.2(19)        &    4.1(14)        &      2.3(17)         \nl
$\rm ^{23}Na(n,\gamma)^{24}Na$    &  2.3(18)          &    1.6(19)        &    2.5(14)        &      6.8(16)         \nl
$\rm ^{21}Ne(\alpha,n)^{24}Mg$    &  1.3(18)          &    5.2(19)        &    1.2(15)        &      8.0(17)         \nl
$\rm ^{24}Mg(n,\gamma)^{25}Mg$    &  1.1(18)          &    2.0(19)        &    4.2(14)        &      2.7(17)         \nl
$\rm ^{27}Al(n,\gamma)^{28}Al$    &  7.5(17)          &    5.9(18)        &    1.0(14)        &      4.4(16)         \nl
maximum integrated flux           &  4.0(20)          &    2.4(21)        &    3.2(16)        &      6.2(18)         \nl
\enddata        
\end{deluxetable}


==> tablsc6.tex <==
\begin{deluxetable}{lcc}
\tablenum{6}
\tablewidth{10cm}
\tablecaption{Selected properties of the C convective shells 
for $\rm 25~M_\odot$ model.}
\tablehead{
                     &
\colhead{(1)}    &
\colhead{(2)}    
}
\startdata  
$\rm ^{12}C$                      & 0.110-1.63(-2)    & 0.155-2.04(-2)    \nl
$\rm ^{20}Ne$                     & 9.09(-2)-0.208    & 3.21(-2)-0.195    \nl
$\rm ^{22}Ne$                     & 6.61(-3)-2.48(-3) & 9.04(-3)-1.31(-3) \nl
$\rm ^{23}Na$                     & 9.64(-3)-1.17(-2) & 4.94(-3)-9.26(-3) \nl
$\rm ^{24}Mg$                     & 4.53(-3)-1.99(-2) & 1.46(-3)-2.26(-2) \nl
$\rm ^{25}Mg$                     & 6.72(-3)-1.03(-2) & 5.85(-3)-1.14(-2) \nl
$\rm ^{27}Al$                     & 4.19(-3)-6.15(-3) & 2.10(-3)-6.25(-3) \nl
$n_{\rm n}$                       & 1.11(11)-2.76(10) & 4.03(12)-1.10(12) \nl
$T$                               & 1.03(9)-1.23(9)   & 1.07(9)-1.39(9)   \nl
$\rho$                            &  1.73(5)-1.24(5)  & 1.14(5)-1.66(5)   \nl                    
$\rm ^{22}Ne(\alpha,n)^{25}Mg$    &  2.1(15)          &    1.0(17)        \nl
$\rm ^{20}Ne(n,\gamma)^{21}Ne$    &  2.1(15)          &    9.4(16)        \nl
$\rm ^{21}Ne(\alpha,n)^{24}Mg$    &  1.4(15)          &    7.0(16)        \nl
$\rm ^{25}Mg(n,\gamma)^{26}Mg$    &  4.4(14)          &    2.7(16)        \nl
$\rm ^{24}Mg(n,\gamma)^{25}Mg$    &  3.6(14)          &    1.8(16)        \nl
$\rm ^{23}Na(n,\gamma)^{24}Na$    &  2.3(14)          &    9.5(15)        \nl
$\rm ^{27}Al(n,\gamma)^{28}Al$    &  1.5(14)          &    6.7(15)        \nl
maximum integrated flux           &  2.9(16)          &    9.4(17)        \nl
\enddata        
\end{deluxetable}


==> tablsc7.tex <==
\begin{deluxetable}{lcc}
%\small
\tablenum{7}
\tablewidth{10cm}
\tablecaption{Integrated flux of the ost efficient weak interactions during central O burning
for $\rm 15~M_\odot$ and $\rm 25~M_\odot$.}
\tablehead{
\colhead{Reaction}   &
\colhead{$\rm 15~M_\odot$}    &
\colhead{$\rm 25~M_\odot$}    
}
\startdata  
$\rm ^{31}S(\beta^{+})^{31}P$      &     6.7(19)      & 6.4(16)   \nl
\tablevspace{0.2cm}
$\rm ^{33}S(e^{-},\nu)^{33}P$      &     1.2(19)      & 3.0(15)   \nl
\tablevspace{0.2cm}
$\rm ^{30}P(e^{-},\nu)^{30}Si$     &     3.7(18)      & 9.8(14)   \nl
\tablevspace{0.2cm}
$\rm ^{37}Ar(e^{-},\nu)^{37}Cl$    &     3.1(18)      & 2.8(15)   \nl
\tablevspace{0.2cm}
\cline{1-3}
\tablevspace{0.2cm}
maximum integrated flux            &   5.4(21)        &  9.9(19)  \nl
\tablevspace{0.2cm}
$Y_{\rm e}$                        &   0.488          &  0.495    \nl
\enddata        
\end{deluxetable}


==> tablsc8.tex <==
\begin{deluxetable}{lccclcc}
%\small
\tablecolumns{7}
\tablenum{8}
\tablewidth{15cm}
\tablecaption{Most efficient weak interactions during central Si burning and beyond
for $\rm 15~M_\odot$ and $\rm 25~M_\odot$.}
\tablehead{
\colhead{}  & \multicolumn{2}{c}{$\rm 15~M_\odot$} & \colhead{} & \colhead{} & \multicolumn{2}{c}{$\rm 25~M_\odot$} \\
\cline{2-3} \cline{6-7} \\
\colhead{Reaction}   &
\colhead{Int. Eff. Flux}    &
\colhead{$\varphi$}    &
\colhead{} &
\colhead{Reaction} &
\colhead{Int. Eff. Flux}    &
\colhead{$\varphi$}    
}
\startdata  
\cutinhead{Convective Si burning}
$\rm ^{53}Mn(e^{-},\nu)^{53}Cr$ & 5.87(+16)& 0.999 & & $\rm ^{55}Fe(e^{-},\nu)^{55}Mn$ &  9.34(+16)& 0.999 \nl  
$\rm ^{55}Fe(e^{-},\nu)^{55}Mn$ & 4.36(+16)& 0.998 & & $\rm ^{53}Mn(e^{-},\nu)^{53}Cr$ &  7.63(+16)& 0.999 \nl  
$\rm ^{33}S (e^{-},\nu)^{33}P $ & 1.15(+16)& 0.999 & & $\rm ^{54}Fe(e^{-},\nu)^{54}Mn$ &  5.08(+16)& 0.999 \nl  
$\rm ^{54}Mn(e^{-},\nu)^{54}Cr$ & 9.29(+15)& 0.998 & & $\rm ^{55}Co(e^{-},\nu)^{55}Fe$ &  2.78(+16)& 0.999 \nl  
$\rm ^{51}Cr(e^{-},\nu)^{51}V $ & 7.68(+15)& 0.999 & & $\rm ^{56}Co(e^{-},\nu)^{56}Fe$ &  2.21(+16)& 0.999 \nl  
$\rm ^{54}Fe(e^{-},\nu)^{54}Mn$ & 7.25(+15)& 0.999 & & $\rm ^{57}Co(e^{-},\nu)^{57}Fe$ &  2.09(+16)& 0.999 \nl  
$\rm ^{57}Co(e^{-},\nu)^{57}Fe$ & 5.18(+15)& 0.999 & & $\rm ^{51}Cr(e^{-},\nu)^{51}V $ &  7.82(+15)& 0.999 \nl  
$\rm ^{35}Cl(e^{-},\nu)^{35}S $ & 3.58(+15)& 0.999 & & $\rm ^{54}Mn(e^{-},\nu)^{54}Cr$ &  5.29(+15)& 0.999 \nl  
$\rm ^{31}P (e^{-},\nu)^{31}Si$ & 2.52(+15)& 0.998 & & $\rm ^{33}S (e^{-},\nu)^{33}P $ &  3.28(+15)& 0.999 \nl  
$\rm ^{32}S (e^{-},\nu)^{32}P $ & 1.53(+15)& 0.986 & & $\rm ^{59}Ni(e^{-},\nu)^{59}Co$ &  3.16(+15)& 0.999 \nl  
$\rm ^{56}Co(e^{-},\nu)^{56}Fe$ & 1.21(+15)& 0.999 & & $\rm ^{50}Cr(e^{-},\nu)^{50}V $ &  2.73(+15)& 0.999 \nl  
$\rm ^{56}Fe(e^{-},\nu)^{56}Mn$ & 1.10(+15)& 0.989 & & $\rm ^{35}Cl(e^{-},\nu)^{35}S $ &  2.61(+15)& 0.999 \nl  
$\rm ^{50}Cr(e^{-},\nu)^{50}V $ & 9.50(+14)& 0.999 & & $\rm ^{58}Ni(e^{-},\nu)^{58}Co$ &  1.90(+15)& 0.999 \nl       
$\rm ^{52}Cr(e^{-},\nu)^{52}V $ & 8.81(+14)& 0.989 & & $\rm ^{53}Fe(e^{-},\nu)^{53}Mn$ &  1.85(+15)& 0.999 \nl  
$\rm ^{58}Co(e^{-},\nu)^{58}Fe$ & 6.14(+14)& 0.999 & & $\rm ^{32}S (e^{-},\nu)^{32}P $ &  1.55(+15)& 0.998 \nl  
$\rm ^{49}V (e^{-},\nu)^{49}Ti$ & 6.13(+14)& 0.999 & & $\rm ^{52}Mn(e^{-},\nu)^{52}Cr$ &  1.43(+15)& 0.999 \nl  
$\rm ^{30}P (e^{-},\nu)^{30}Si$ & 6.02(+14)& 0.999 & & $\rm ^{58}Co(e^{-},\nu)^{58}Fe$ &  1.11(+15)& 0.999 \nl  
$\rm ^{37}Ar(e^{-},\nu)^{37}Cl$ & 5.18(+14)& 0.999 & & $\rm ^{56}Fe(e^{-},\nu)^{56}Mn$ &  7.71(+14)& 0.996 \nl    
\cline{1-7}\nl
$\rm ^{31}P (\alpha,p )^{30}Si$\tablenotemark{a} & 1.24(+20)& 3.84(-4)& & $\rm ^{56}Fe(n,\gamma)^{57}Fe$\tablenotemark{a} & 1.97(+20)& 1.91(-4)\nl  
\cutinhead{From Si exhaustion up to NSE}
$\rm ^{53}Mn(e^{-},\nu)^{53}Cr$ & 6.82(+16)& 0.997 & & $\rm ^{55}Fe(e^{-},\nu)^{55}Mn$ &  1.33(+15)& 0.933 \nl 
$\rm ^{55}Fe(e^{-},\nu)^{55}Mn$ & 5.61(+16)& 0.990 & & $\rm ^{53}Mn(e^{-},\nu)^{53}Cr$ &  8.19(+14)& 0.975 \nl 
$\rm ^{54}Mn(e^{-},\nu)^{54}Cr$ & 1.29(+16)& 0.979 & & $\rm ^{54}Mn(e^{-},\nu)^{54}Cr$ &  5.90(+14)& 0.935 \nl 
$\rm ^{54}Fe(e^{-},\nu)^{54}Mn$ & 9.20(+15)& 0.999 & & $\rm ^{57}Co(e^{-},\nu)^{57}Fe$ &  3.88(+14)& 0.968 \nl 
$\rm ^{51}Cr(e^{-},\nu)^{51}V $ & 8.96(+15)& 0.999 & & $\rm ^{58}Co(e^{-},\nu)^{58}Fe$ &  2.31(+14)& 0.984 \nl 
$\rm ^{57}Co(e^{-},\nu)^{57}Fe$ & 8.24(+15)& 0.996 & & $\rm ^{54}Fe(e^{-},\nu)^{54}Mn$ &  1.17(+14)& 0.989 \nl 
$\rm ^{56}Co(e^{-},\nu)^{56}Fe$ & 1.99(+15)& 0.999 & & $\rm ^{56}Co(e^{-},\nu)^{56}Fe$ &  8.29(+13)& 0.999 \nl 
$\rm ^{58}Co(e^{-},\nu)^{58}Fe$ & 1.47(+15)& 0.994 & & $\rm ^{59}Ni(e^{-},\nu)^{59}Co$ &  7.63(+13)& 0.997 \nl 
$\rm ^{56}Fe(e^{-},\nu)^{56}Mn$ & 1.30(+15)& 0.830 & & $\rm ^{51}Cr(e^{-},\nu)^{51}V $ &  7.57(+13)& 0.999 \nl 
$\rm ^{33}S (e^{-},\nu)^{33}P $ & 1.12(+15)& 0.999 & & $\rm ^{56}Fe(e^{-},\nu)^{56}Mn$ &  6.49(+13)& 0.579 \nl 
$\rm ^{50}Cr(e^{-},\nu)^{50}V $ & 9.44(+14)& 0.999 & & $\rm ^{55}Co(e^{-},\nu)^{55}Fe$ &  2.17(+13)& 0.999 \nl 
$\rm ^{59}Ni(e^{-},\nu)^{59}Co$ & 7.51(+14)& 0.999 & & $\rm ^{52}Cr(e^{-},\nu)^{52}V $ &  1.05(+13)& 0.561 \nl 
$\rm ^{55}Co(e^{-},\nu)^{55}Fe$ & 6.72(+14)& 0.999 & &                                 &           &       \nl 
$\rm ^{52}Cr(e^{-},\nu)^{52}V $ & 6.36(+14)& 0.850 & &                                 &           &       \nl
$\rm ^{35}Cl(e^{-},\nu)^{35}S $ & 6.06(+14)& 0.999 & &                                 &           &       \nl
\cline{1-7}\nl
$\rm ^{52}Cr(n,\gamma)^{53}Cr$\tablenotemark{a} & 1.27(+20)& 2.84(-5)& & $\rm ^{57}Co(\gamma,p)^{56}Fe$\tablenotemark{a} & 1.90(+20)& 4.85(-4)\nl  
\cutinhead{From NSE to collapse}
$\rm ^{54}Mn(e^{-}    ,\nu)^{54}Cr$ & 4.60(+19)& 0.855 & & $\rm ^{55}Fe(e^{-},\nu)^{55}Mn$ &  4.12(+19)& 0.869 \nl
$\rm ^{60}Co(e^{-}    ,\nu)^{60}Fe$ & 3.92(+19)& 0.809 & & $\rm ^{54}Mn(e^{-},\nu)^{54}Cr$ &  2.65(+19)& 0.867 \nl
$\rm ^{58}Co(e^{-}    ,\nu)^{58}Fe$ & 3.45(+19)& 0.961 & & $\rm ^{58}Co(e^{-},\nu)^{58}Fe$ &  2.40(+19)& 0.964 \nl
$\rm ^{55}Fe(e^{-}    ,\nu)^{55}Mn$ & 3.16(+19)& 0.845 & & $\rm ^{53}Mn(e^{-},\nu)^{53}Cr$ &  1.76(+19)& 0.935 \nl
$\rm ^{53}Mn(e^{-}    ,\nu)^{53}Cr$ & 1.49(+19)& 0.934 & & $\rm ^{57}Co(e^{-},\nu)^{57}Fe$ &  1.59(+19)& 0.929 \nl
$\rm ^{59}Fe(\beta^{-},\nu)^{59}Co$ & 1.12(+19)& 0.228 & & $\rm ^{60}Co(e^{-},\nu)^{60}Fe$ &  5.75(+18)& 0.819 \nl
$\rm ^{57}Co(e^{-}    ,\nu)^{57}Fe$ & 1.10(+19)& 0.923 & & $\rm ^{56}Fe(e^{-},\nu)^{56}Mn$ &  5.10(+18)& 0.470 \nl
$\rm ^{57}Mn(\beta^{-},\nu)^{57}Fe$ & 5.83(+18)& 0.305 & & $\rm ^{59}Ni(e^{-},\nu)^{59}Co$ &  4.14(+18)& 0.990 \nl
$\rm ^{56}Fe(e^{-}    ,\nu)^{56}Mn$ & 5.27(+18)& 0.231 & & $\rm ^{51}Cr(e^{-},\nu)^{51}V $ &  1.21(+18)& 0.997 \nl
$\rm ^{59}Ni(e^{-}    ,\nu)^{59}Co$ & 2.29(+18)& 0.992 & & $\rm ^{56}Co(e^{-},\nu)^{56}Fe$ &  1.06(+18)& 0.998 \nl
$\rm ^{60}Co(\beta^{-},\nu)^{60}Ni$ & 1.71(+18)& 0.260 & & $\rm ^{57}Mn(e^{-},\nu)^{57}Fe$ &  9.35(+17)& 0.227 \nl
$\rm ^{55}Cr(\beta^{-},\nu)^{55}Mn$ & 1.04(+18)& 0.171 & & $\rm ^{54}Fe(e^{-},\nu)^{54}Mn$ &  8.58(+17)& 0.958 \nl
$\rm ^{51}Cr(e^{-}    ,\nu)^{51}V $ & 7.92(+17)& 0.998 & & $\rm ^{52}Cr(e^{-},\nu)^{52}V $ &  3.93(+17)& 0.369 \nl
$\rm ^{52}Cr(e^{-}    ,\nu)^{52}V $ & 3.73(+17)& 0.170 & & $\rm ^{59}Co(e^{-},\nu)^{59}Fe$ &  3.06(+17)& 0.031 \nl
$\rm ^{50}V (e^{-}    ,\nu)^{50}Ti$ & 2.33(+17)& 0.998 & & $\rm ^{60}Co(e^{-},\nu)^{60}Ni$ &  2.35(+17)& 0.067 \nl
$\rm ^{54}Fe(e^{-}    ,\nu)^{54}Mn$ & 2.04(+17)& 0.950 & & $\rm ^{50}V (e^{-},\nu)^{50}Ti$ &  1.83(+17)& 0.997 \nl
$\rm ^{56}Co(e^{-}    ,\nu)^{56}Fe$ & 1.75(+17)& 0.999 & & $\rm ^{58}Ni(e^{-},\nu)^{58}Co$ &  9.90(+16)& 0.919 \nl
$\rm ^{51}V (e^{-}    ,\nu)^{51}Ti$ & 1.05(+17)& 0.350 & & $\rm   p    (e^{-},\nu)n      $ &  6.93(+16)& 0.995 \nl
$\rm ^{49}V (e^{-}    ,\nu)^{49}Ti$ & 3.07(+16)& 0.994 & &                                 &           &       \nl
$\rm ^{58}Ni(e^{-}    ,\nu)^{58}Co$ & 1.47(+16)& 0.888 & &                                 &           &       \nl
$\rm ^{49}Ti(e^{-}    ,\nu)^{49}Sc$ & 8.37(+15)& 0.868 & &                                 &           &       \nl
$\rm      p (e^{-}    ,\nu)n      $ & 8.11(+15)& 0.997 & &                                 &           &       \nl
\tablenotetext{a}{Nuclear reaction having the maximum integrated flux}
\enddata        
\end{deluxetable}


==> tablsc9.tex <==
\begin{deluxetable}{lrrrr}
%\small
\tablenum{9}
\tablewidth{10cm}
\tablecaption{Key zones which keep track of the various nuclear burnings 
for $\rm 13~M_\odot$, $\rm 15~M_\odot$, $\rm 20~M_\odot$ and $\rm 25~M_\odot$ models.}
\tablehead{
\colhead{Nuclear burning}     &
\colhead{$\rm 13~M_\odot$}    &
\colhead{$\rm 15~M_\odot$}    &
\colhead{$\rm 20~M_\odot$}    &
\colhead{$\rm 25~M_\odot$}    
}
\startdata  
                     &  13.000  &  15.000  & 20.000  & 25.000  \nl
Hydrogen (Central)   &          &          &         &         \nl
                     &   3.477  &   4.282  &  6.152  &  8.269  \nl
Hydrogen (Shell)     &          &          &         &         \nl
                     &   3.066  &   3.520  &  5.585  &  7.638  \nl
Helium (Shell)       &          &          &         &         \nl
                     &   1.751  &   2.323  &  3.630  &  5.190  \nl
Helium (Central)     &          &          &         &         \nl
                     &   1.749  &   2.174  &  2.850  &  4.560  \nl
Carbon               &          &          &         &         \nl
                     &   1.503  &   1.754  &  2.370  &  2.937  \nl
Neon                 &          &          &         &         \nl
                     &   1.390  &   1.643  &  2.144  &  2.113  \nl
Oxygen               &          &          &         &         \nl
                     &   1.290  &   1.429  &  1.551  &  1.569  \nl
Silicon              &          &          &         &         \nl
                     &   0.740  &   1.080  &  1.105  &  1.370  \nl
NSE                  &          &          &         &         \nl
                     &   0.000  &   0.000  &  0.000  &  0.000  \nl
\enddata        
\end{deluxetable}

